Bolt-Dumbo Transformer: Asynchronous Consensus As Fast As the Pipelined BFT

An urgent demand of deploying BFT consensus over the Internet is raised for implementing blockchain services. The deterministic (partial) synchronous protocols can be simple and fast in good network conditions, but are subject to denial-of-service when synchrony assumption fails. Asynchronous protocols, on the contrary, are robust against the adversarial network, but are substantially more complicated and slower for the inherent use of randomness. Facing the issues, optimistic asynchronous atomic broadcast ( Kursawe-Shoup, 2002; Ramasamy-Cachin, 2005) was proposed to improve the normal-case performance of the slow asynchronous consensus. They run a deterministic fastlane if the network condition remains good, and can fall back to a fully asynchronous protocol via a pace-synchronization mechanism if the fastlane fails. Unfortunately, existing pace-synchronization directly uses a heavy tool of asynchronous multi-valued validated Byzantine agreement (MVBA). We present Bolt-Dumbo Transformer (BDT), a generic framework for practical optimistic asynchronous atomic broadcast. At the core of BDT, we set forth a new fastlane abstraction that is simple and fast, while preparing honest parties to gracefully face potential fastlane failures caused by malicious leader or bad network. This enables a highly efficient pace-synchronization to handle fallback. The resulting design reduces a cumbersome MVBA to a variant of the conceptually simplest binary agreement only. Besides detailed security analyses, we also give concrete instantiations of our framework and implement them. Extensive experiments demonstrate that BDT can enjoy both the low latency of deterministic protocols (e.g. 2-chain version of HotStuff) and the robustness of state-of-the-art asynchronous protocols in practice.

==> CCS 22 long-version/analysis.tex <==
%!TEX root = main.tex

%\subsection{Security of $\sys$}
%\label{sec:boltanalysis}


%In this section, we prove that   $\sys$    satisfies all properties of atomic broadcast in the asynchronous network against   computationally bounded adversary. For   brevity, we might omit to mention that all  statements   hold with all but negligible probabilities and all  messages/subprotocols in discussions are associated to the same epoch.




 \smallskip
\noindent
{\bf Security intuitions.} We brief the   security  intuitions of      $\BDT$   in the following, and defer   detailed proofs to Appendix \ref{append:bdt} for space limit. 

%\begin{itemize}
	%\smallskip
	 	\noindent
	 \underline{\smash{\em Safety}}. The core ideas of proving agreement and total-order are:
	 \vspace{-0.1cm}
	 \begin{itemize}[leftmargin=0.6cm]
	 	\item {\em $\trans$ returns a common index}. All honest parties must obtain the same block index from $\trans$, so they always agree the same fastlane block to continue the pessimistic path (or retry the fastlane). This is ensured by   $\tcvba$'s agreement.
	 	\item {\em $\trans$ returns an index   not ``too large''}. For the index returned from $\trans$, at least $f+1$ honest parties did receive all blocks (with valid proofs) up to this index. As such, if any party misses some blocks, it can easily fetch the correct blocks from these $f+1$ parties. 
	 	%
	 	This is because the notarizability of $\tobc$ prevents the adversary from forging a proof for a fastlane block with an index higher than the actually delivered block. So no honest party would input some index of an irretrievable block to $\tcvba$, and then the validity of $\tcvba$ simply guarantees the claim.
	 	
	 	\item {\em $\trans$ returns an index   not ``too small''}. No honest party would revoke any fastlane block that was already committed as a finalized output. Since each honest party waits for $2f+1$  $\view$ messages   from distinct parties, then due to the  notarizability of $\tobc$, there is at least one $\view$ message contains $s-1$, where $s$ is the latest fastlane block (among all parties). So every honest party at least inputs $\tcvba$ with $s-1$. The validity of $\tcvba$ then ensures the output at least to be $s-1$ as well.
	 	Recall that there is   a ``safe buffer'' to hold the latest fastlane block as a pending one, the claim is then correct.
	 	
	 	\item {\em Pessimistic path and fastlane are safe}. Pessimistic path is trivially safe due to its agreement and total order. Fastlane  has total-order by definition, and its weaker agreement (notarizability) is complemented by $\trans$ as argued above.
	 \end{itemize}
	
 %\vspace{-0.1cm}
	\noindent
	 \underline{\smash{\em Liveness}}. This stems from  the liveness of all three phases.	 
	 The liveness of fastlane is guaranteed by the ``timeout'' parameter $\tau$. That means, all honest parties can leave the fastlanes without  ``getting stuck''.  %So all honest parties will mulitcast $\view$ messages  and  therefore   switch to the $\trans$ phase. 
	%
	After that, all parties would invoke $\tcvba$  and   obtain $\mathsf{syncPace}$ as the $\tcvba$  output due to the termination   of   $\tcvba$; moreover, if any honest party realizes that it misses some fastlane blocks after obtaining $\mathsf{syncPace}$, it can   sync up to   $\mathsf{syncPace}$ within only two asynchronous rounds, because at least $f+1$ honest parties can help it to fetch the missing blocks. So no honest party would ``stuck'' during the $\trans$ phase.
	%
	Finally, the honest parties would enter the $\Pessimistic$ phase if the fastlanes completely fail to output nothing. After that, the protocol must   output expected $\bigO(B)$-sized transactions, and ensures that  any transactions (at the $B$-top of all honest parties' backlogs) can output with a constant probability, 
	thus ensuring liveness even if in the worst case.
	


	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\ignore{		
		\item {\em Liveness and safety of $\trans$}. It is easy to see that once an honest party switches to the $\trans$ phase of the epoch $e$, then all honest parties will do so, because   an honest party starts $\trans$ only if it has   received  at least $n-f$ $\view$ messages from distinct parties for epoch $e$, indicating that at least those $f+1$ honest parties abandon    $\tobc[e]$. As a result,
		the $\tobc[e]$ instance would no longer output any valid block to any honest parties, so all honest parties' timers must     interrupt and then abandon $\tobc[e]$ in at most $\bigO(\tau)$ asynchronous rounds.
		
		Clearly, this induces that all honest parties will mulitcast $\view$ messages  and  therefore   switch to the $\trans$ phase of the epoch $e$. 
		After that, all of them would invoke $\tcvba$  and then obtain $s$ as the $\tcvba[e]$  output due to the termination property of the $\tcvba$ primitive. As such, no honest party would ``stuck'' during the $\trans$ phase.
				
		\item  {\em Optimistic liveness and safety of  $\tobc$}. During the  $\tobc$ phase, there would be no violation of the total-order since the fastlane itself also enjoys the property.
		The probable disagreement during the phase would be eventually fixed by the $\trans$ phase, since the $\tcvba$ module in $\trans$ would make all parties reach an agreement to sync up to a common optimistic path block.

		\item  {\em Liveness and safety of  $\dumbo$}. This can be easily seen as  this phase is a fully-fledged asynchronous protocol.}
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\end{itemize}



\smallskip
	\noindent{\bf Efficiency analysis.} The complexities can be analyzed by counting these of each underlying module.
	Overall, $\mathsf{BDT}$ would cost (expected) $\bigO(n)$ communicated  bits per output transaction, %in both optimistic cases (where the synchrony assumption holds) and pessimistic cases (where the network becomes asynchronous). 
	and the  latency of each output block is of expected constant rounds. 
	These  complexities hold in all cases (no matter the network   is synchronous or asynchronous). 
	We defer such tedious counting on the number  of exchanged bits and  execution rounds to Section \ref{sec:complex}. 


\smallskip
\noindent{\bf Optimistic conditions.} 
%Besides securely implementing fully asynchronous atomic broadcast, 
$\BDT$ has a simple and efficient deterministic fastlane that might  keep on progressing
under certain optimistic conditions, which intuitively are: (i) the actual network delay is smaller than some guessed timing parameter and (ii) the leader of fastlane is honest.
In Appendix \ref{app:optimistic}, we discuss why such optimistic conditions  can ensure  the progress of fastlanes.


\ignore{
	##############################################################################################################
	##############################################################################################################

	
\noindent
{\bf Safety proof}. We first prove the  total-order and agreement, assuming the underlying $\tobc$, $\tcvba$ and $\acs$ are secure.


\begin{claim}
	\label{aa}
	If an honest party activates $\tcvba[e]$,   then at least $n-2f$ honest parties have already invoked $\abandon(e)$, and from now on: suppose these same parties invoke $\abandon(\id)$ before they output $\block$:=$ \langle e, R, \cdot,\cdot \rangle $, then	any party (including the faulty ones) cannot receive (or forge) a valid $\block$:=$ \langle e, R+1, \cdot,\cdot  \rangle $, and all honest parties  would activate $ \tcvba[e]$. 
	
	%	Besides, if these same parties invoke $\abandon(\id)$ before they output $\block$:=$ \langle e, R, *,* \rangle $, then	any party (including the faulty ones) cannot receive (or forge) a valid $\block$:=$ \langle e, R+1, *,* \rangle $. 	
\end{claim}


{\em Proof:} When  an honest party $\node_i$ activates $ \tcvba[e]$, it must have received $n-f$ valid $\view$ messages from distinct parties, so there would be at least $n-2f$ honest parties multicast $\view$ messages. By the pseudocode, it also means that  at least $n-2f$ honest parties have invoked $\abandon(e)$. Note that $n-2f\ge f+1$ and these same parties invoke $\abandon(\id)$ before they output $\block$:=$ \langle e, R, \cdot,\cdot  \rangle $, so no party would deliver any valid $\block$:=$ \langle e, R+1, \cdot,\cdot  \rangle $ in this epoch's $\tobc$ phase due to the {\em abandonability} property of $\tobc$. It is also implies that any parties cannot from the $\tobc$ receive valid  $\block$:=$ \langle e, R+1, \cdot,\cdot  \rangle $ , then all honest parties will eventually be interrupted by the ``timeout'' mechanism after $\tau$ asynchronous rounds and then multicast $\view$ messages. This   ensures that all honest parties finally receive $n-f$ valid $\view$ messages from distinct parties, causing all honest parties to activate $ \tcvba[e]$. 
$\hfill\square$ 




\begin{claim}
	Suppose that  some party receives a valid $\block$:=$\langle e, R, \cdot , \cdot\rangle$ from $\tobc[e]$ when an honest party invokes $ \tcvba[e]$ s.t. this $\block$ is the one with largest slot number among all parties' valid $\notarized$ blocks (which means the union of the honest parties' actual $\notarized$ blocks and the malicious parties' arbitrary  valid  $\tobc[e]$ block), 	then all honest parties'     $\maxview_e$ must be same and be either $R$ or $R-1$.
	\label{dd}
\end{claim}	

{\em Proof:}
Following   Claim \ref{aa}, once an honest party invokes $ \tcvba[e]$, 
the $\tobc[e]$ $\block$ with the largest slot number $R_{max}$ would not change anymore.
Let us call this already fixed $\tobc[e]$ $\block$ with highest slot number as $\block_{max}$.
Since there is someone that receives $\block_{max}$:=$\langle e, R, \cdot , \cdot\rangle$,
at least $f+1$ honest parties (e.g., denoted by $Q$) have already received the block $\langle e, R-1, \cdot , \cdot\rangle$,
which is because of the {\em notarizability} property of $\tobc$. 
So these honest parties would broadcast a valid $\view(e, R-1,\cdot)$ message or a valid $\view(e, R,\cdot)$ message. 
%
According to the pseudocode in Figure \ref{fig:mule}, $\maxview_e$ is the maximum number in the set of $\mathsf{Paces}_e$, where       $\mathsf{Paces}_e$ contains the slot numbers encapsulated by $n-f$ valid $\view$ messages. Therefore, $\mathsf{Paces}_e$ must contain one $\view$ message's slot number from at least $n-2f \ge f+1$ honest parties (e.g., denoted by $\bar{Q}$). 
All honest parties' local $\mathsf{Paces}_e$ set must   contain $R-1$ and/or $R$, because $\bar{Q}$ and $Q$ contain at least one common honest party. Moreover, there is no valid $\view$ message containing any slot larger than $R$ since the proof for that is unforgeable, which means $R$ is the largest possible value in all honest parties' $\mathsf{Paces}_e$. So any honest party's $\maxview_e$ must be     $R$ or $R-1$.
$\hfill\square$ 



\begin{claim}
	No honest party would get a $\mathsf{syncPace}_e$ smaller than the slot number of it latest finalized block $\out[-1]$ (i.e., no block  finalized in some honest party's $\out$ can   be revoked).
	\label{norevoke}
\end{claim}

{\em Proof:} 
Suppose an honest party invokes $ \tcvba[e]$ and a valid $\tobc[e]$  block $\langle e, R, \cdot , \cdot\rangle$ is the one with largest slot number among  the union of the honest parties' actual $\notarized$ blocks and the malicious parties' arbitrary  valid  $\tobc[e]$ block. Because of Claim \ref{dd}, all honest parties will activate $\tcvba[e]$ with taking either $R$ or $R-1$ as input. According to the {\em strong validity} of  $\tcvba$, the output $\mathsf{syncPace}_e$ of $\tcvba[e]$  must be either $R$ or $R-1$. 
Then we consider the next two cases:

\begin{enumerate}
	\item Only malicious parties have this  $\langle e, R, \cdot , \cdot\rangle$ block;
	
	\item Some honest party $\node_{i}$ also has the $\langle e, R, \cdot , \cdot\rangle$ block.
\end{enumerate}	

{\em For Case 1)} Due to the {\em notarizability} property of $\tobc$ and this case's baseline, there exist $f+1$ honest parties (denoted by a set   $Q$) have  the block $\langle e, R-1, \cdot , \cdot\rangle$ as their local $\notarized$. 
Note that remaining honest parties  (denoted by a set   $\bar{Q}$) would have local $\notarized$ block not higher than $R-1$.  According to the algorithm in Figure \ref{fig:mule}, we can state that: 
(i) if the output is $R$, then all honest parties will sync their $\out$ up to the block  $\langle e, R, \cdot , \cdot\rangle$ (which include all honest parties' local $\notarized$); 
(ii) similarly, if the output is $R-1$, all honest parties will sync up till $\langle e, R-1, \cdot , \cdot\rangle$ (which also include all honest parties' local $\notarized$). So in this case, all honest parties (i.e., $\bar{Q} \cup Q$) will not discard their $\notarized$ $\block$, let alone discard some $\tobc$ that are already finalized to output into $\out$.


{\em For Case 2)} Let $Q$ denote the set of honest parties that have  the block $\langle e, R, \cdot , \cdot\rangle$ as their local $\notarized$. 
Note the remaining honest parties $\bar{Q}$ would have the $\notarized$ block not higher than $R$. In this case,  following the algorithm in Figure \ref{fig:mule}, we can see that: 
(i) if the output is $R$, then all honest parties will sync their $\out$ up to the block  $\langle e, R, \cdot , \cdot\rangle$ (which include all honest parties' local $\notarized$); 
(ii) similarly, if the output is $R-1$, all honest parties will sync up to $\langle e, R-1, \cdot , \cdot\rangle$ (which include $\bar{Q}$ parties' local $\notarized$ and ${Q}$ parties' finalized output $\out$). So in this case, all honest parties (i.e., $\bar{Q} \cup Q$) will not discard any block in their finalized  $\out$.
$\hfill\square$ 



\begin{claim}
	If $\tcvba[e]$ returns $\mathsf{syncPace}_e$, then at least $f+1$ honest parties  can append $\block$s with slot numbers from $1$ to $\mathsf{syncPace}_e$ from $\tobc[e]$  into the $\out$ without invoking $\gethelp$  function.
	\label{provable}
\end{claim}	

{\em Proof:}
Suppose $\tcvba[e]$ returns $\mathsf{syncPace}_e$, according to the {\em strong validity}  of $\tcvba$, then at least one honest party inputs the number $\mathsf{syncPace}_e$. The same honest party must receive a valid message 	$\view(e, \mathsf{syncPace}_e, \prf)$, 
which means there must exists a valid   $\tobc$ block  $\langle e, \mathsf{syncPace}_e, \cdot , \prf \rangle$. Following the pseudocode, the honest party will multicst $\view(e, \mathsf{syncPace}_e, \prf)$ if $\tcvba[e]$ returns $\mathsf{syncPace}_e$, then all honest parties can get the $\prf$. According to the {\em notarizability} and {\em total-order} properties of $\tobc$, at least $f+1$ honest parties  can append  $\block$s  from $\langle e, 1, \cdot , \cdot\rangle$ to $\langle e, \mathsf{syncPace}_e, \cdot , \cdot\rangle$ into the $\out$ without invoking $\gethelp$  function..
$\hfill\square$ 



\begin{claim}
	\label{callhelp}
	If an honest party invokes $\gethelp$  function to retrieve a block $\out[i]$, it eventually can get it;
	if another honest party   retrieves a block $\out[i]'$   at the same log position $i$ from the $\gethelp$ function, then $\out[i]= \out[i]'$.
\end{claim}	

{\em Proof:} Due to Claim \ref{provable} and {\em total-order} properties of $\tobc$, any block $\out[i]$ that an honest party is retrieving through $\gethelp$ function shall have been in the output $\log$ of at least $f+1$ honest parties, so it eventually can get $f+1$ correct $\hlp$ messages with the same Merkle tree root $h$ from distinct parties, then it can interpolate the $f+1$ leaves to reconstruct $\out[i]$ which is same to other honest parties' local $\out[i]$. 
%
We can argue the agreement by contradiction, in case the interpolation of honest party  fails or it recovers a block $\out'[i]$ different from the the honest party's local $\out[i]$, that means the Merkle tree with root $h$ commits some leaves that are not coded fragments of  $\out[i]$; nevertheless, there is at least one honest party encode $\out[i]$ and commits the block's erasure code to have a Merkle tree root $h$; so the adversary indeed breaks the collision resistance of Merkle tree, implying the break of the collision-resistance of hash function, which is computationally infeasible. So all honest parties that attempt to retrieve a missing block $\out[i]$ must   fetch the block consistent to other honest parties'.
$\hfill\square$ 



\begin{lemma}
	\label{agreement}
	If all honest parties enter the  $\tobc$ phase with the same $\out$, then they will always finish the  $\trans$ phase with still having the same   $\out'$. 
\end{lemma}

{\em Proof:} 
When all honest parties enter the epoch with the same $\out$, it is easy to see that they all will eventually raise some interruption to abandon the $\tobc$ phase.	
Due to Claim \ref{aa},  all honest parties  would activate $\tcvba[e]$. Following the  {\em agreement and termination} of $\tcvba[e]$, all parties would finish $\tcvba[e]$ to get a common $\mathsf{syncPace}_e$  and then sync up to the same $\out$ with the highest slot number $\mathsf{syncPace}_e$ (due to {\em total-order} properties of $\tobc$, Claim \ref{provable} and Claim \ref{callhelp}), and hence all parties will finish the  $\trans$ phase with   the same output $\out$.
$\hfill\square$ 


\begin{lemma}
	\label{order}
	For any two honest parties before finishing the  $\trans$ phase, then 
	%If any two honest parties are both staying in the  $\tobc$ phase or the  $\trans$ phase,
	there exists one party, such that its $\out$ is a prefix of (or equal to) the other's.
\end{lemma}

{\em Proof:} The blocks outputted before the completion of the  $\trans$ phase were originally generated from the $\tobc$ phase, then the Lemma holds immediately by following the {\em total-order} property of $\tobc$ and Claim \ref{norevoke}.
$\hfill\square$ 




\begin{lemma}
	\label{dumbo}
	If any honest party enters the  $\Pessimistic$ phase, then all honest parties will enters the phase and
	always leave the  phase with having the same   $\out$.
\end{lemma}

{\em Proof:} If any honest party enter the $\Pessimistic$ phase, all honest parties would enter this phase, which is due to Claim \ref{aa}, the {\em agreement and termination} property of $\tcvba$ and $\mathsf{syncPace}_e=0$.
Let us assume that all honest parties enter the $\Pessimistic$ phase with the same $\out$, it would be trivial too see the statement for the agreement and termination properties of $\acs$ and the correct and robustness properties of threshold public key encryption.
Then considering Lemma \ref{agreement} and the simple fact that all honest parties activate with the common empty $\out$,
we can inductively reason that all honest parties must enter any $\Pessimistic$ phase with the same $\out$. So the Lemma holds.
$\hfill\square$ 



\begin{lemma}
	\label{orderr}
	For any two honest parties   in the same epoch,  
	there exists one party, such that its $\out$ is a prefix of (or equal to) the other's. 
\end{lemma}

{\em Proof:} 
If two honest parties do not enter the $\Pessimistic$ phase during the epoch, 
both of them only participate in $\tobc$ or $\trans$, so this Lemma holds immediately by following Lemma \ref{order}.
For two honest parties that one enters the $\Pessimistic$ phase and one does not, this Lemma holds because the latter one's $\out$ is either a prefix of the former one's or equal to the former one's due to Lemma  \ref{agreement} and \ref{order}.
For the remaining case that both   honest parties   enter the $\Pessimistic$ phase, they must   initially have exactly same $\out$ (due to Lemma \ref{agreement}).
Moreover, in the phase, all honest parties would execute the $\acs$ instances in a sequential manner (e.g., there is only one $\acs$ instance in our exemplary pseudocode), 
so every honest party would output in one ACS instance only if it has already outputted in all earlier ACS instances.
Besides,  any two honest party would output the same transaction batch in every $\acs$ instance for the agreement property of $\acs$.
So this Lemma also holds for any two honest parties that are staying in the same epoch.
$\hfill\square$ 



\begin{theorem}
	\label{key1}
	The $\sys$ protocol satisfies the {\em agreement} and {\em total order} properties.
\end{theorem}	

{\em Proof:}
The {total order} be induced by Lemma \ref{orderr} along with the fact the protocol is executed epoch by epoch. 
The agreement  follows immediately from   Lemma \ref{agreement}  and \ref{dumbo} along with the fact that all honest parties initialize with the same empty $\out$ to enter the first epoch's $\tobc$ phase.
$\hfill\square$ 




\noindent
{\bf Liveness proof}. Then we prove the liveness property of $\sys$.

\begin{lemma}
	\label{boltlive} Once all honest parties enter the $\tobc$ phase, they must leave the phase in at most constant asynchronous rounds and then all enter the $\trans$ phase.
\end{lemma}

{\em Proof:} At worst case, all honest parties' timeout  will  interrupt, causing them to abandon the $\tobc$ phase in at most $\tau+\kappa Esize$ asynchronous rounds,
where $\kappa$, according to the {\em optimistic liveness} property of $\tobc$, is a tiny constant  that represents the running time of generating a new optimistic $\tobc$ block and depends on the underlying $\tobc$ instantiation (e.g., it is two in the  $\mathsf{Bolt}$-$\mathsf{sCAST}$ instantiation). 
Upon timeout, the broadcast of $\view$ message will take one more asynchronous round. After that, all honest parties would receive enough $\view$ messages to enter the $\trans$ phase, which costs at most $\tau+\kappa Esize + 1$ asynchronous rounds. 
$\hfill\square$ 



\begin{lemma}
	\label{translive}  If all honest parties enter the $\trans$ phase, they all leave the phase in expected constant asynchronous rounds and then either enter the $\Pessimistic$ phase or enter the next epoch's $\tobc$ phase.
\end{lemma}

{\em Proof:} 
If all honest parties enter the $\trans$ phase, it
is trivial to see the Lemma since the underlying $\tcvba$ terminates in on-average constant asynchronous rounds. If the output of $\tcvba$ equal 0, then enter the $\Pessimistic$ phase, otherwise,   enter the next epoch's $\tobc$ phase.
$\hfill\square$ 


\begin{lemma}
	\label{dumbolive} If all honest parties enter the $\Pessimistic$ phase, all honest parties will leave this $\Pessimistic$ phase in on-average constant asynchronous rounds with outputting some blocks containing on-average $\bigO(B)$-sized transactions. 
\end{lemma}

{\em Proof:} 
Similar to \cite{honeybadger}'s analysis, $\Pessimistic$ at least outputs $\bigO(B)$-sized transactions (without worrying that the adversary can learn any bit about the transactions to be outputted before they are actually finalized as output) for each execution. Here we remark that the original analysis in \cite{honeybadger} only requires IND-CPA security of threshold  public key encryption might be not enough, since we need to simulate that the adversary can query decryption oracle by inserting her ciphertext into the ACS output. Moreover, the underlying $\dumbo$ ACS construction \cite{guo2020dumbo}   ensures all parties to leave the phase in on-average constant asynchronous rounds.
$\hfill\square$ 



\begin{theorem}
	\label{key2}	
	The $\sys$ protocol satisfies the {\em liveness} property.
\end{theorem}	


{\em Proof:}
Due to Lemma \ref{boltlive} and \ref{translive}, the adversary would not be able to stuck the honest parties during the $\tobc$ and $\trans$ phases.
%
Even if in the worst cases, the two phases do not deliver any useful output and the adversary intends to prevent the parties from running the
$\Pessimistic$ phase (thus not eliminating any transactions from the honest parties' input buffer),
we still have a  timeout mechanism against censorship, which can ensure to execute the $\Pessimistic$ phase for every $\bigO(T)$ asynchronous rounds if there is a suspiciously censored $\tx$ in all honest parties' buffers due to some timeout parameter $T$. 
%
Recall Lemma \ref{dumbolive}, for each $\tx$ in all honest parties' buffers, it would take $\bigO(XT/B)$ asynchronous rounds at worst (i.e., we always rely on the timeout $T$ to invoke the $\Pessimistic$ phase) to make   $\tx$ be one of the top $B$ transactions in all parties' buffers, where $X$ is the bound of buffer size (e.g., an unfixed polynomial in $\lambda$).
After that, any luckily finalized optimistic phase block would output $\tx$ (in few more $\delta$), or still relying on the timeout to invoke the $\Pessimistic$ phase, causing the worst case latency $\bigO( (X/B + \lambda)\delta T)$, which is a function in the actual network delay $\delta$ factored by some  (unfixed) polynomial of security parameters. 
$\hfill\square$ 

##############################################################################################################
##############################################################################################################
}




\input{evaluation}





\ignore{
	

	##############################################################################################################
	##############################################################################################################
	##############################################################################################################
	##############################################################################################################
	

	
\section{Complexity and Numerical Analyses} 
\label{sec:ca}


This section   discusses the critical complexity metrics   of  the $\sys$  framework and its key modules. 
It then  assigns   each module    a running time cost according to our real-world experimental data, 
thus enabling more precise numerical analysis to estimate the expected latency of $\mathsf{BDT}$ in various ``simulated'' unstable deployment environments.



\noindent
{\bf Complexity analysis}.
Here we analyze the complexities of $\sys$ regarding its performance metrics. 

For the optimistic path $\tobc$, we have two instantiations, namely $\mathsf{Bolt}$-$\mathsf{sCAST}$ and $\mathsf{Bolt}$-$\mathsf{sRBC}$. As shown in Table \ref{tab:tobc},
$\mathsf{Bolt}$-$\mathsf{sCAST}$ is with linear $\mathcal{O}(n)$ per-block message complexity, and the leader's per-block bandwidth usage$\mathcal{O}(nB)$ is also linear in $n$;
$\mathsf{Bolt}$-$\mathsf{sRBC}$ is with quadratic per-block message complexity as $\mathcal{O}(n^2)$, while the per-block bandwidth usage of every party is not larger than the batch size $\mathcal{O}(B)$; for both ``fastlane'' instantiations, though the generation of each $\mathsf{Bolt}$ block will cost exact $\mathcal{O}(1)$ rounds, $\mathsf{Bolt}$-$\mathsf{sCAST}$ uses slightly less concrete asynchronous rounds on average.


\begin{table}[h]
	%	\vspace{-0.3cm}
	\caption{Per-block Performance    of Different \Bolt\/ Instantiations (also Per-block Cost of  {\sf BDT}  in Optimistic Case)}
	\label{tab:tobc}
	\centering
	\begin{footnotesize}
		\begin{tabular}{c|c|c|c|c|c}
			\hline\hline\rule{0pt}{10pt}
			\multirow{2}{*}{} & \multirow{2}{*}{Msg.} & \multirow{2}{*}{Comm.} & \multirow{2}{*}{Round} & \multicolumn{2}{c}{Bandwidth Cost} \\ \cline{5-6} \rule{0pt}{10pt}
			&                       &                &        & Leader               & Others              \\ \hline\rule{0pt}{10pt}
			$\mathsf{Bolt}$-$\mathsf{sCAST}$               & $\mathcal{O}(n)$                   & $\mathcal{O}(nB)$  &   $\bigO(1)$               &  $\mathcal{O}(nB)$                 &  $\mathcal{O}(B)$                \\ \hline\rule{0pt}{10pt}
			$\mathsf{Bolt}$-$\mathsf{sRBC}$                   &$\mathcal{O}(n^2)$                   & $\mathcal{O}(nB)$      &   $\bigO(1)$          &$\mathcal{O}(B)$             & $\mathcal{O}(B)$              \\ \hline\hline
		\end{tabular}
	\end{footnotesize}
	%	\vspace{-0.1cm}
\end{table}

In addition, there is a worst-case overhead of $\bigO(\tau)$ asynchronous rounds to leave this phase without outputting any valid blocks.
%without generating any meaningful blocks.
%
During the $\trans$ phase, all parties would participate in $\tcvba$, in which the message complexity is  $\mathcal{O}(n^2)$,  the communication complexity is $\mathcal{O}(\lambda n^2)$, and the bandwidth cost of each parties is $\mathcal{O}(\lambda n)$. Besides, if the output value of $\tcvba$ is large than zero, then the $\gethelp$ subroutine could probably be invoked, this process will incur $\mathcal{O}(n^2)$ overall message complexity and $\mathcal{O}(nB)$ per-block communication complexity, and causes each party to spend $\mathcal{O}(B)$ bandwidth to fetch each block.  

Note that in the {\em optimistic case} when (i) the fastlane leaders are always honest and (ii) the network condition is benign such that the fastlanes never timeout, the $\Pessimistic$ phase is not executed, 
%and the $\trans$ phase is executed for every $Esize$   blocks, 
so the fastlane cost shown in Table \ref{tab:tobc} would also reflect the amortized complexities of the overall $\mathsf{BDT}$ protocol (in case that the epoch size $Esize$ is   large enough, e.g., $n$).


\begin{table}[h]
	\caption{Per-block Performance of $\mathsf{BDT}$ in Worst Case}
	\label{tab:bolt}
	\centering
	\begin{footnotesize}
		\begin{tabular}{c|c|c|c|c|c}
			\hline\hline\rule{0pt}{10pt}
			\multirow{2}{*}{} & \multirow{2}{*}{Msg.} & \multirow{2}{*}{Comm.} & \multirow{2}{*}{Round} & \multicolumn{2}{c}{Bandwidth Cost} \\ \cline{5-6} \rule{0pt}{10pt}
			&                       &                 &       & Leader               & Others              \\ \hline\rule{0pt}{10pt}
			$\mathsf{BDT}$-$\mathsf{sCAST}$           & $\mathcal{O}(n^3)$                   & $\mathcal{O}(nB)$        &    $\bigO(\tau)$$^*$      &  $\mathcal{O}(nB)$                 &  $\mathcal{O}(B)$                \\ \hline\rule{0pt}{10pt}
			$\mathsf{BDT}$-$\mathsf{sRBC}$                 &$\mathcal{O}(n^3)$                   & $\mathcal{O}(nB)$      &     $\bigO(\tau)$$^*$     & $\mathcal{O}(B)$               & $\mathcal{O}(B)$                \\ \hline\hline
		\end{tabular}
	\end{footnotesize}
	\\{\ }
	{\footnotesize
		\begin{spacing}{1.0}
			$^*$ Note that  $\bigO(\tau)$ can be close to $\bigO(1)$, since we essentially let $\tau$ ``clock ticks'' to approximate  the   period of ``heartbeats''  (i.e., generate a new block) in   the $\mathsf{Bolt}$ path. %which essentially are     generated per $\bigO(1)$ asynchronous rounds.   
		\end{spacing}
	}
	%\vspace{-0.3cm}
\end{table}


In the pessimistic phase, all parties participate in $\dumbo$ BFT protocol, which incurs   $\mathcal{O}(n^3)$ overall message complexity,  $\mathcal{O}(nB)$  overall communication complexity,  and $\mathcal{O}(B)$ bandwidth usage for each party. The latency of generating a block during this phase is of $\bigO(1)$ rounds on average. 
%
To summarize these, we can have the worst-case per-block performance illustrated in Table \ref{tab:bolt}.
%, in which $\mathsf{BDT}$-$\mathsf{HS}$ means $\sys$ with using $\mathsf{Bolt}$-$\mathsf{HS}$ as fastlane and $\mathsf{BDT}$-$\mathsf{RBC}$ is the instantiation using $\mathsf{Bolt}$-$\mathsf{RBC}$ as fastlane.
Note that 
%their major difference is the fastlane  leader's per-block bandwidth usage, and 
the $\bigO(\tau)$ worst-case running time of generating a block reflects two possible worst cases: (i) the fastlane finalizes few blocks (e.g., one) and then times out, so $\bigO(\tau)$ has to be added to the few fastlane blocks; or (ii) the fastlane finalizes nothing and then times out, and thus   $\bigO(\tau)$ must be added to the pessimistic $\dumbo$ blocks. 
Nevertheless, the timeout parameter $\tau$ in our system is not necessarily close to the network delay upper bound $\Delta$, 
and it can represent  some adversary-controlling ``clock ticks''  to approximate   the number of asynchronous rounds spent to generate each fastlane block, i.e., $\bigO(\tau) = \bigO(1)$. 
%To reflect the theoretic merit  in real-world implementations, $\tau$ can be set aggressively to estimate  the actual  global Internet delay on  good days instead of the delay upper bound to cover all cases. %(c.f. Section \ref{sec:def} for the  clock ``implementation'').



\begin{table}[h]
	\begin{center}
		\centering
		
		\begin{footnotesize}
			\newcommand\xrowht[2][0]{\addstackgap[.5\dimexpr#2\relax]{\vphantom{#1}}}
			%\fontsize{6.5}{8}\selectfont  
			\caption{Complexities of BFT protocols in various settings
				(where $B$ is sufficiently large s.t. all $\lambda$ terms are omitted, and $\alpha + \beta =1$)}  
			\label{tab:performance_comparison}  
			%\vspace{-0.5cm}
			\resizebox{0.49\textwidth}{!}{%
				\begin{tabular}{c|c|c|c}  
					\hline 	\hline   \rule{0pt}{10pt}
					\multirow{2}{*}{Protocol}&\multicolumn{2}{c|}{Per-block Com. Compl.}&\multicolumn{1}{c}{Normalized average latency}\cr
					\cline{2-3}  \rule{0pt}{10pt}
					& Optim. &Worst& considering fastlane latency as 1\cr  
					
					\hline  \xrowht{8pt}
					PBFT \cite{pbft}  &$\mathcal{O}(nB)$&$\infty$&  $1/\alpha$ \cr
					%$\mathcal{O}(n^2)$$\infty$ \cr
					\hline \rule{0pt}{8pt}
					HotStuff \cite{hotstuff} &$\mathcal{O}(nB)$&$\infty$&$1/\alpha$ \cr
					\hline \rule{0pt}{8pt}
					HBBFT \cite{honeybadger} &$\mathcal{O}(nB)$&$\mathcal{O}(nB)$&  $C$ \cr
					%$\mathcal{O}(n^3)$$\mathcal{O}(n^3)$ \cr
					\hline \rule{0pt}{8pt}
					Dumbo \cite{guo2020dumbo} &$\mathcal{O}(nB)$&$\mathcal{O}(nB)$& $c$ \cr
					\hline \xrowht{9pt}
					%	CKPS01 \cite{cachin01} &$\mathcal{O}(n^3B)$&$\mathcal{O}(n^3B)$&$\mathcal{O}(n^2)$$\mathcal{O}(n^2)$ \cr
					%\hline \rule{0pt}{10pt}
					KS02 \cite{kursawe05}&$\mathcal{O}(n^2B)$&$\mathcal{O}(n^3B)$& $(\alpha+\frac{\beta}{C+kc})^{-1}$  $^\star$\cr
					%$1/(a+\frac{1-a}{\kappa C})$ \cr
					\hline \xrowht{9pt}
					RC05 \cite{cachin05} &$\mathcal{O}(nB)$&$\mathcal{O}(n^3B)$& $(\alpha+\frac{\beta}{C+c})^{-1}$\cr
					%$1/(a+\frac{1-a}{2 C})$  \cr
					
					%$\frac{t_1}{6}+\frac{t_2}{12}$ \cr
					\hline \xrowht{9pt}
					%\multirow{2}{*}{Hybrid}&\multirow{2}{*}{Yes}&\multirow{2}{*}{$\mathcal{O}(n)$}&\multirow{2}{*}{$\mathcal{O}(n)$}&\multirow{2}{*}{$\mathcal{O}(1)$\multirow{2}{*}}&$\mathcal{O}(n^2)$ \cr
					%\cline{6-6}  
					%& &&&&$\mathcal{O}(n)$\cr  		
					BDT  (ours) &$\mathcal{O}(nB)$&$\mathcal{O}(nB)$& $(\alpha+\frac{\beta}{c+1})^{-1}$\cr				
					\hline  \hline
				\end{tabular}  
			}
		\end{footnotesize}
	\end{center}
	{
		\footnotesize		
		$^\star$ There is an integer parameter $k$ in \cite{kursawe05} to specify the degree of parallelism for the fastlane, thus probably incurring extra cost of fallback.
	}
	
\end{table} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




Here we also summarize the communication complexities of $\mathsf{BDT}$ and some known BFT protocols in the optimistic case and the worst case, respectively.
%
To quantify   the latency of those protocols in unstable network environment, 
Table \ref{tab:performance_comparison} also  lists each protocol's (normalized) average latency. 
This metric considers that the fastlane   has a probability $\alpha\in [0,1]$ to output blocks in time, 
and also has a chance of $\beta = 1-\alpha$ that  falls back and then executes the pessimistic asynchronous protocol. 
%To denote the latency of asynchronous protocols,
Let  $C$ be the latency of using earlier asynchronous protocols \cite{cachin01,honeybadger} directly as the pessimistic path
and $c$ be that of the state-of-the-art  Dumbo BFT \cite{guo2020dumbo} and that of using MVBA  for  synchronization during fallback.
Both $C$ and $c$ are  represented in the unit of  fastlane latency. According to the experimental data \cite{honeybadger,guo2020dumbo}, $C$ is normally at hundreds and the latter $c$ is typically dozens (\cite{honeybadger} runs $n$ instances of $\ABA$, thus rounds depend on number of parties, while \cite{guo2020dumbo} reduces it to constant).   %(since they are way faster by invoking MVBA with small inputs).
Our fallback  is almost as fast as the fastlane, so it is one.
%
We can do a simple calculation as in Table  \ref{tab:performance_comparison} to make a {\em rough estimation} for the (relative) latency of all those protocols deployed in the realistic fluctuating network. 

##############################################################################################################
##############################################################################################################
##############################################################################################################
##############################################################################################################
}








==> CCS 22 long-version/background.tex <==
%!TEX root = main.tex

\section{Introduction}
\label{sec:intro}

%Distributed fault-tolerant protocols (in particular, atomic broadcasts) are promising to realize highly available web services, and often serve as the core components of mission-critical systems such as banking and e-commercing in the real world. 
%Nevertheless, the traditional point of view \cite{Kafka, Chubby} mainly focuses on designing such protocols to fit a relatively friendly in-house deployment environment. 
%For example, Google Chubby and Apache Kafka are used for a tight and small group of local-area network parties to tolerate crash faults. 
%So these protocols essentially only capture some rather limited scenarios where the adversary is too weak to fully corrupt any party or the network.

%The recent explosive success of blockchain technology \cite{bitcoin, buterin2014next, ethereum} not only delivers fantastic  cryptocurrencies  to the community,
%but dramatically 
%the unprecedentedly urgent demand of decentralization
%reprograms our mind to adapt the decentralization
%Byzantine fault-tolerant state machine replications (BFT SMR) over the global Internet.

The explosive popularity of decentralization \cite{bitcoin, buterin2014next}   
creates an unprecedented demand of deploying robust Byzantine fault tolerant (BFT) consensus on the global Internet.  
These consensus protocols were conventionally abstracted as BFT atomic broadcast ($\mathsf{ABC}$) to replicate an ever-growing linearized log of transactions
among $n$ parties \cite{cachin2017blockchain}.
Informally, $\mathsf{ABC}$ ensures {\em Safety} and {\em Liveness}   despite  that an adversary controls the communication network (e.g.,  delay messages) and corrupt some participating parties (e.g., $n/3$).  Safety ensures all honest parties to eventually  output the same log of transactions, and liveness guarantees that any transaction inputted by some honest party eventually appears in honest parties' logs.

%and . 
%  $\mathsf{ABC}$    can attain  the following indispensable securities: 
%(i) {\em Safety}, i.e., the honest parties can  output the same linearly-ordered log of transactions;
%(ii) {\em Liveness}, i.e., any transaction inputted by some honest party can  appear in each honest party's output log eventually. 
%Sometimes, one might require liveness to also capture efficiency that the transactions shall  output reasonably quickly \cite{cachin01,ittai19,pass2017sleepy}, e.g., in a polynomial amount of rounds.%\footnote{It can even be necessary to require output  within a polynomial number of rounds (in the security/system parameters), if using computationally-secure cryptographic primitives such as digital signature and hash function.}


\ignore{
\begin{itemize}
	\item {\em Safety}.  The honest parties can  output the same linearly-ordered log of transactions;
	\item {\em Liveness}. Any transaction inputted by some honest party can  appear in each honest party's output log eventually; sometimes, one might consider a higher efficient liveness that the transactions shall  output reasonably quickly \cite{cachin01,ittai19,pass2017sleepy}, e.g., in a polynomial amount of rounds.\footnote{It can even be necessary to require output  within a polynomial number of rounds (in the security/system parameters), if using computationally-secure cryptographic primitives such as digital signature and hash function.}
\end{itemize}
}



%
\medskip
\noindent
{\bf A desideratum for robust BFT in the absence of   synchrony}. The dynamic nature of   Internet poses new fundamental challenges for implementing  secure yet still highly efficient BFT consensus protocols. 
%
Traditionally, most practical BFT   protocols   were studied for the in-house scenarios where participating parties are geographically close and well connected. 
Unsurprisingly, their securities rely on some form of assumptions about the network conditions. For example,  classic synchrony assumption needs all messages to deliver within a known delay, and its weaker variant called partial synchrony \cite{partialsync} (a.k.a. eventual synchrony) 
assumes that after an unknown global stabilization time (GST), all messages can be delivered synchronously.
%
%For example,
%a class of synchronous protocols (e.g., Sync-HotStuff and Sync-Streamlet) rely on a known bound of network delay (i.e., network synchrony) for both safety and liveness;
%and another category of partial-synchronous protocols (including the classic PBFT \cite{pbft} and many recent progresses such as HotStuff \cite{yin2018hotstuff-full} and Streamlet)
%rely on partial synchrony \cite{partialsync} (a.k.a. eventual synchrony) that the network can eventually become synchronous to deliver all messages within a known delay.
%the synchrony assumption that all messages will be delivered within a known time, or the weaker variant called 
%This is because they were mainly studied for stable in-house scenarios where the participating parties are geographically close and well connected, e.g., by local-area networks (LANs). 
%
%\footnote{Remark that in the BFT problem, safety can somehow be considered as a nickname of agreement (and validity), while liveness can somehow be considered as an alias of termination.}
%
Unfortunately, these    synchrony assumptions may not always hold in the wide-area network (WAN), because of fluctuating bandwidth, unreliable links, substantial delays, and even network attacks.
What's worse, in an   asynchronous network \cite{attiya2004distributed},
such (partially)  synchronous protocols \cite{pbft,tendermint,chan2020streamlet,sbft,bft-smart,thunderella,amir2010prime,700,700aublin,veronese2009spin,aublin2013rbft} will grind to a halt (i.e., suffers from the inherent {\em loss of liveness} \cite{FLP85,honeybadger}), and Bitcoin might even have a {\em safety} issue of potential double-spending \cite{saad2021revisiting} when the adversary can arbitrarily schedule message deliveries.
That said, when the network is adversarial,  
relying on synchrony could lead to fatal vulnerabilities.% such as {\em denial-of-service}!
 
It becomes a {\em sine qua non}  to consider robust BFT consensus that can thrive in   the unstable or even adversarial Internet  for mission-critical applications (e.g.,  financial  services or cyber-physical systems).
Noticeably, the class of fully asynchronous protocols  \cite{cachin01,honeybadger,beat,guo2020dumbo,yang2021dispersedledger}  can ensure safety and liveness simultaneously without any form of network synchrony, and thus become the  arguably most  robust candidates for implementing mission-critical applications.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\begin{table}[]
		\centering
		\caption{Securities of the (partial) synchronous and asynchronous protocols in the asynchronous network, i.e., when the network is the adversary}
		\label{tab:securities}	
	\resizebox{0.5\textwidth}{!}{%
		\begin{tabular}{r|l|c|c}
			\hline\hline
			\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}r@{}}Assumption\\about Network\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Exemplary \\ Protocols\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Securities\\ in async. network\end{tabular}}} \\ \cline{3-4} \rule{0pt}{10pt}
			&                                                                                          & \textbf{Safety}                                  & \textbf{Liveness}                                 \\ \hline\rule{0pt}{10pt}
			{\em Synchrony}                                                                               & \begin{tabular}[c]{@{}l@{}}Sync-HotStuff \cite{sync-hotstuff}, Sync-Streamlet \cite{chan2020streamlet}\end{tabular}                  & X                                                & X                                                 \\ \hline\rule{0pt}{14pt}
			\begin{tabular}[c]{@{}r@{}}{\em Partial-Synchrony}\\ \end{tabular}   & \begin{tabular}[c]{@{}l@{}}PBFT \cite{pbft}, Prime \cite{amir2010prime}, SPIN \cite{veronese2009spin}, RBFT \cite{aublin2013rbft},\\ HotStuff \cite{hotstuff}, Streamlet \cite{chan2020streamlet}\end{tabular}       & $\checkmark$                                                 & X                                     \\ \hline \rule{0pt}{15pt}
			{\em Asynchrony}                                                                             & \begin{tabular}[c]{@{}l@{}}HoneyBadger, BEAT\\ Dumbo, VABA, {\bf This Work}\end{tabular}      & $\checkmark$                                     & $\checkmark$                                      \\ \hline\hline
		\end{tabular}
	}
\end{table}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%
%Moreover, the opt-out of synchrony assumptions brings an additional benefit called {\em responsiveness}, that means an even stronger liveness to ensure the average latency of transactions only depends on
%the actual network delay.
%when actually building the system, asynchronous protocols do not require the engineers to manually tune the time-out mechanism, which is often frustrating and error-prone.

%Following that, the fully asynchronous BFT atomic broadcast becomes the arguably most robust candidatemission-critical replicated services deployed over the    unstable global  network.



%Following that, a \cite{sync-hotstuff, hotstuff, tendermint, pala, libra, honeybadger, beat, thunderella}.
%Following that, 
%the minds of academia and industry are profoundly opened to re-think the BFT problem, which was mainly studied in the last decades for benign scenarios, in the more adversarial global Internet environment \cite{sync-hotstuff, hotstuff, tendermint, pala, libra, honeybadger, beat, thunderella}.
%In particular, it is calling for the critical infrastructure of consortium blockchain (a.k.a., permissioned blockchain) \cite{libra, hyperledger}. 
%Essentially, the consortium blockchain is a fault-tolerant atomic broadcast protocol running among many mutually distrustful Internet parties. 
%The wide-area Internet setting fundamentally challenges the historical  tradition of using fault-tolerant protocols in benign in-house environment,  (e.g., Kafka and Chubby) are rendered into ineffectiveness, as their weak security notion cannot capture arbitrary Byzantine failures, let alone the highly unstable Internet environment. 
%Nevertheless, it is fundamentally challenging to design BFT protocols to fit the unstable global Internet, as 




%To ,   \cite{sync-hotstuff, hotstuff, tendermint, pala, libra, honeybadger, beat, thunderella}

%\subsection{Background and related work}

%As such, our goal is to develop an atomic broadcast protocol for building highly robust and performing consortium blockchain in the environment of unstable Internet.


%\noindent
%{\bf Breaking safety and/or liveness when synchrony fails!}


%That said, for  the   deterministic (partially) synchronous BFT,
%although tuning  the timeout parameter larger can make   the eventual synchrony assumption to hold almost certainly  in    unstable wide-area networks and   thus    promise more  robust liveness \cite{pbft,castro2002practical,naor2019cogsworth,bravo2020making,dolev1983authenticated},
%it unfortunately makes these protocols ``less responsive'' and  causes potential performance deterioration {under the influence of failures and/or attacks}  \cite{amir2008byzantine,veronese2009spin,clement2009making},   resulting in an inherent  {liveness-responsiveness dilemma}.% lying in 

%the  deterministic    protocols running over the   open Internet.
%of performance degradation attacks even more serious and result in greatly harmed latency and throughput.
% that the     latency and throughput could be greatly harmed \cite{attacks},
%.
%
%
%For example, \yuan{pbft example} \cite{pbft}.
%
%A few recent studies \cite{pass2017hybrid,thunderella} a larger

%As such, if we aim to establish a mission-critical replicated web service via BFT protocols over  probably adversarial global network, it is desirable to  get rid of the skeptical timing assumptions for realize the high-assurance of liveness without.


%\subsection{Establishing consortium blockchain from asynchronous BFT}
\medskip
\noindent
{\bf Fully asynchronous BFT? Robustness with a high price!}
%Due to the considerably harmful timing assumptions, realistic worries are raised partially-synchronous BFT protocols .
%Especially when messages can be arbitrarily delayed due to network asynchrony,
Nevertheless, the higher security assurance of asynchronous BFT consensus does not come for free: the seminal FLP ``impossibility'' \cite{FLP85}  states that no {\em deterministic} protocol can ensure both safety and liveness in an asynchronous network.
So    asynchronous $\mathsf{ABC}$   must run {\em randomized} subroutines to circumvent the ``impossibility'', which already hints its complexity. 
%
%In contrast to  the deterministic partially-synchronous or synchronous   protocols, 
%randomized    protocols can achieve fully asynchronous BFT that  would ensure liveness and responsiveness without any form of timing assumptions. 
%
%In particular, the transactions at the top of each party's backlog (a.k.a. transaction pool or transaction buffer) would always   output in some  polynomial  asynchronous rounds, which is  only related to the actual network delay $\delta$ instead of the %timeout parameter $\tau$ or the 
 % delay upper bound $\Delta$,
%\footnote{Note that  an asynchronous BFT protocol is said optimal resilience if it can tolerate $f=\lfloor (n-1)/3 \rfloor$ Byzantine faulty parties, and we will focus on optimally-resilient asynchronous  protocols through the paper.}
%
%thus realizing robust liveness  and high responsiveness simultaneously. 
%Also the  asynchronous  protocols  remove  the necessity of  complicated manual timeout policies and save    practitioners' life. 
%
%It follows that  the
%asynchronous  BFT protocols  become   arguably the most robust candidates  for mission-critical replicated services deployed over the    unstable global  network.
%
%
%allow a system  of $n$ parties to tolerate at most $f$ arbitrary Byzantine faults
%
%
%The cost of   randomization could be large or even prohibitive.
%Prior to some very recent breakthroughs \cite{honeybadger,dumbo,beat}, 
Indeed, few   asynchronous   protocols have been   deployed in practice during the past decades due to large complexities, 
until the recent  $\mathsf{HoneyBadgerBFT}$  \cite{honeybadger} and  $\dumbo$ protocols \cite{guo2020dumbo} (and very recent their improved variants \cite{yang2021dispersedledger,guo2022speeding}) provide novel paths to {\em practical} asynchronous ABC in terms of realizing optimal linear communication cost per output transaction. %(through   the batching technique that trades off latency). 
%(via a huge batch of transactions per block and trading off latency).

%For example, an earlier construction  of asynchronous atomic broadcast is from an sub-optimal  multi-value validated asynchronous Byzantine agreement (MVBA)  \cite{cachin01} and incurs  huge $\bigO(n^3)$ communicated bits for each output transaction.
%
%Such the breakthrough delivers us the first communication-optimal asynchronous atomic broadcast, 
%and more importantly, hints a brand new path toward practical asynchronous atomic broadcast protocols. 



Despite those  recent progresses, %on practical asynchronous BFT, %designs are (amortized) communication-optimal as well as  robust  and responsive, 
the actual performance of state-of-the-art randomized asynchronous consensus  is still far worse than the  deterministic (partial) synchronous ones (e.g., $\mathsf{HotStuff}$  \cite{yin2018hotstuff-full}\footnote{Remark that \cite{yin2018hotstuff-full} gave  a 3-chain $\mathsf{HotStuff}$ protocol along with a 2-chain variant. Throughout the paper, we let $\mathsf{HotStuff}$ refer to the 2-chain version (with minor difference to fix the view-change issue) for the lower latency of the 2-chain version.}), especially regarding the critical latency metric. 
%As shown in Fig. \ref{fig:async-vs-sync}, 
For example, in the same WAN deployment environments consisting of $n$=16, 64, 100 Amazon  EC2 instances across the globe,
$\mathsf{HotStuff}$ is dozens of times faster than the state of the art $\dumbo$ protocol \cite{guo2020dumbo}. 
%(and still a few times faster than a later improved version Speeding Dumbo \cite{speedingdumbo}). % and about an order-of-magnitude faster than its recent speedy variant \cite{guo2022speeding}.
Even worse,
the inferior latency performance of  asynchronous protocols 
 stems from the fact that all parties  generate some common randomness (e.g.,  ``common coin'' \cite{canetti1993fast,cachin00}),
% to clip the power of adversarial asynchronous network, 
and multiple repetitions are necessary to ensure the parties to coincidentally output with an overwhelming probability.
%As a result, a dozen of   rounds on average are   needed, 
Even if in one of the fastest existing asynchronous protocols such as $\dumbo$ \cite{guo2020dumbo} and its improved version $\mathsf{Speeding}$-$\dumbo$ \cite{guo2022speeding}, they still cost about a dozen of   rounds  on average.
While for their (partial) synchronous counterparts,
only a very small number of rounds are required in the optimistic cases when the underlying  communication network is   luckily synchronous \cite{abraham2021good}, e.g., 5 in the two-chain $\mathsf{HotStuff}$ and 3 in PBFT. 

\ignore{%%%%%
\footnote{One might   suggest to choose a conservative timeout parameter to make (partially) synchronous BFT survive in the adversarial network. Besides that they cannot be secure in asynchronous network, it might also bring serious performance degradation in latency, e.g., the exaggeratedly slow   Bitcoin.
	% because the latency of (partially) synchronous protocols  inherently depends on this delay bound due to the classic Dolev-Strong result \cite{dolev1983authenticated}. 
	%e.g., slow block generations in Bitcoin and slow   view-changes in PBFT and HotStuff, which can be understood as the result of lacking the critical responsiveness property to make the   latency only depend  on the actual network delay instead of the exaggerated delay upper bound. %Worse still, though a few recent nice results \cite{shrestha2020optimality,thunderella,sync-hotstuff} make synchronous protocols to attain fast confirmation in the absence of faulty leaders, they still suffer from inherent slow confirmation in the general cases with corruptions.
	Actually, a large number of ``robust'' (partially) synchronous protocols such as Prime \cite{amir2010prime}, SPIN \cite{veronese2009spin} and RBFT \cite{aublin2013rbft}   are still  subject to this robustness-latency trade-off, let alone their main motivation is to mitigate the impact of corrupted parties instead of lifting robustness against adversarial network. %Because although larger timeout parameters might cause synchrony assumption to hold with a higher probability, they also result in slower confirmation in the absence of adversary (due to the classic Dolev-Strong result \cite{dolev1983authenticated}). %because the adversary-influencing latency of them  inherently depends on the  upper bound due to the classic Dolev-Strong result \cite{dolev1983authenticated}. %Let alone, none of them can guarantee liveness in an asynchronous network.
	%resolve the {\em denial-of-service} threat when the adversary might compromise the network.
}
}%%%%%%

%(e.g., all parties are closed to the Internet backbone).  %%%%%%%%%%%%%\yuan{insert a comparison figure}
%Indeed, as argued in \cite{honeybadger}, the asynchronous  protocols were believed to suit the scenarios where throughput is more favorable over latency. 
%as the common coin subroutine

%\smallskip
The above issues correspond to a fundamental ``dilemma'' lying in the  design space of BFT consensus protocols suitable for the open Internet: the cutting-edge (partially) synchronous deterministic protocols can optimistically work very fast,  but lack  liveness guarantee in adversarial networks;
on the contrary, the fully asynchronous randomized protocols  are robust even in malicious networks, but  suffer from poor latency performance in the normal case. 
Facing that, a natural question arises:  

\begin{center}
	{\em Can we    design a BFT consensus  achieving  the best of both synchronous and asynchronous paradigms, such that it (i)  is   ``as fast as'' the state-of-the-art    deterministic  BFT consensus on the normal Internet with fluctuations and (ii)    performs nearly same to the existing performant    asynchronous BFT consensus  even if in a worst-case asynchronous network?
		%such that it is ``as fast as'' the state-of-the-art deterministic protocols in the real-world networks? Additionally, can we , such that it can perform same to the currently most efficient asynchronous protocols in the worst-case?
	}
\end{center}
 
% since their multiple round executions are quintessential to ensure the overwhelming probability of termination despite any adversarial network.  
%One might argue that the performance bottlenecks of asynchronous atomic broadcasts \cite{cachin01, honeybadger} are probably the ``prices'' of robust liveness against the extremely hostile asynchronous network to go through FLP's impossible results. 
%Especially when the Internet condition is moderately unpredictable instead of being fully adversarial, 
%these performance bottlenecks cause asynchronous protocols \cite{cachin01, honeybadger} far lagging behind 
%many popular partial-synchronous protocols \cite{pbft, hotstuff, pala, tendermint} in terms of concrete performance.
%
%\footnote{The recent partial-synchronous protocol HotStuff reported that its peak performance could be doubled than PBFT, while HBBFT \cite{honeybadger} merely realized a peak performance closed to PBFT.}
%
%
%Even worse,   the performance bottlenecks in these randomized asynchronous protocols are seemingly inherent, since their probabilities of termination are closing to one with continuing executions, they usually on average , while in some benign cases.  
%This leaves us the following unanswered question:




==> CCS 22 long-version/conclusion.tex <==
%!TEX root=main.tex

\section{Conclusion}

==> CCS 22 long-version/contribution.tex <==
%!TEX root = main.tex
%\medskip
\subsection{Our contributions}
%: breaking the bottleneck for best of both}

%\medskip
%\noindent
%{\bf Effectivenesses of our results}. %In short, our immediate result is 
We answer  the aforementioned question affirmatively, by presenting the first {\em practical} and {\em generic} framework for   optimistic  asynchronous  atomic broadcast  called $\sys$ (or $\BDT$ for short). Here, optimistic  asynchronous  atomic broadcast \cite{kursawe05,cachin05,gelashvili2021jolteon} refers to an asynchronous consensus that has a deterministic fastlane that might luckily progress in the benign network environment (optimistic case) without randomized execution.
%and was proposed by Kursawe-Shoup \cite{kursawe05} (KS02)  and a later improvement of Ramasamy-Cachin \cite{cachin05} (RC05).

\begin{figure}[h] 
	%\captionsetup{font={normalsize}}
	\vspace{-0.2cm}
	\begin{center}
		\includegraphics[width=8.3cm]{fig/framework.pdf}
		\vspace{-0.2cm}
		\caption{The overview of $\sys$.}	\label{fig:BDT}
		%\caption{The overview of our new practical and generic optimistic atomic broadcast framework, nicknamed by $\sys$.}	\label{fig:BDT}
	\end{center}
	\vspace{-0.3cm}
\end{figure}

%Here, an  optimistic  asynchronous  atomic broadcast protocol  is  .

At a very high-level, $\BDT$   has three phases as shown in Fig. \ref{fig:BDT}:
\begin{itemize}[leftmargin=0.7cm]
	\item {\em Fastlane} (nickname $\mathsf{Bolt}$): It initially runs a deterministic protocol as  fastlane to quickly progress in the optimistic case that synchrony assumption holds.
	\item {\em Pace-synchronization} (called pace-sync for short or nickname $\trans$): If the fastlane fails to progress in time, a  fast {pace-synchronization} mechanism (analog to view-change with asynchronous securities)  is triggered to make all honest parties agree on from where and how to restart (directly restart $\Bolt$ or enter pessimistic path).
%	The pace-sync  of $\BDT$ is  simple and  conceptually minimum, in the sense of only requiring  one single binary   agreement.
%	Actually, the binary-agreement enabled $\trans$   is the crux of making $\BDT$ practical, as it overcomes the main efficiency obstacle lying in previous multi-valued agreement based designs \cite{kursawe05,cachin05} (to be explained in details in Section \ref{sec:prior}).
	\item {\em Pessimistic path} (nickname $\Dumbo$ \footnote{Here we call the pessimistic path $\Dumbo$ and call the concrete ABC protocol in \cite{guo2020dumbo} Dumbo-BFT. The latter could be an instantiation for the former (as in our experiments), but other better ABC protocol could also instantiate the former pessimistic path.}): In case the fastlane was completely failed to make progress, the honest parties enter a {pessimistic path} of asynchronous BFT to ensure liveness even in the worst case. 
	%In $\BDT$, the pessimistic path can be instantiated by any state-of-the-art asynchronous BFT consensus, and  thus inherit the benefits of all recent progresses. 
	%While, if the pace-synchronization reveals that the fastlane still can output something (e.g. one block), 
	%the pessimistic path is   skipped, and all honest parties directly retry the fastlane.
\end{itemize}




  









 

%\smallskip
%\noindent
%{\bf Summary of results}.  
{$\BDT$ is featured with guaranteed {\em liveness} and safety even in a hostile asynchronous network} with optimal tolerance against $n/3$ byzantine parties.
More importantly, as depicted in Fig. \ref{fig:changing-net}, it indeed realizes the best of its both paths, i.e., it is as fast as deterministic protocols (such as the state-of-the-art pipeline BFT protocols, e.g.,   2-chain   $\mathsf{HotStuff}$) in ``good'' synchronous periods; and also as robust as asynchronous protocols in the ``bad'' network. %Specifically:

\ignore{%%%%%%
\begin{itemize}
	%\item $\BDT$ with optimal tolerance against $n/3$  Byzantine corruptions;
	%\item In the optimistic case, 
	\item In the normal cases where  the network is mostly synchronous  and only encounters short-term network fluctuations,
	% (i.e., the network is {\em not} always the adversary),
	$\BDT$ can be as fast as the state-of-the-art pipeline BFT protocols (e.g.,   2-chain   $\mathsf{HotStuff}$) and   performs much faster than existing asynchronous   protocols.
	\item In the worse cases where    long-lasting   asynchronous periods exist, $\BDT$ can   perform as robustly as the underlying asynchronous protocol to closely track the actual network bandwidth and delay, despite the synchronous protocols might suffer from denial-of-service in the environment.
\end{itemize}
}%%%%%



\begin{figure}[h] 
	\vspace{-0.2cm}
	%\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=8cm]{fig/changing-network.pdf}\\
		\vspace{-0.3cm}
		\caption{Simulated executions of $\mathsf{BDT}$, 2-chain $\mathsf{HotStuff}$ and $\dumbo$-{\sf BFT} under fluctuating network ($n$=64). Bad network happens twice: one lasts 2 seconds and one lasts 120 seconds. See Section \ref{evaluation} for the details on simulation setup.}	\label{fig:changing-net}
		%\caption{The overview of our new practical and generic optimistic atomic broadcast framework, nicknamed by $\sys$.}	\label{fig:BDT}
	\end{center}
	\vspace{-0.3cm}
\end{figure}


\smallskip
\noindent
{\bf Technical overview}.
Different from pioneering studies  \cite{kursawe05,cachin05,700,700aublin} that only demonstrated theoretic feasibility and had questionable practicability because of complex and slow {\em asynchronous} pace-synchronization (cf. Section \ref{sec:prior} for detailed discussions on their efficiency bottleneck),
$\BDT$ makes  several technical contributions   to harvest the best of both paths in practice. In greater detail,

%\vspace{-0.1cm}

%To construct the \BDT\/ framework achieving the best of both fastlane and pessimistic path, we 
%stress on the next immediate  improvements for concrete efficiency as clarified in Fig. \ref{fig:BDT}:

%\begin{itemize}
	%\item 
	\smallskip
		\noindent\underline{\smash{\em A new fastlane abstraction \rev{better prepared for failures}}}.
%
%At the core of   $\BDT$ framework, 
\rev{
To simplify the   complicated pace-sync, % to simpler binary agreement,
we propose a new fastlane abstraction of notarizable weak atomic broadcast ($\mathsf{nw\textnormal{-}ABC}$ for short)
to prepare    honest parties in a graceful condition  when facing potential fastlane failures.} 
Notably, $\mathsf{nw\textnormal{-}ABC}$ realizes $\mathsf{ABC}$   in the optimistic case, and only ensures ``notarizability'' otherwise:  any output block is with a quorum proof to  attest that sufficient honest parties have  received a previous block (along with valid  proof). Such an $\mathsf{nw\textnormal{-}ABC}$ can be easily constructed to be very fast, e.g.,   from a sequence of simple (provable) multicasts;
%
and more importantly, the notarizability (as we will carefully analyze) guarantees that any two honest parties will be at neighboring blocks when entering pace-sync, \rev{thus enables us to leverage simpler binary agreement to replace the cumbersome full-fledged asynchronous atomic broadcast or  multi-value agreement  used in prior art \cite{700aublin,700,kursawe05,cachin05}. }
%In addition, such a fastlane can still be   easily and efficiently implemented, } 

\medskip
	\noindent\underline{\smash{\em  Cheapest possible pace-synchronization}}. More importantly, with the preparation of $\mathsf{nw\textnormal{-}ABC}$, %With the help of our new abstraction of fastlane (to be explained soon), 
	$\Trans$
	%At the core of  $\mathsf{BDT}$, it is a much more efficient pace synchronization mechanism,  \Trans\/, to allow secure and practical fallback when the fastlane fails to make in-time progress. 
 reduces pace-sync to a problem that we call {\em two-consecutive-valued Byzantine agreement} ($\tcvba$), which is essentially an  asynchronous {\em binary} Byzantine agreement ($\ABA$). In contrast, prior art  \cite{kursawe05,cachin05} leveraged cumbersome multi-valued agreement ($\mathsf{MVBA}$) for pace-sync (cf. Sec. \ref{sec:prior} for a careful review).  %and is dozens of times faster than the underlying pessimistic path.
	%
	%The new $\tcvba$ requires a special validity that: 
	%if the honest parties input one of two consecutive integers, the common output shall be one of the honest input values.
	%
	%We also give very simple constructions of $\tcvba$ from any asynchronous {\em binary} agreement.
	%We  give a very simple construction for this concrete module by only replacing  three  lines of the pseudocode of the binary agreement in \cite{guo2020dumbo}. 	
	  $\Trans$ thus improves the communication complexity of pace-sync   by an $\bigO(n)$ factor, and is essentially optimal for  pace-sync, because the pace-sync problem can be viewed as a version of asynchronous consensus, and $\ABA$ is the arguably simplest asynchronous consensus. %Such improvement becomes the crux to, cf. Fig. \ref{fig:bottleneck} (c).
 In practice, $\Trans$  attains a minimal overhead   similar to the fastlane latency. Further care is needed for invoking $\mathsf{nw\textnormal{-}ABC}$ to ensure the safety (see next section).

	%\item 

%Therefore, all honest parties would either vote for $s$ or vote for $s-1$ in pace-sync (where $s$ represents the index of latest fastlane output with valid quorum proof).
%Clearly, we only have  to solve a binary agreement problem:   from $s$  to fallback or from $s-1$ to fallback. 
%This avoids the use of complicated asynchronous multi-valued byzantine agreement.
%
%Together with the recent progress of asynchronous consensus  (e.g., $\Dumbo$ or its optimized variants) as the pessimistic path, $\BDT$   can be instantiated to realize the following merits, cf. Fig \ref{fig:BDT}. %Specifically, %it realizes the following immediate   efficiency improvements:
%Moreover, the fastlane abstraction is generic and can be instantiated by   running sequential reliable broadcasts or pipelined multicasts.

\medskip
	%\item 
\noindent\underline{\smash{\em Avoiding pessimistic path whenever we can}}. To further exploit  the benefits brought by   fast $\Trans$, we add a simple check after pace-sync to create two-level fallbacks: 
	if pace-sync reveals that  the fastlane still made some output, it immediately restarts another fastlane  without running the actual pessimistic path.
	%(ii) otherwise, the fastlane completely failed to output nothing, it enters the level-2 fallback to run the pessimistic path.
	%
	%The pessimistic path is tentatively {\em not} executed except when .
	%In other words, we make two levels of fallback: (i) in the level-1, 
	%(ii) in the level-2, 
	% thus have to execute the pessimistic asynchronous protocol to move forward, we let them switch back to the fastlane immediately.
	This is in contrast with previous works \cite{kursawe05,cachin05} where the slow pessimistic path will always   run after each pace-sync, which is often unnecessarily costly if there are only short-term network fluctuations. Remark that the  earlier studies cannot effectively adopt our two-level fallback tactic, because their heavy pace-sync  might   bring extra cost \rev{and it may even nullify the advantages of the fastlane} in case of frequent fallbacks.
	
	%Moreover, we 
	
	%\item 
	\medskip 
	\noindent\underline{\smash{\em Generic framework enabling flexible instantiations}}.	$\mathsf{BDT}$  is generic, as it  enables  flexible choices of the underlying building blocks for all three phases. For example, we present two exemplary fastlane instantiations, resulting in two $\mathsf{BDT}$ implementations that   favor  latency and throughput, respectively, so one can instantiate $\mathsf{BDT}$ according to the actual application scenarios. Also,  $\Trans$ can be constructed around any asynchronous binary agreement, thus having the potential of using any more efficient $\ABA$ to further reduce the fallback overhead  \rev{(e.g., by adopting the  recent progress from Crain \cite{crain2020two}, Das et al. \cite{das2021practical} and Zhang et al. \cite{zhang2022pace})}. Similarly,  though currently we use  $\mathsf{Dumbo}$-BFT as the pessimistic path, this can be   replaced by more efficient recent designs \cite{guo2022speeding}.


%\end{itemize}





%\begin{table}[htp]
%	\vspace{-0.2cm}
%	\caption{List of components and nicknames in   $\mathsf{BDT}$}\label{tab:nickname}
%	\vspace{-0.4cm}
%	\resizebox{0.485\textwidth}{!}{%
%		\begin{tabular}{r|c|c|l}
%			\hline\hline\rule{0pt}{10pt}
%			& \textbf{Core Component}                                          & \textbf{Nickname} & \textbf{Instantiations}                                                                                       \\ \hline\rule{0pt}{16pt}
%			\textbf{\begin{tabular}[c]{@{}r@{}}Optimistic\\ Fastlane\end{tabular}} & $\mathsf{nw\textnormal{-}ABC}$                                                           & $\mathsf{Bolt}$              & \begin{tabular}[c]{@{}l@{}}$\mathsf{Bolt\textnormal{-}sRBC}$ or $\mathsf{Bolt\textnormal{-}sCAST}$\\ (cf. Section III.A)\end{tabular}                             \\ \hline\rule{0pt}{23pt}
%			\textbf{Pace-Sync}                                                     & $\mathsf{tcv\textnormal{-}BA}$                                                           & $\mathsf{Transformer}$       & \begin{tabular}[c]{@{}l@{}}From any $\mathsf{ABBA}$  or\\ slightly adapt $\mathsf{ABBA}$ in \cite{MMR15}\\ (cf. Section III.B)\end{tabular}       \\ \hline\rule{0pt}{23pt}
%			\textbf{\begin{tabular}[c]{@{}r@{}}Pessimistic\\ Path\end{tabular}}    & \begin{tabular}[c]{@{}c@{}}asynchronous\\ consensus\end{tabular} & $\dumbo$             & \begin{tabular}[c]{@{}l@{}}$\mathsf{ACS}$ from $\dumbo$ \cite{guo2020dumbo} or\\ any multi-value consensus\\  (e.g., $\mathsf{MVBA}$ \cite{cachin01,lu2020dumbo,ittai19})\end{tabular} \\ \hline\hline
%		\end{tabular}
%	}
%	\vspace{-0.2cm}
%\end{table}








%As briefly mentioned, our novel fastlane is centered around a new  broadcast primitive called notarized weak atomic broadcast ($\mathsf{nw\textnormal{-}ABC}$), and we let $\tobc$ to be its nickname;
%Our novel pace-sync  mechanism is nicknamed by $\trans$, at the core of which is a variant of binary agreement called two-consecutive-value Byzantine agreement ($\tcvba$); For the pessimistic path, it can be reduced to any asynchronous consensus, and we nickname it by $\dumbo$ as instantiating it via the state-of-the-art asynchronous  protocol --- $\dumbo$.



%\subsection{Extensive  evaluations}



 \medskip
\noindent
{\bf Extensive  evaluations}.
To demonstrate the practical performance of $\BDT$,
% that \BDT\/ achieves the best of its both paths in practice,
we  implement the  framework using $\Dumbo$-{\sf BFT} \cite{guo2020dumbo} as the exemplary   pessimistic path. 
%
%Two optimistic paths are implemented, one of which is based on a stable leader version of simplified HotStuff and the other of which is based on causal broadcast by sequentially executing provable reliable broadcast (RBC).
%
We compare   two typical $\BDT$ implementations to   $\dumbo$ and $\mathsf{HotStuff}$, and conduct extensive experiments in   real-world/simulated environments. %to showcase its   practicality. 
%For fair comparison, we implement all protocols in the same language with same cryptographic libraries.
%Extensive  evaluations 







We first deploy all protocols  in the same real-world WAN environment consisting of up to 100 Amazon EC2 c5.large instances     across the globe. 
Some highlighting   experimental results could be found in Table \ref{table:summary}, which are: (i) % the  optimistic path keeps on delivering blocks in time,
the $\BDT$ implementation based on sequential multicasts can  attain a basic latency about only 0.44 second (i.e., nearly same to 2-chain HotStuff's and less than 3\% of $\dumbo$'s latency),
even if we intentionally raise frequent pace synchronizations after every 50 optimistic blocks; % to amplify the average latency;
(ii) in the worst case that we intentionally make fastlane to always fail,
the throughput of $\BDT$ remains 90\% of $\dumbo$ BFT's and is close to 20,000 transaction per second, 
even if we do let $\BDT$ wait as long as 2.5 seconds to timeout before invoking pace-sync.
%
%
%
Those demonstrate  $\BDT$  can be ``as fast as'' the deterministic protocols in normal cases and can  maintain  robust performance in  the worst case.







To understand  more scenarios in-between, we then conduct  evaluations in a controlled test environment that can simulate fluctuating network (i.e., switching between ``good'' and ``bad'' networks).
In the simulated good network   (i.e., 50 ms packet delay and 200 Mbps peer-to-peer link), $\BDT$ is almost as fast as 2-chain HotStuff; while in the simulated bad network (i.e., 300 ms packet delay and 50 Mbps peer-to-peer link), $\BDT$ can closely track  the performance of underlying pessimistic asynchronous protocol, though HotStuff might grind to a halt due to inappropriately chosen timeout parameter.% \rev{We also give direct comparisons using $\BDT$ and in earlier framework }

See Section \ref{evaluation} for  more detailed experiment  setup and   results.


\begin{table}[htp]
	\vspace{-0.15cm}
	%\centering
	\captionsetup{font={normalsize}}
	\caption{$\mathsf{BDT}$, 2-chain $\mathsf{HotStuff}$ and $\dumbo$-{\sf BFT}  running over {\bf 100}   EC2 c5.large servers across {\bf 16} regions in {\bf 5} continents}
	\vspace{-0.45cm}
	\label{tab:experiement-highlight}
	\resizebox{0.495\textwidth}{!}{%
		
		\begin{tabular}{c|c|c|c|c|c}
			
			 \hline\rule{0pt}{18pt} 
			\multirow{2}{*}{}                                                  & \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Good-Case v.s. HotStuff\\ (fastlanes always complete)\end{tabular}}}                   & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Worst-Case  v.s. Dumbo\\ (fastlanes always fail)\end{tabular}}} \\ \cline{2-6} \rule{0pt}{15pt}
			& \begin{tabular}[c]{@{}c@{}}\hspace{-0.15cm}$\mathsf{BDT}$-$\mathsf{sCAST}$$^{**}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\hspace{-0.15cm}$\mathsf{BDT}$-$\mathsf{sRBC}$$^\dagger$\end{tabular} &\hspace{-0.15cm} $\mathsf{HotStuff}$$^\S$ & \begin{tabular}[c]{@{}c@{}}\hspace{-0.15cm}$\mathsf{BDT}$-$\mathsf{Timeout}$$^\ddagger$\end{tabular}                       & \hspace{-0.15cm}$\mathsf{DumboBFT}$                      \\ \hline\rule{0pt}{10pt}
			\hspace{-0.25cm}Basic latency    (sec)      & 0.44                                                     & 0.67                                                      & 0.42     & 21.95                                                                               & 16.36                      \\ \hline\rule{0pt}{10pt}
			\begin{tabular}[c]{@{}c@{}}\hspace{-0.25cm}Throughput   (tx/sec)$^{*}$ \end{tabular} & 9,253                                                     & 18,234                                                     & 10,805    & 18,806                                                                               & 21,242                      \\ \hline 
		\end{tabular}
	}%
	
	{
		\footnotesize
		\begin{itemize}[leftmargin=0.4cm]
			\item[*] Each transaction has 250 bytes to approximate the basic Bitcoin transaction.
			\item[**] $\mathsf{BDT}$-$\mathsf{sCAST}$ is $\mathsf{BDT}$ with using $\mathsf{Bolt}$-$\mathsf{sCAST}$, where $\mathsf{Bolt}$-$\mathsf{sCAST}$ is the   fastlane instantiation built from pipelined multicasts.
			\item[$^\dagger$] $\mathsf{BDT}$-$\mathsf{sRBC}$  is $\mathsf{BDT}$ with using $\mathsf{Bolt}$-$\mathsf{sRBC}$, where $\mathsf{Bolt}$-$\mathsf{sRBC}$ is the   fastlane instantiation built from sequential reliable broadcasts.
			\item[$^\ddagger$]  $\mathsf{BDT}$-Timeout idles for 2.5 sec in the  fastlane,  and then runs Pace-Sync+$\dumbo$.
			\item[$^\S$] Reasons why our evaluations for HotStuff   different from \cite{yin2018hotstuff-full}: (i)  we   tested  among 16 AWS regions instead of   one AWS region; (ii) we let the  implementation  to   agree  on 250-byte tx instead of 32-byte tx hash; (iii)   we use a single-process   network layer written in Python, differing from    multi-processing network layer in \cite{yin2018hotstuff-full}.
		\end{itemize}
	}
	
	
	\label{table:summary}
	\vspace{-0.2cm}
\end{table}


% .

%are presented in Section \ref{evaluation} and   \ref{sec:complex}.


%In particular, the optimistic case is taken place when a fastlane protocol called \Bolt\/ can luckily output, if the network is benign to deliver messages within an estimated network delay $\tau$ \footnote{Remark that $\tau$ in our protocol can be set aggressively using estimated network delay in good days since now liveness is ensured by fallback.} (and the leader in \Bolt\/ is honest). There is also a {pace synchronization} phase, that we call \Trans\/, will be executed if enough honest parties suspect that \Bolt\/ is stuck. If \Trans\/ reveals that   \Bolt\/ completely fails and makes no progress at all, the pessimistic path would be invoked to execute an asynchronous BFT protocol that we call \Dumbo\/, otherwise another \Bolt\/ instance will be executed. More concretely, our technical contribution is fourfold:




%\subsection{Roadmap}
%\yuan{todo...........}
%Sections II and III present the preliminary primitives and the problem definitions, respectively. 
%After that, Section IV introduces the new fastlane formulation notarizable weak atomic broadcast and present two instantiations
%for it. Section V then defines and constructs two-consecutivevalued binary agreement, which is the key ingredient for our
%new fallback mechanism. In Section VI, we construct our
%new generic practical framework Bolt-Dumbo Transformer
%for optimistic asynchronous atomic broadcast and analyze its
%security in details. We then implement the framework and
%demonstrate its high applicabilities by extensive real-world experiments across the globe in Section VII. Complexity analysis
%and numerical estimations are presented in Section VIII to
%further discuss the applicability of Bolt-Dumbo Transformer
%in unstable network environments.




%\noindent
%{\bf Technical overview}. 




\input{hybrid-intro}

%\section{Solution in a Nutshell}



\medskip
\noindent
{\bf Our Solution in a Nutshell}.
%Let us first briefly recall  
%why    MVBA is used for pace synchronization, and poses the main practical hurdle in existing optimistic asynchronous atomic broadcasts?
%If the leader is corrupted or the network is failed as a synchronous network, then the fastlane could fail to progress, in this case, each honest party can wait for a set of $2f+1$ fallback requests sent from distinct parties, and each fallback request (called complaint message in KS02 and RC05)  contains an index $s$ of the latest  fastlane block along with the corresponding quorum ``certificate'' (which usually is a collection of signatures from distinct parties). %proving all broadcasts with indices up to $s$ were indeed delivered.  
%The goal of pace synchronization is to decide a common index contained by some fallback sent from an honest party,
%such that all honest parties can agree to enter the pessimistic path from this position. %and they also can obtain some missing blocks from some honest parties (because some honest one proposed  
%To this end, 
%prior studies utilized Cachin et al.'s MVBA  \cite{cachin01} 
%to pick up a set of $2f+1$ valid fallback requests from distinct parties,
%and the {\em largest} index $s$ among these fallbacks naturally becomes the agreed fastlane position to start fallback. 
%In addition, due to the nice property of   valid quorum ``certificates'', it is guaranteed that enough parties did receive the blocks with indices until $s$,
%so the honest parties can expect to fetch the missing blocks.% all the way to the index $s$. 
%
%\footnote{Ramasamy-Cachin \cite{cachin05} reduced the message complexity asymptotically  using  strong consistent broadcasts weaker than   reliable broadcasts in \cite{kursawe05}, and it also reduced the communicated bits running the first MVBA for agreeing on the fastlane progress by reducing the size of ``certificate'' by a   $n$ factor.}
%In case the fastlane        can activate $k$ broadcasts instances in parallel as in \cite{kursawe05}, it is   possible that some honest party was running ahead and did output in a broadcast instance indexed by $s+k$,
%(where $k$ is a protocol parameter   to specify the degree of parallelism), 
%so the parties  will   execute more MVBA instances through for $s$ until for $s+k$ one-by-one  to sync  all possible  outputs to avoid influencing   safety.
%Since consistent broadcast cannot ensure a strong all honest nodes to eventually receive what another honest node received, after agreeing to synchronise at block $s$ via an MVBA protocol, each node will ask for help from other honest nodes to actually catch up. 
%}
%
%When the above {\em pace-synchronization}   finishes, all parties have to run MVBA again as the fully asynchronous consensus to ensure transactions lying in their transaction buffer to output despite the network adversary, then they can restart the fastlane.
%====
Now we walk through how we overcome the above challenge and reduce the   complex pace-sync  problem to only a variant of asynchronous binary agreement.


	%\vspace{-0.1cm}

	\smallskip
	\noindent \underline{\smash{\em First ingredient: a  new abstraction of the fastlane}}.
	We put forth a new simple  fastlane abstraction called {\em notarizable weak atomic broadcast} (\nwabc, with nickname $\Bolt$). In the optimistic case, it performs as a full-fledged atomic broadcast  protocol and can output  a block per $\tau$ clock ticks. But if the synchrony assumption fails to hold, it won't have liveness nor exact agreement, only a  {\em notarizability} property can be ensured: whenever any party outputs a block at position $j$ with   a valid quorum proof, at least $f+1$ honest parties already output   at the position $j-1$, cf. Fig. \ref{fig:nw-abc}. 
	%This property is critical for preparing \Bolt\/ to pair with a very efficient \Trans\/ that we will introduce next. 
	%
	%Also, \nwabc\/ is easy to obtain from  the popular lock-commit paradigm adopted in many deterministic BFT protocols \cite{pbft,sbft,hotstuff,chan2020streamlet} (and the fastlane in \cite{cachin05}).
	%   since it does share the similar essence of the popular lock-commit paradigm adopted in many deterministic  BFT protocols \cite{pbft,sbft,hotstuff,chan2020streamlet} (and the fastlane in \cite{cachin05}).  
	%grafted to Dumbo BFT as benchmarks to demonstrate its flexibility to cater different real-world demands on varying performance metrics. 
	%
	%It is also easy to implement \nwabc. We present two exemplary constructions.
	%The first one   assigns a stable leader to sequentially multicast its input proposals and other parties simply vote by digital signatures, 
	%and is appropriate for the scenarios that favor latency. 
	%The second one is to let a stable leader sequentially execute reliable broadcasts (using erasure code to reduce the leader's bandwidth usage \cite{cachin2005asynchronous,honeybadger}) and is more friendly for large input proposals, thus achieving a throughput higher than the first instantiation on the global Internet.
	%
	
	%normal synchronous protocol 
	%	In the optimistic case, when messages are delivered within a guessed time parameter $\tau$ and the leader is honest, we may consider directly deploying a (partially) synchronous BFT protocol. 
	


		

	
	
		\smallskip
	\noindent \underline{\smash{\em How ``notarizability'' better prepares   honest parties?}} To see how      notarizability simplifies pace-sync, 
	%
	let us examine the pattern of the honest parties' fastlane outputs before entering pace-sync. %(for simplicity, we only consider the indices of the fastlane blocks). 
	
	
	
	
	Suppose all honest parties have quit the fastlane,
	exchanged their fallback requests (containing their latest block index and the corresponding quorum proof),
	received such $2f+1$ fallback requests, and thus entered the pace synchronization.
	At the time, let $s$ to be the largest index of all fastlane  blocks with valid proofs.  %(which means with a valid quorum certificate as proof for validity). 
	%
	
	We can   make two easy claims: 
	%\begin{enumerate}
	%	\item[(i)] No honest party can see a valid fallback with an index equal or larger than $s+1$;
	%	\item[(ii)] All honest parties must see some fallback with an index equal or larger than $s-1$.
	%\end{enumerate}
	(i) no honest party can see a valid fallback request with an index equal or larger than $s+1$;
	%$s^+\geq s+2$; 
	(ii) all honest parties must see some fallback request with an index equal or larger than $s-1$. %Namely, 
	%
	%$s_{\_}< s-1$, .
	%
	If (i) does not hold, following notarizability, at least one party can produce a proof for block $s+1$, which contradicts the definition of $s$. 
	While for (ii), since block $s$ is with a valid proof, at least $f+1$ honest parties received block $s-1$ with valid proof.
	So for any party waits for $2f+1$ fallback requests, it must see at least one fallback sent from some of these $f+1$ honest parties, thus seeing $s-1$; otherwise, there would be $3f+2$ parties. %(contradicting our baseline assumption that the number of corrupted parties $f$ is optimal $\lfloor (n-1)/3 \rfloor$).
	%We call the set $\mathsf{Good}$ formed by those $f+1$ nodes. Recall that each node has a set $\mathsf{C}$ of complaints with size $2f+1$. Thus $\mathsf{C}\cap\mathsf{Good}\neq \emptyset$. It follows that every honest input (the largest index in each received complaint set) must be at least $v-1$.
	
	The above two   claims    narrow the range of the honest parties' fallback positions  to   $\{s-1,s\}$, i.e., {\em two  unknown   consecutive integers}. %Now, we can conclude that, the simple abstraction of \nwabc\/ ensures: all honest nodes either input $\{v-1,v\}$.
	
	%We can next make two fine-grained claims: (iii) If all malicious nodes complained with indices smaller than $v+1$,  then $v+1$ cannot be any of the honest inputs to pace synchronization; (iv) Otherwise (one malicious node complained with $v+1$), then $v-1$ cannot be any of the honest inputs.
	
	%Claim (iii) is obvious, as largest honest index is also $v$. To see (iv), it is similar as (ii). From notarizability, $f+1$ honest nodes received notarized block $v$. We call the set $\mathsf{Better}$ formed by those $f+1$ nodes. Similarly, $\mathsf{C}\cap\mathsf{Better}\neq \emptyset$, where $C$ is a complain set. It follows that every honest input (the largest index in each received complaint set) must be at least $v$.
	
	
	\begin{figure}[h] 
		\vspace{-0.45cm}
		\captionsetup{font={normalsize}}
		\begin{center}
			\includegraphics[width=8.5cm]{fig/nw-abc.pdf}\\
			\vspace{-0.45cm}
			\caption{  {Notarizability}   of   fastlane abstraction ($\mathsf{nw\textnormal{-}ABC}$).}	\label{fig:nw-abc}
		\end{center}
		\vspace{-0.5cm}
	\end{figure}
	
	%Now, we can conclude that, the simple abstraction of \nwabc\/ ensures: all honest nodes either input $\{v-1,v\}$, or $\{v,v+1\}$. 
	\smallskip
	\noindent \underline{\smash{\em Second ingredient: async. agreement for   consecutive values}}.
	%
	Pace-sync now is reduced to pick one  value  of two  unknown consecutive integers  $\{s-1,s\}$. To handle the problem, we further define  {\em two-consecutive-valued Byzantine agreement} ($\tcvba$), which can be easily implemented  from any asynchronous {\em binary} Byzantine agreement (cf. Section \ref{sec:fast} for the concrete construction).
	
	%  a much simpler specific-purpose asynchronous {\em binary} Byzantine agreement, we call it {\em two-consecutive-valued binary agreement} ($\tcvba$ for short).  It not only easily brings in an  $\bigO(n)$ factor improvement to prior results  \cite{kursawe05,cachin05}, more importantly, 	$\tcvba$ has a minimal overhead (similar to that of the fastlane) compared to pessimistic path in practice.
	%
%	The new $\tcvba$ requires a special validity that: 
%	if the honest parties input one of two consecutive integers, the common output shall be one of the honest input values.
	%
%	We also give very simple constructions of $\tcvba$ from any asynchronous {\em binary} agreement.
	%We  give a very simple construction for this concrete module by only replacing  three  lines of the pseudocode of the binary agreement in \cite{guo2020dumbo}. 	
%	\Trans\/ is essentially optimal, since pace synchronization can be viewed as a version of BFT protocols itself. 
	
	
	
	
	
\ignore{%%%%%%	%	Different from  existing  MVBA instantiations that are much heavier and slower than binary agreement, 
	 {\em A general practical framework and further benefits}.
	With the two abstractions, we give a generic framework of \BDT: we start with an \nwabc, when sufficient honest parties get ``stuck'', they multicast their latest block index with the ``certificate'' and start $\tcvba$. Once they agree how to proceed and synchronize the tail, either they run \Dumbo, or restart \Bolt. Thanks to the {\em notarizability} property of \nwabc\/, when \Trans\/ is invoked, indeed enough honest  players will enter, and have one of the two indices as input thus the simple  $\tcvba$ can be used. 
	%
	Detailed security analysis requires more efforts and we prove  that the  \BDT\/  protocol    
	%lying in the new design space 
	can attain  safety and liveness in the fully asynchronous setting, without global clock or any timing assumptions.
	%
}%%%%%
	\smallskip
	\noindent\underline{\smash{\em Final piece of the puzzle: adding ``safe-buffer'' to the fastlane.}} When $\tcvba$ outputs $u$,  all honest parties can sync up to block $u$ accordingly. Because no matter $u$ is $s$ or $s-1$, the $u$-th fastlane block is with a valid quorum proof, so it can be retrieved due to notarizability (cf. Fig. \ref{fig:nw-abc}).  
	Nevertheless, a subtle issue remains: $\tcvba$ cannot guarantee $u=s$, and thus $u$ could be $s-1$. 
	This is because an asynchronous adversary can always delay the messages of the honest parties that input $s$ to make them seemingly crashed.
	That means, if a party outputs a fastlane block immediately when seeing its   proof,
	it faces a threat that the pace-sync  returns a   smaller index and revokes the latest output fastlane  block.
	This can even temporarily violate safety requirement, if   other parties output a different block after pace-sync.
	%To protect the fastest honest party in $\Bolt$ from revoking its latest fastlane block after pace-sync, 
	To solve the issue,
	we introduce a ``safe buffer'' to let the newest fastlane block
	 be {\em pending}, i.e., not output until one more fastlane block with valid proof is received.
	%only if it receives two notarized blocks, with the latter one {\em pending}.
	
	%if in $\Bolt$, each node commits a block whenever he sees the certificate, there is one honest node has already committed block $v$. But it is possible that $u=v-1$. In this case, other honest nodes may get and commit a different block $v$ thus temporarily violate safety requirement.	To resolve this, we simply introduce a ``safe buffer'' for the fastest honest node that in $\Bolt$, each node commits one block if he receives two notarized blocks, with the latter one {\em pending}.  %a block. If they are asked directly to sync to block $u$, 
	
	
	\ignore{%%%%%%
	There are several  further benefits brought about by the efficient fallback: (i) the time-out parameter now can be set aggressively, e.g., using the estimation in good days only. Doing this could quickly replace a slow (or even malicious) leader. %to synchronize (like a checkpoint) to 
	%avoid any transactions from being censored, without the need of threshold encryption \cite{honeybadger}.
	%thus achieve the {\em strong} liveness property without much overhead. 
	(ii). To better exploit the efficiency of our \Trans\/, we add a simple check to minimize the actual usage of \Dumbo: except when all honest parties  made no progress at all in the fastlane and thus have to execute the pessimistic asynchronous protocol to move forward, we let them switch back to the fastlane immediately.
	This is in contrast with previous works of \cite{kursawe05,cachin05} that the pessimistic protocol will always be run at the end of fallback, which is often unnecessarily costly. (iii) We may also execute \Trans\/ once in a while (without triggering the pessimistic path), to give each party a chance to be fastlane leader to propose blocks. 
	}%%%%%
	% in real-world Internet.
	
	%Even in the extreme case that network never keeps flucuating,  pace synchronizations is always executed before the network can eventually stabilize.
	%The overhead of frequent pace synchronizations might not only     eliminate  the   improvement of introducing the fastlane  but   even deteriorate  the overall performance  and cause it much worse than running asynchronous protocol alone.
	%, if the pace synchronization is inefficient (e.g., as slow as the underlying pessimistic path). 
	%Luckily, our highly efficient pace synchronization frees us from this worry.	
	
	%	Namely, our   ``pace'' synchronization is nearly as efficient as the state-of-the-art asynchronous binary agreement, 
	%	which seemingly is close to the best we can hope to  resolve the fallback issue in the fully asynchronous communication networks.
	
	
	
	%==
	%	What is more, the guessed network delay $\Delta_{guessed}$ is even not necessarily close to the delay upper bound $\Delta$ of unstable global Internet,
	%	since the robustness of livenss is now decoupled from $\Delta_{guessed}$ and relies on the pessimistic fallback mechanism, 
	%	that means,   aggressive timeout policies such as EOS's 500 ms per block   become   reasonable to some extent  
	%	and can be adopted to make the deterministic optimistic path much more resilient against adversary-influencing performance degradation. 
	
	%	\smallskip
	%	\item {\em Generic framework for flexible dual-path combinations.} 
	%	Moreover, our new ``pace'' synchronization protocol is powerful in the sense that it bootstraps as a generic framework that can ``graft'' varying synchronous wisdoms to many asynchronous breakthroughs. 
	%	The pessimistic path of $\mathsf{BDT}$ framework can be reduced to any asynchronous common subset (ACS) implementation, for instance, we can simply choose the state-of-the-art candidate $\dumbo$ BFT.
	%	The optimistic path is reducible to a weak atomic broadcast primitive with only asynchronous safety but no asynchronous liveness,
	%	as long as each optimistic block is outputted along with a corresponding quorum certificate (a.k.a.  a proof) to attest that enough parties (e.g., $n-f$) did optimistically output this block.
	
	%	Given  $\mathsf{BDT}$ framework,
	

	

%\end{itemize} 


%	In $\mathsf{BDT}$, each optimistic block would be finalized, once two more consecutive optimistic blocks are outputted.
%	Hence when the network is benign (e.g., a guessed network delay $\tau$ holds),
%	the optimistic path can withhold a constant probability (e.g., $1-f/n$) to drive consensus reached quickly in a deterministic manner.


%It enjoys the best of both paradigms:  (i) when the network is benign as expected (e.g., some probably aggressively guessed network delay $\Delta_{guessed}$ is satisfied), it can be really high-performing as if the state-of-the-art synchronous protocols, and (ii) while the network condition becomes worse than thought, it can efficiently fall back to perform (nearly) same to the state-of-the-art asynchronous BFT protocols.



%	{\em Remarks}. %Here   are a few remarks on the above definitions:
%
%The total-order is actually standard notions borrowed from asynchronous atomic broadcast due to \cite{cachin01, honeybadger}. %It is worth pointing out that $\tobc$ does not satisfy the standard validity notion of atomic broadcast \cite{cachin01, honeybadger}. Recall that the validity of atomic broadcast requires the protocol to make some progresses as long as there are $f+1$ honest parties have undelivered inputs. However, we do not put forth similar notion to $\tobc$. It is clear to see that the lack of validity might cause the lack of liveness guarantee. 
%
%The notarizability corresponds to a notion that is weaker than the standard agreement property of atomic broadcast. 
%To some extent, it is similar to consistency of many blockchains \cite{garay2015bitcoin}, that means any already outputted $\out[j]$ of correct parties is same, but there is no guarantee  to ensure all correct parties eventually output $\out[j]$. 
%Comparing to atomic broadcast, $\tobc$ do not have the agreement and liveness properties:
%(i) to compensate the lack of agreement, the notarizability is introduced to  guarantee that whenever an honest party outputs a block $\out[j]$ at position $j$, then at least $f+1$ honest ones already output  a block at the position $j-1$; %As such, strong consistency is essentially a notion weaker than agreement but stronger than consistency.
%(ii) liveness does not exist to any extent, as a trivial implementation actually can be: ``each party remains idle to do nothing, until the abandon interface is invoked and it aborts'';  nevertheless, this weakening allows the optimistic path  to be easily implementable in the asynchronous setting by simple deterministic protocols. Here down below we present two exemplary concise constructions.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
	
	When the optimistic path fails and has to fallback into the pessimistic path, different honest parties might have their own ``views'' on how many messages already delivered during the optimistic epoch, and it becomes necessary to make these honest parties to agree on a consistent ``view'' before falling back.
	To this end, all prior studies \cite{cachin05,kursawe05} require correct parties to ``multicast'' their ``views'' along with ``proofs'' attesting their reach of the corresponding ``views'', and then activate an MVBA instance with passing a vector of $n-f$ valid ``view-proof'' pairs as input \cite{cachin05, kursawe05},	which at least causes  $\bigO(n^3)$ communications (by any existing MVBA constructions \cite{cachin01, ittai19}). 
	%Instead, we focus on a key observation that was somehow overlooked by \cite{cachin05, kursawe05}, which is: the ``views'' of parties could be both unforgeable and already weakly agreed.
	%In particular, we consider two facts: (i) if anyone (including the adversary) presents a ``proof'' attesting its reach at a particular ``view'', there must be many honest parties (e.g. $n-2f$) that already reach the immediately precedent ``view''; (ii) many correct parties (e.g. $n-2f$) must stay at some ``views'' that are same to (or very closed to) the actual highest ``view''. 
	Instead, we develop a novel path fundamentally different from \cite{cachin05} and \cite{kursawe05} 
	to avoid the redundancy of invoking MVBA to agree on a vector of $n-f$  ``view-proof'' pairs but directly try to agree on a ``view'' number (that is very closed to the actual highest ``view''), which brings an improvement of $\bigO(n)$ factor in communication. 
	
	
	
	\item {\em Practical pessimistic path from fast asynchronous common subset.} 
	The recent elegant results of asynchronous atomic broadcast \cite{honeybadger, beat} can be naturally leveraged as the core component of the pessimistic path. However, these studies center around the asynchronous common subset (ACS) due to Ben-Or {\em et al.}, which suffers from $\bigO(\log n)$ running time and $\bigO(n^3)$ messages per instance. 
	%
	We develop fast ACS (or $\fACS$ in short), which is a novel trade-off option for ACS in the style of Ben-Or's. In particular, the critical running time and the number of messages can be asymptotically reduced. While the ``price'' of above asymptotic improvements is just the slightly amplified bandwidth usage by a constant factor $\kappa$, where $\kappa$ is a security parameter (e.g. $\kappa = 21$).
	%by slightly trading the communication off (without scarifying the asymptotic complexity of communications). 
	%First, $\fACS$ expectedly terminates in $\bigO(1)$ running time, which strictly shortens the $\bigO(\log n)$ running time of Ben-Or ACS.	
	%Second, our ACS design significantly reduces the messages complexity of Ben-Or ACS by a $\bigO(n)$ factor, 
	%as the total message per ACS instance becomes $\bigO(\kappa n^2)$
	%instead of Ben-Or's $\bigO(n^3)$ (where $\kappa$ is a security parameter, e.g., $\kappa=21$ in practice).
	%Last but not least, the ``price'' of above asymptotic improvements is just the slightly amplified bandwidth usage by a constant factor $\kappa$, where $\kappa$ is a security parameter (e.g. 21) in practice.
	
	
	The new $\fACS$ design offers a novel trade-off option for the pessimistic path of our protocol, such that it can consume less messages and progress much faster than HBBFT \cite{honeybadger} and any variants \cite{beat} (without asymptotically scarifying communication complexity). Especially in some prevalent cases that the system load is small (and/or the bandwidth of network is abundant), the new trade-off option of $\fACS$ will allow the pessimistic path of our hybrid protocol to better perform in practice.
	%
	We also remark that $\fACS$ and its novel trade-off   could be of independent interests.
	
	
	\item {\em Optimistic path in the lens of blockchain.}
	The first optimistic path design was relying on consecutive reliable broadcasts \cite{kursawe05}, which incurs $\bigO(n^2)$ messages per output. Later improvement focused on designing the optimistic path from leader-driven consistent broadcasts \cite{cachin05} to reduce message complexity to $\bigO(n)$.
	To some extent, our optimistic path is similar to \cite{cachin05} with a few changes to incorporate the recent pipelining idea \cite{hotstuff, sync-hotstuff, pala, casper} through the lens of blockchain to further improve the concrete performance.
	
	An optimistic  epoch in our protocol is driven by a leader to proceed in slots. In each slot, the (correct) leader shall decide a block that contains $n-f$ signatures that are produced by distinct parties for the block of the immediately precedent slot.	
	Moreover, this block-wise pipelining optimistic path essentially provides a couple of nice properties to be compatible with our efficient ``view-change'' design, which are: (i) the signatures contained in each block naturally becomes ``proof'' attesting a particular ``view'' (i.e., the delivery of the immediately precedent block); (ii) there are at least $n-2f$ correct parties stay at the highest ``view'' or the second-to-highest ``view''. 
	
	We for the first time well abstract the above simple design (which is essentially block-wise pipelining without leader rotation) to highlight the desired properties of the optimistic path of ``hybrid'' asynchronous atomic broadcast. In particular, though our formulation is particularly tailored in block-wise setting, it can be slightly tuned to capture the similar prior art such as \cite{cachin05}).
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%\subsection{Benchmarking in global networks}








\ignore{%%%%
	====
	To bound the rollback of optimistic blocks,
	prior studies let the honest parties sign and   broadcast their current ``paces'' in the optimistic path, 
	then each party can wait $n-f$ such pace-signature pairs and take them as input to invoke an MVBA instance. 
	A set of $n-f$ valid pace-signature pairs would   be chosen by   MVBA and returned to all honest parties.
	Since each signed pace is also attached with a small proof attesting that at least $n-2f$ honest parties indeed output its precedent blocks,  
	the parties can choose the maximum pace out of the output set of MVBA minus one as the final common pace of optimistic path to sync up, 
	which would simply bound the rollback of optimistic path because the MVBA result contains at least one honestly signed pace that is at most one block earlier than the latest block outputted by the optimistic path.
	
	
	
	{\em Our methodology}. We realize that the above ``pace'' synchronization  of using a whole set of $n-f$  pace-signature pairs as MVBA input is unnecessary.
	At the core of the $\sys$ framework,
	we provide a highly efficient alternative ``pace'' synchronization mechanism  as fast as binary agreement.
	%which can avoid the costly and slow MVBA module as well as strictly bound the possible rollback of optimistic blocks.
	
	Our main observation lies in the fact that: there are at least $n-2f$ honest parties that do output the latest two optimistic path blocks,
	so once all parties receive $n-f$ valid pace-signature pairs,
	they can simply compute the maximum among these paces. Thanks to the ``notarizability'' of our fastlane abstraction, the honest parties would get either the same value or two consecutive integers,
	and our task of ``pace'' synchronization is therefore reduced to make the honest parties choose one common integer out of those two unknown consecutive values. 
	To this end, we propose and construct a novel asynchronous Byzantine agreement primitive to solve the specific issue of agreeing between two uncertain consecutive values. The construction has  message patterns and execution flows exactly same to the state-of-the-art binary agreement protocol in \cite{guo2020dumbo} %(and its instantiation version \cite{guo2020dumbo}) 
	and only has three different lines in pseudocode for checking  slightly updated ``if-else'' conditions.
	
	
	%{\em Other design mindsets}.
	For the   efficiency of this new pace synchronization,
	we now can adopt some more aggressive  optimistic tactics as follows.
	First, different from \cite{kursawe05} that keeps on running optimistic path until it becomes problematic, we can proactively and even frequently raise ``pace'' synchronizations once the optimistic path has made enough progresses, 
	which is important to ensure ``fairness'' when the optimistic path is leader-based. 
	%Without an efficient ``pace'' synchronization, proactive switches optimistic path leaders would cause extra overhead.
	Second, different from \cite{kursawe05,cachin05} where the pessimistic path is always executed after ``pace'' synchronization, we now can invoke the pessimistic path only if the optimistic path is completely failed, i.e., even if the optimistic path seemingly goes problematic during the course of executing, 
	we would keep on trying the optimistic path again after ``pace'' synchronization as long as it remains to return some minimal output (e.g.,   one single block).
	
	====
}%%%%

%\subsection{Our contributions}




%and present a practical  framework of dual-path asynchronous BFT protocols that can enjoy the best of both synchronous and regular asynchronous protocols, namely, it realizes low-latency and high-throughput in optimistic cases and ensures robust performance in worse network scenarios. The key innovation of this article is to abstract sufficient properties for the fastlane so that we can be prepared for a very efficient fallback mechanism. In this way, the whole system can be further optimized in various aspects. % the added xxxx
%To best of our knowledge, this result is first asynchronous BFT protocol 
%time construct an asynchronous atomic broadcast protocols that is practically optimistic.
%
%In more detail, our main   contributions are: 

%This design not only enhances the performance of asynchronous protocols, but also avoid complicated timeout policy in many synchronous protocols to guess the actual 


%If enough of the party parties do not make progress in time, they will jointly execute a 


%\begin{itemize}
	
	%\smallskip
	







==> CCS 22 long-version/evaluation.tex <==
%!TEX root = main.tex

 \vspace{-0.1cm}
\section{Performance Evaluation}
\label{evaluation}

%To showcase the applicability of $\sys$, 
%We perform extensive  experiments to evaluate the prototype implementation of $\sys$ among Amazon EC2  instances distributed across five continents.
%We also comprehensively compare it  to $\mathsf{HotStuff}$ and $\mathsf{Dumbo}$ %, i.e., the state-of-the-art pipelined partially synchronous BFT and the state-of-the-art   asynchronous BFT, in the same global Internet setting.

%\medskip
%\noindent
%{\bf Highlighted experimental results}.
%Our experiments across 64 and 100 global AWS servers support an enticing  proposition that   $\sys$ (BDT)   can    achieve  the best of its both paths while being deployed in the wide-area network:
%\begin{itemize}
%	\item In the benign   case  (when each epoch's  $\tobc$ path always succeeds and then smoothly moves to the next epoch's $\tobc$ path after doing the pace synchronization via $\trans$), 
%	we verify that $\mathsf{BDT}$ can enjoy   quick confirmation as fast as $\mathsf{HotStuff}$ despite the $\trans$ overhead {\color{black}(i.e., 36 times faster than $\mathsf{Dumbo}$),}
%	demonstrating how cheap the critical $\trans$ subprotocol is to make $\mathsf{BDT}$ applicable on good days, cf. Figure \ref{fig:blatency}.
	%because our new efficient $\trans$ subprotocol adds little overhead to the $\tobc$ execution. 
%	\item In   the somewhat worse scenario   when $1/3$ optimistic paths are timed out due to $n/3$ crash faults,
%	our results   demonstrate that   $\mathsf{BDT}$   still achieves a throughput nearly as high as  the robust $\dumbo$'s  (i.e., twice of $\mathsf{HotStuff}$'s)
%	while remaining an average latency one order of magnitude smaller than $\dumbo$'s , indicating how practical $\mathsf{BDT}$ is in the unstable network, cf. Figure \ref{fig:fault}.
%	\item Even if in the arguable worst case  when all optimistic $\tobc$ executions halt to progress,
%	we realize $\mathsf{BDT}$ only has slightly increased latency when comparing to $\mathsf{Dumbo}$,
%	e.g., only few more seconds than $\dumbo$'s  (when their throughputs are same), cf. Figure \ref{fig:overhead}.
%\end{itemize}


%\subsection{Experiments setup}








 
\noindent
{\bf Implementation details}.
%The prototype implementations of BDT, $\dumbo$ and $\mathsf{HotStuff}$ are written in Python 3.
%
%For fair comparison, 
We   program the proof-of-concept implementations of $\mathsf{BDT}$, $\dumbo$ and 2-chained $\mathsf{HotStuff}$ in the same language (i.e. Python 3), with using the  same libraries and security parameters
for all   cryptographic implementations.
The   BFT protocols are implemented by single-process code.
Besides, a common     network layer is programmed   by using  unauthenticated TCP sockets.
The network layer is implemented as a separate   Python process to provide    non-blocking communication interface.% to BFT processes. 
%Inter-process communications between the BFT process and the network process are optimized for broadcasting, thus   a message broadcast incurs only constant communication between the two processes.

For common coin, it is realized by hashing   Boldyreva's pairing-based unique   threshold signature \cite{boldyreva2003threshold} (implemented over MNT224 curve).
%
For quorum proofs, we concatenate ECDSA signatures (implemented over secp256k1 curve).
%, which helps us achieve a $\dumbo$ implementation that can perform  better than the original result \cite{guo2020dumbo} where Boldyreva's   threshold signature \cite{boldyreva2003threshold} is used.
%
For threshold public key encryption, the hybrid encryption approach implemented in HoneyBadger BFT is used  \cite{honeybadger}.
%
For  erasure coding, the Reed-Solomon implementation in the zfec library is adopted.
For timeout mechanism, we  use the    clock  in each EC2 instance to implement the local time in lieu of the adversary-controlling ``clock''  in our formal security model.
\rev{Our proof-of-concept codebase is available at https://github.com/yylluu/BDT}.

%Two $\tobc$ instantiations  given in Section \ref{sec:fast}, namely, $\tobc$-$\mathsf{sCAST}$ and $\tobc$-$\mathsf{sRBC}$, are implemented.  
For notations,  $\mathsf{BDT}$-$\mathsf{sCAST}$ denotes $\mathsf{BDT}$     using       $\tobc$-$\mathsf{sCAST}$ as fastlane, 
while    $\mathsf{BDT}$-$\mathsf{sRBC}$ denotes the other instantiation   using $\tobc$-$s\RBC$. 
%
In addition, $\mathsf{BDT}$-$\mathsf{Timeout}$ denotes to use an idle fastlane that   just waits for timeout, which  can be used as benchmark to ``mimic'' the worst case that the fastlanes always  output  nothing due to constant denial-of-service attacks.
% is also a theoretic ``implementation'' of $\tobc$ (without   optimistic liveness), which is denoted as and might be used as benchmark to ``mimic'' the worst cases that the fastlanes always  output  nothing.

Due to space limitation, we only presented most intuitive experiments here, more evaluations can be found in Appendix \ref{app:data}.




\subsection{Evaluations in   wide-area network}

\noindent
{\bf Setup on Amazon EC2}. 
To demonstrate the practicability of $\BDT$ in realistic wide-area network (WAN),
we evaluate it among   Amazon EC2 c5.large instances (2 vCPUs and 4 GB   RAM) for $n$=64 and 100 parties, and also test $\dumbo$ and $\mathsf{HotStuff}$ in the same setting as reference points. 
%The evaluations are performed on  64 and 100  c5.large instances, respectively.
%Comprehensive evaluations are performed  on  64     and 100  c5.large instances, respectively. 
All  EC2 instances  are evenly distributed in 16 AWS  regions, i.e., Virginia, Ohio, California, Oregon, Central Canada, S\~ao Paulo, Frankfurt, Ireland, London, Paris, Stockholm, Mubai, Seoul, Singapore, Tokyo and Sydney. %All experiments incur about 200 GB cross-region data transfer.
\rev{All evaluation results in the WAN setting are measured back-to-back and averaged over two executions (each run for 5-10 minutes).} 

In the  WAN setting  tests, we might fix some parameters of $\mathsf{BDT}$ to intentionally amplify the fallback cost.
For example,   let each fastlane interrupt  after  output   only 50   blocks, so     $\trans$   is   frequently invoked.
We also set the fastlane's timeout parameter $\tau$ as large as 2.5 sec (nearly twenty times of the  one-way network latency in our test environment), so all fallbacks  triggered by    timeout would incur a 2.5-second overhead in addition to the $\trans$'s latency. 


\smallskip
\noindent
{\bf Basic latency}. %We   measure the latency of a transaction as the time elapsed between the moment when it appears in the front of a party's input   backlog and the moments when it is outputted to the finalized log. It is worth   noticing that  a transaction is not finalized when 
%the transaction is included by a fastlane block that is just delivered, since this block is only a $\notarized$ block, and we have to wait one more $\mathsf{Bolt}$ block for its finalization to   count the transaction's latency. 
We firstly measure   the basic latency  to reflect how fast the protocols are  (in the good cases without faults or timeouts), if all blocks have nearly zero payload (cf. Fig. \ref{fig:blatency}). This     provides us the baseline   understanding about how fast BDT, $\mathsf{HotStuff}$ and $\dumbo$ can be to  handle the scenarios favoring low-latency. 




\begin{figure}[h] 
	\captionsetup{font={normalsize}}
	\vspace{-0.2cm}
	\begin{center}
		\includegraphics[width=7.5cm]{fig/latency.pdf}\\
		\vspace{-0.4cm}
		\caption{Basic latency   in experiments over WAN for two-chain $\mathsf{HotStuff}$, $\mathsf{BDT}$-$\mathsf{sCAST}$, $\mathsf{BDT}$-$\mathsf{sRBC}$ and $\dumbo$.}	
		\label{fig:blatency}
		\vspace{-0.2cm}
	\end{center}
\end{figure}

When $n=100$, $\mathsf{BDT}$-$\mathsf{sCAST}$ is 36x faster than $\dumbo$, and  $\mathsf{BDT}$-$\mathsf{sRBC}$ is 23x faster than $\dumbo$;  when $n=64$,
$\mathsf{BDT}$-$\mathsf{sCAST}$ is 18x faster than $\dumbo$, and  $\mathsf{BDT}$-$\mathsf{sRBC}$ is 10x faster than $\dumbo$; moreover, the execution speed of both $\mathsf{BDT}$-$\mathsf{sCAST}$ and  $\mathsf{BDT}$-$\mathsf{sRBC}$ are at the same magnitude of $\mathsf{HotStuff}$. In particular, the basic latency of $\mathsf{BDT}$-$\mathsf{sCAST}$ is almost as same as that of 2-chain  $\mathsf{Hotstuff}$, which is because the fastlane of $\mathsf{BDT}$-$\mathsf{sCAST}$ can be thought of a stable-leader 2-chain  $\mathsf{Hotstuff}$ and its optimistic latency has five rounds \footnote{The five-round latency of $\mathsf{BDT}$-$\mathsf{sCAST}$ in the best cases can be   counted as follows: one round for the leader to multicast the proposed batch of transactions, one round for the parties to vote (by signing), one round for the leader to multicast the quorum proof   (and thus all parties can get a   pending block), and finally two more rounds for every parties to receive one more   block and therefore output the earlier pending block. The concrete of rounds of $\mathsf{BDT}$-$\mathsf{sRBC}$ in the best cases  can be counted similarly.}, i.e., same to that of 2-chain $\mathsf{Hotstuff}$.
%\footnote{Same as \cite{hotstuff}, we observed that $\mathsf{Hotstuff}$ with   small payload might have  a latency slightly shorter than its zero-payload case, but the difference between them is quite tiny when comparing to global Internet delay, so we still measure $\mathsf{Hotstuff}$'s basic latency by   zero payload instead of some small payload.}



\smallskip
\noindent
{\bf Peak throughput}. We then measure throughput in unit of transactions per second (where each transaction is a 250 bytes string to  approximate the size of
a typical Bitcoin transaction).  %Therefore, the throughput  can be counted as the number of output transactions over the running time of   test.
The peak throughput is depicted in Fig. \ref{fig:tps}, and 
gives us an insight how well $\mathsf{BDT}$, $\mathsf{HotStuff}$ and $\dumbo$ can handle transaction burst. \footnote{Note that we didn't implement an additional layer of mempool as in \cite{gao2022dumbong} and \cite{danezis2022narwhal}, and we can expect much higher throughout if we adopt their mempool techniques.}



\begin{figure}[h] 
	\vspace{-0.2cm}
	\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=7.2cm]{fig/tps.pdf}\\
		%\vspace{-0.1cm}
		\vspace{-0.4cm}
		\caption{Peak throughput in experiments over WAN for two-chain $\mathsf{HotStuff}$, $\mathsf{BDT}$-$\mathsf{sCAST}$, $\mathsf{BDT}$-$\mathsf{sRBC}$ and $\dumbo$.}\label{fig:tps}	
	\end{center}
	\vspace{-0.2cm}
\end{figure}




$\mathsf{BDT}$-$\mathsf{sCAST}$ realizes a peak throughput   about 85\% of $\mathsf{HotStuff}$'s  when either $n$ is 100 or 64,  
$\mathsf{BDT}$-$\mathsf{sRBC}$ achieves a peak throughput that is as high as around 90\% of $\dumbo$'s   for  $n=64$ case and about 85\% of $\dumbo$'s    for  $n=100$ case. All these throughput numbers are achieved despite frequent $\trans$ occurrence, as we intend to let each fastlane to  fallback after  output mere   50 blocks.











\medskip
\noindent
{\bf Overhead of $\trans$}. It is critical for us to understand the  practical cost   of $\trans$.
%since cheaper $\trans$ can enable smoother fallback from the optimistic fastlane to the pessimistic path.
%the overhead of optimistic path failures, and therefore more aggressive   design spaces,  
%(e.g., a tighter $\tau$ chosen to more closed to each block's generation latency in the $\mathsf{Bolt}$ path) 
%such as 
%for example, smaller timeout parameter $\tau$ can be attempted to squeeze performance out of any good  periods when the network is on   good days.
%
We estimate such overhead from two different perspectives as shown in Fig. \ref{fig:vc} and \ref{fig:overhead}.
%\rev{In particular, Fig. \ref{fig:vc} compares $\BDT$'s $\trans$ to RC05's $\mathsf{MVBA}$ fallback, and Fig \ref{fig:overhead} plots the latency-throughput trade-offs of $\BDT$ (without successful fastlanes) and Dumbo, because their  variance captures the cost of $\trans$.}



\begin{figure}[h] 
	\vspace{-0.2cm}
	\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=7.5cm]{fig/view.pdf}\\
		\vspace{-0.43cm}
		\caption{Latency of   $\trans$ for pace-sync  in $\mathsf{BDT}$-$\mathsf{sCAST}$ and $\mathsf{BDT}$-$\mathsf{sRBC}$ (when no fault and 1/3 crash, respectively). MVBA fallback in RC05 is also tested   as a reference point.}	
		\label{fig:vc}
	\end{center}
	\vspace{-0.2cm}
\end{figure}




As shown in Fig. 	\ref{fig:vc}, we   measure the execution time of   $\trans$   in various settings
by taking combinations of the following setups: (i)   $\mathsf{BDT}$-$\mathsf{sCAST}$ or $\mathsf{BDT}$-$\mathsf{sRBC}$; (ii)    $1/3$ crashes on or off; (iii) 64 EC2 instances or 100 EC2 instances. \rev{Moreover, in order to comprehensively compare $\trans$ with the prior art \cite{kursawe05,cachin05,700aublin},	
	we   also measure the latency of $\mathsf{MVBA}$   pace-sync (which instantiates the $\mathsf{Backup}$/$\mathsf{Abstract}$ primitive in \cite{700aublin} to combine the fastlane and $\mathsf{Dumbo}$ \footnote{\rev{Following \cite{700aublin} that used full-fledged $\mathsf{SMR}$ to instantiate Backup for fallback, 
			one can %use a block of asynchronous $\mathsf{SMR}$ to implement pace-sync 
			combine stable-leader 2-chain $\mathsf{HotStuff}$ (the fastlane of $\mathsf{BDT}$-$\mathsf{sCAST}$) and $\mathsf{Dumbo}$ by a single block of asynchronous $\mathsf{SMR}$.
			This intuitive idea can be realized from $\mathsf{MVBA}$  \cite{cachin01,cachin05} as follows after the fastlane times out: each party   signs and multicasts the highest quorum proof  received from $\mathsf{HotStuff}$, then waits for $n-f$ such signed   proofs from distinct parties, and takes them as $\mathsf{MVBA}$ input;   $\mathsf{MVBA}$ thus would output $n-f$ valid $\mathsf{HotStuff}$ quorum proofs (signed by $n-f$   parties), and the highest quorum proof in the   $\mathsf{MVBA}$ output can represent the $\mathsf{HotStuff}$ block   to continue $\mathsf{Dumbo}$.}}) as a basic reference point, cf. Section 2 for the idea of using $\mathsf{Backup}$/$\mathsf{Abstract}$ for asynchronous fallback \cite{700aublin}.
}    
The comparison indicates that $\trans$ is much cheaper in contrast to the high cost of $\mathsf{MVBA}$ pace-sync.
For example,   $\trans$     always costs less than 1 second in $\mathsf{BDT}$-$\mathsf{sRBC}$, despite $n$ and on/off of crashes, while $\mathsf{MVBA}$ pace-sync is about 10 times slower.
%in all cases, $\mathsf{BDT}$-$\mathsf{sCAST}$ has a $\trans$ phase   longer       than  that in $\mathsf{BDT}$-$\mathsf{sRBC}$, which is because in $\mathsf{BDT}$-$\mathsf{sRBC}$, all parties would more likely take the same input to $\tcvba$, causing this randomized module easier to terminate. % and then saving some overhead on average.



\begin{figure}[h] 
	\captionsetup{font={normalsize}}
	\vspace{-0.3cm}
	\begin{center}
		\includegraphics[width=7.5cm]{fig/overhead.pdf}\\
		\vspace{-0.3cm}
		\caption{Latency v.s. throughput for experiments of $\mathsf{BDT}$ with   idling fastlane (i.e.,   fastlane just timeouts after 2.5 sec).}	
		\label{fig:overhead}
	\end{center}
	\vspace{-0.4cm}
\end{figure}



%
As illustrated in Fig. \ref{fig:overhead}, 
we measure the latency-throughput tradeoffs for $\mathsf{BDT}$-$\mathsf{Timeout}$, namely, to see how   $\mathsf{BDT}$   worse than $\dumbo$ when $\mathsf{BDT}$'s fastlane is under denial-of-service.
This is arguably the   worst-case  test vector for  $\mathsf{BDT}$, since relative to $\mathsf{Dumbo}$, it always costs extra 2.5 seconds to timeout and then executes the    $\trans$ subprotocol. Nevertheless,    the performance of $\mathsf{BDT}$  is still close to $\dumbo$. In particular, to realize the same throughput, $\mathsf{BDT}$    spends only a few additional seconds (which is  mostly caused by our conservation 2.5-second timeout parameter).



\medskip
\noindent
{\bf Latency-throughput trade-off}.  \rev{Figure \ref{fig:nofault} plots   latency-throughput trade-offs of $\mathsf{BDT}$-$\mathsf{sCAST}$, $\mathsf{BDT}$-$\mathsf{sRBC}$, $\mathsf{HotStuff}$ and $\mathsf{Dumbo}$ in the WAN setting for $n$= 64 and 100 parties. This illustrates that  $\mathsf{BDT}$ has low latency close to that of $\mathsf{HotStuff}$ under varying system load.}


\begin{figure}[h] 
	\vspace{-0.4cm}
	\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=7.5cm]{fig/nofault.pdf}\\
		\vspace{-0.3cm}
		\caption{Throughput v.s. latency for experiments  over WAN  when $n=64$ and $100$, respectively (in case of periodically running pace-sync in $\mathsf{BDT}$ per only 50 fastlane blocks).}	
		\label{fig:nofault}
	\end{center}
	\vspace{-0.3cm}
\end{figure}

Either $\mathsf{BDT}$-$\mathsf{sCAST}$ or $\mathsf{BDT}$-$\mathsf{sRBC}$ is much faster than $\dumbo$ by several orders of magnitude in all cases, while the two $\mathsf{BDT}$ instantiations have different favors  towards distinct scenarios.
%
$\mathsf{BDT}$-$\mathsf{sCAST}$ has a latency-throughput trade-off similar to that of 2-chain $\mathsf{HotStuff}$, and their small variance in latency is because we intentionally trigger timeouts in $\mathsf{BDT}$-$\mathsf{sCAST}$ after each 50 fastlane blocks.
%,
%and is more favoring latency comparing to $\dumbo$. For example, when fixing throughput around 5000 tps, $\mathsf{BDT}$-$\mathsf{sCAST}$ has  a latency only   about $0.5$ sec  when $n=64$, and a latency   about $0.9$ sec   when $n=100$; in contrast, $\dumbo$ needs about 10 sec or 20 sec to realize the same throughput for $n=64$ and $n=100$, respectively. %This results in the difference of latency in several magnitudes when requiring only moderate throughput, say 5000 tps.
%
$\mathsf{BDT}$-$\mathsf{sRBC}$ has a latency-throughput trend quite different from $\mathsf{HotStuff}$ and $\mathsf{BDT}$-$\mathsf{sCAST}$. 
Namely, when fixing larger throughput, $\mathsf{BDT}$-$\mathsf{sRBC}$ has a latency less than $\mathsf{BDT}$-$\mathsf{sCAST}$'s;
when fixing   small throughput,  $\mathsf{BDT}$-$\mathsf{sRBC}$ could be slower.
This separates them clearly in terms of application scenarios, since $\mathsf{BDT}$-$\mathsf{sRBC}$ is   a better choice for large throughput-favoring cases and $\mathsf{BDT}$-$\mathsf{sCAST}$ 
is more suitable for latency-sensitive scenarios. %The rationale behind the different latency-throughput favoring is that the $\mathsf{sRBC}$ based fastlane can better balance the network load, causing eventual better performance when leaning towards higher throughput.





\medskip
\noindent
{\bf Summary of evaluations in the  WAN setting}.
The above   results clearly demonstrate the   efficiency of our pace-synchronization---$\trans$.
And thanks to that, $\BDT$  in the WAN setting is:
\begin{itemize}[leftmargin=0.6cm]
	\item As fast as 2-chain $\mathsf{HotStuff}$ in the best case (i.e., synchronous network without faulty parties); \footnote{\rev{As discussed in Footnote 4, $\mathsf{BDT}$-$\mathsf{sCAST}$'s fastlane has a 5-round latency, which is same to that of 2-chain $\mathsf{HotStuff}$. The tiny difference between their evaluated latency is because we periodically trigger $\Trans$  in the experiments of $\mathsf{BDT}$-$\mathsf{sCAST}$.}}
	\item As robust as the underlying asynchronous pessimistic path  in the worst case (i.e., the fastlane always completely fails).
\end{itemize}

%For sake of completeness, we also measure (i)    latency and throughput on varying batch sizes and (ii) the      latency-throughput trade-off of all tested protocols. See Appendix \ref{app:exp} for these minor results.




\subsection{Evaluation in  controlled  dynamic  network}

\noindent
{\bf Setup on the simulated fluctuating  network}. 
%To take an in-depth understanding about the effectiveness of $\BDT$ in the fluctuating Internet environment (i.e.,   scenarios between  the worst case and  the best case), 
We also deploy our Python-written protocols for  $n$=64 parties in  a high-performance server
 having 4 28-core   Xeon Platinum 8280 CPUs and 1TB RAM. 
% 
The   code is same to the earlier WAN experiments, except that we implement all   TCP sockets   with controllable bandwidth and delay. This allows us to  simulate a dynamic  communication network. 

In particular, we  interleave    ``good'' network (i.e., 50ms delay and 200Mbps bitrate) and   ``bad'' network  (i.e.,  300ms delay and 50Mbps bitrate) in the following experiments to reflect network fluctuation. \rev{Through  the subsection, $\BDT$ refers to $\BDT$-$\mathsf{sCAST}$, the   approach of using  Abstract  primitive \cite{700aublin}  to combine   stable-leader  2-chain $\mathsf{HotStuff}$ ($\BDT$-$\mathsf{sCAST}$'s fastlane)  and $\mathsf{Dumbo}$    is denoted by $\mathsf{HS}$+$\mathsf{Abstract}$+$\mathsf{Dumbo}$ (where   Backup/Abstract   is instantiated by $\mathsf{MVBA}$ as explained in Footnote 5).
	For experiment parameters, the fastlane's timeout   is  set as 1 second, the fastlane block and  pessimistic   block  contain  $10^4$ and  $10^6$ transactions respectively, and we would   report the number of confirmed transactions over time in   random sample executions.} 






\smallskip
\noindent
{\bf Good network with  very short fluctuations}. We first examine in a network that mostly stays at good condition except interleaving some short-term bad network condition   that lasts only 2 seconds (which just triggers fastlane timeout). The sample executions in the setting are  plotted in Fig. \ref{fig:change-1}. 
The result indicates that the performance of $\BDT$ does not degrade due to the several short-term network fluctuation, 
and it remains as fast as 2-chain $\mathsf{HotStuff}$. This feature is because $\BDT$ adopts a two-level fallback mechanism, such that   it can just execute the light pace-sync and then immediately retry another fastlane. \rev{In contrast,   using $\mathsf{Backup}$/$\mathsf{Abstract}$ primitive (instantiated by $\mathsf{MVBA}$) as pace-sync     would encounter rather long latency ($\sim$25 sec) to run the heavy pace-sync and   pessimistic path after the short-term network fluctuations.} 

%. All sockets have  for most time, and only encounter some short-term bad network condition   that lasts only 2-seconds.
 
 
 

\begin{figure}[h] 
	%\vspace{-0.2cm}
	\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=7.2cm]{fig/change-1.pdf}\\
		\vspace{-0.35cm}
		\caption{Sample executions of $\mathsf{BDT}$, 2-chain $\mathsf{HotStuff}$, $\dumbo$, \rev{and the  composition of $\mathsf{HotStuff}$+$\mathsf{Abstract}$+$\mathsf{Dumbo}$} for $n$=64, when facing a few 2-second bad periods. The red region represents the 2-second period of bad network.}	\label{fig:change-1}
		%\caption{The overview of our new practical and generic optimistic atomic broadcast framework, nicknamed by $\sys$.}	\label{fig:BDT}
	\end{center}
	\vspace{-0.4cm}
\end{figure}

\smallskip
\noindent
{\bf Intermittent network with long  bad time}. We then evaluate the effect of long-lasting bad network condition. We visualize such sample executions in Fig. \ref{fig:change-2}. Clearly, $\BDT$   can closely track the performance of its underlying pessimistic path during the long  periods of bad network condition. Again, this feature is a result of efficient pace-sync, as it adds minimal overhead to the fallback. \rev{In contrast,  using Backup/Abstract primitive (instantiated by $\mathsf{MVBA}$)   to compose stable-leader $\mathsf{HotStuff}$ and $\dumbo$  would incur a latency  $\sim$10 seconds larger than $\BDT$ during the bad network due to its cumbersome pace-sync.}





\begin{figure}[h] 
	\vspace{-0.4cm}
	\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=7.2cm]{fig/change-2.pdf}\\
		\vspace{-0.4cm}
		\caption{Sample executions of $\mathsf{BDT}$,  2-chain $\mathsf{HotStuff}$, $\dumbo$, \rev{and the composition of $\mathsf{HotStuff}$+$\mathsf{Abstract}$+$\mathsf{Dumbo}$} for $n$=64, when suffering from 120-second bad network. The red region represents the 120-second period of bad network.}	\label{fig:change-2}
		%\caption{The overview of our new practical and generic optimistic atomic broadcast framework, nicknamed by $\sys$.}	\label{fig:BDT}
	\end{center}
	\vspace{-0.4cm}
\end{figure}
 

\smallskip
\noindent
{\bf Summary of evaluations in   fluctuating network}. %Besides that $\BDT$ is as fast as 2-chain HotStuff in the best case and as robust as underlying pessimistic path in the worst case, 
As expected by our efficient pace-sync subprotocol, $\BDT$ also performs well in the fluctuating network environment. Specifically,
\begin{itemize}[leftmargin=0.6cm]
	\item When   encountering short-term network fluctuations, $\BDT$ can quickly finish pace-sync and restart a new fastlane, thus progressing at a speed same to 2-chain $\mathsf{HotStuff}$.
	\item When the network   becomes slow for longer periods (and even $\mathsf{HotStuff}$   grinds to a halt), $\BDT$ still is robust to  progress    nearly as fast as the underlying   asynchronous    protocol.
\end{itemize}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> CCS 22 long-version/fast.tex <==
%!TEX root = main.tex

%\medspace
\section{AllSpark: Fastlane Abstraction and  Two-Consecutive-Value BA}\label{sec:fast}


%As briefly discussed in Introduction, 
%The  practical impact of    
%$\mathsf{BDT}$     immediately benefits from the   efficient pace-synchronization   ($\mathsf{Transformer}$) centered around the conceptually simplest binary agreement in lieu of   any complicated multi-value agreement. 

The simple and efficient pace-synchronization is the crux of making $\mathsf{BDT}$ practical,  
and this becomes possible for two critical ingredients, i.e., a novel fastlane abstraction ($\mathsf{nw\textnormal{-}ABC}$) and a new variant of binary Byzantine agreement ($\mathsf{tcv\textnormal{-}BA}$). Specifically,




\begin{itemize}[leftmargin=0.6cm]
	\item   $\mathsf{nw\textnormal{-}ABC}$ ensures that all parties' fastlane outputs are somewhat weakly consistent, namely, 
	if the $(s)$-th block is the latest block with valid quorum proof,
	then at least $f+1$ honest parties must already output the $(s-1)$-th block   with the valid quorum proof (cf. Fig. \ref{fig:nw-abc}).
	%Therefore, after all honest parties exchange timeout requests with notifying each other about their latest block's quorum proof, everyone shall at least receive the 2nd to the highest block's proof, and at most receive the highest block's quorum proof.
	\item Considering the above property of $\mathsf{nw\textnormal{-}ABC}$ fastlane, we  can conclude that: after exchanging timeout requests, all honest parties either know $s$  or $s-1$. 
	We thus lift the conventional binary agreement to a special variant ($\mathsf{tcv\textnormal{-}BA}$) for deciding a common value out of $\{s-1, s\}$, despite that 
	the adversary might input arbitrarily, say  $s-2$ or $s+1$.
\end{itemize}

 
%This section would elaborates these two critical ingredients.


%Nevertheless, the challenge of constructing $\mathsf{tcv\textnormal{-}BA}$ remains because the adversary can input fake values outside $\{s, s-1\}$, for example,  $s-2$ or $s+1$.

%The seemingly trivial solution to the issue is letting the index value modulus 2 and then invoke binary agreement.





%\section{Notarizable Weak Atomic Broadcast: Abstraction and Implementations of Bolt}
%\label{sec:fast}




\vspace{-0.2cm}

\subsection{Abstracting and constructing    the fastlane}

%\subsection{Defining $\tobc$: the optimistic path abstraction}
%Our first ingredient   is a new fastlane abstraction and its construction with nickname $\tobc$. 
%This is the key component to ensure that all parties' outputs in the fastlane  are weakly consistent, thus enabling the simplification of pace-synchronization.
%To abstract the key features of this critical building block, we put forth the notion of notarizable weak atomic broadcast ($\mathsf{nw\textnormal{-}ABC}$) as follows. 

%To enable   efficient  pace-synchronization built from  binary agreement only,  
We first put forth  notarizable weak atomic broadcast ($\mathsf{nw\textnormal{-}ABC}$)   to better prepare the fastlane for more efficient pace-sync.

\begin{definition} {{\bf Notarizable weak atomic broadcast}   ($\mathsf{nw\textnormal{-}ABC}$, nicknamed by $\tobc$)}. %{\bf  notarizable  weak  atomic broadcast.}
	In the   protocol with an identification $\id$, %:=(e, h_{\genesis})$ 
	 %It is joined by $n$ nodes that continuously receive a sequence of transactions as input, and each correct participating node might output a sequence of $\blocks$. 
	 each party takes  a  transaction buffer   as input and  outputs a   $\out$ of blocks, where each block $\out[j]$ is in form of $\langle \id, j, \payload_j, \prf_{j} \rangle$. 
	 There also exists two external functions $\LogVerify$  and $\Extract$ taking $\id$, slot $j$ and $\prf_{j}$ as input (whose outputs and functionalities would soon be explained below). We require that $\tobc$   satisfies the following properties except with negligible probability:
	\begin{itemize}[leftmargin=0.6cm]
		\item {\em Total-order}. 
		%If a correct node outputs a sequence of $\blocks$,
		%and another correct node outputs a sequence of blocks $\blocks'$, 
		%then $\blocks[j]=\blocks'[j]$ for every $i$ that $1 \le j \le \min\{|\blocks|,|\blocks'|\} $.
		%\item {\bf Total-order}. If an honest party outputs a sequence of  $\blocks$ called $\out$, and another honest party outputs a sequence of   blocks called $\out'$, then $\out[i]=\out'[i]$ for every $i$ that $1 \le i \le \min\{|\out|,|\out'|\}$, which is 
		Same to   atomic broadcast.
		
		\item {\em Notarizability}. If any (probably malicious) party outputs  $\out[j]:=\langle \id, j, \payload_j, \prf_j \rangle$   s.t.   $\LogVerify(\id, j, \prf_j)=1$,  then: there exist at least $f+1$ honest parties, each of which either already outputs $\out[j]$, or  already outputs $\out[j-1]$ and can    invoke  $\Extract$ function with valid $\prf_j$ to
		extract $\out[j]$  from   received protocol scripts.
		
		\item {\em Abandonability}.  An honest party  will not output any block in $\tobc[\id]$ after invoking $\abandon(\id)$. In addition, if $f+1$ honest parties invoke $\abandon(\id)$ before   output $\out[j]$, then no party can output valid $\out[j+1]$.
		
		\item {\em Optimistic liveness}. There exist  a non-empty collection of optimistic conditions  to specify the honesty of   certain   parties, s.t. once an honest party outputs $\out[j]$, it will output   $\out[j+1]$ in $\kappa$ asynchronous rounds, where  $\kappa$ is a   constant.

	\end{itemize}
\end{definition}






Comparing to    $\mathsf{ABC}$, 
$\mathsf{nw}$-$\mathsf{ABC}$ does not have  the exact agreement and liveness properties:
(i) notarizability   compensates the lack of agreement, as it ensures that  whenever a party outputs a block $\out[j]$ at position $j$,   at least $f+1$ honest parties already output  at the position $j-1$, and in addition, $f+1$ honest parties   already receive the protocol scripts carrying the payload of $\out[j]$, so they can   extract the block $\out[j]$ once seeing   valid $\prf_j$; %As such, strong consistency is essentially a notion weaker than agreement but stronger than consistency.
(ii) liveness is in an optimistic form, which enables       simple deterministic   implementations of $\mathsf{nw}$-$\mathsf{ABC}$ in the asynchronous setting. %in particular, some classic leader-based ones. 
%Note that the optimistic liveness excludes a trivial implementation of fastlane: ``each party remains idle to do nothing, until the abandon interface is invoked to abort''. 
%
%\rev{In addition, we also do a detailed comparison with the Abstract \cite{700aublin}, cf. Appendix \ref{sec:700} for differences.}


Careful readers might   notice  that the above fastlane abstraction, in particular the notarizability property, share similarities with the popular lock-commit paradigm widely used in   (partially) synchronous byzantine/crash fault tolerant protocols \cite{partialsync,tendermint,pbft,sbft,yin2018hotstuff-full}. 
For example, when any honest party outputs some value (i.e. ``commit''), then at least $f+1$ honest parties shall receive and already vote this output (i.e. ``lock'').
%This      is captured by notarizability, so an output block with valid proof can ensure that at least $f+1$ honest parties can extract the same block from its protocol messages (because they must already receive the block and vote it).
%We remark that this new  is fine-tuned for the authenticated asynchronous setting. 
In such a sense, the fastlane can be easily instantiated in many ways through the lens of  (partially) synchronous protocols. 
Unsurprisingly, one candidate is the fastlane  used in KS05 \cite{cachin05}.
Here  we present two more   exemplary  $\tobc$ constructions.


\smallskip
\noindent
\underline{\smash{\em \rev{Comparing with the  $\mathsf{Abstract}$ component in  \cite{700aublin}}}}. 
\rev{As aforementioned, \cite{700aublin} defined $\mathsf{Abstract}$ as a basic component to compose full-fledged BFT consensus with optimistic fastlane.
$\mathsf{Abstract}$ was defined to capture  a very broad array of optimistic conditions (including very optimistic cases such as no fault at all), 
such that a fastlane satisfying $\mathsf{Abstract}$ definition could be designed as simple as possible (with the price that no guarantee of similar progress among honest parties, as we have, before triggering fallback).
For example, \cite{700aublin} presented  $\mathsf{Quorum}$, an implementation of $\mathsf{Abstract}$ that only involves one round trip (with an optimistic condition allowing no fault),
but $\mathsf{Quorum}$ cannot meet the critical notarizability property of $\mathsf{nw}$-$\mathsf{ABC}$ though satisfying $\mathsf{Abstract}$.
%because it deviates from ``lock''-``commit'' paradigm for 2-round optimistic latency. 
Taking $\mathsf{Quorum}$ as example, the  weakening of $\mathsf{Abstract}$ prevents us from using binary agreement to handle some failed $\mathsf{Abstract}$ fastlanes, because the parties cannot reduce the failed position of the fastlane to two consecutive numbers.
This corresponds to the necessity of our stronger $\mathsf{nw}$-$\mathsf{ABC}$ definition in the context of facilitating a simplest possible pace-sync in the asynchronous setting.
}




%\subsection{$\mathsf{Bolt}$-$\mathsf{sCAST}$ from sequential multicasts}
%\medskip
\smallskip
\noindent
{\bf $\mathsf{Bolt}$ from sequential multicasts}. 
  As shown in   Fig. \ref{fig:multicast}, $\tobc$ can be easily constructed  from pipelined multicasts with using threshold signature, %(as a  simplified $\mathsf{HotStuff}$ where the blocks are not ``chained'' because of the specific purpose  for stable leader), 
  and we call it $\mathsf{Bolt}$-$\mathsf{sCAST}$. The   idea  is as simple as: the leader proposes a batch of transactions via   multicast, %\footnote{Remark that our optimistic path abstraction is quite general. As an example, we also can let every party send a signed $tx$ to the leader, and the leader can  combine at least $n-f$ tx-signature pairs as a set $\payload$ and then multicasts $\payload$ as proposal, and other parties   vote only if $\payload$ contains $n-f$ tx-signature pairs. This can guarantee a block-quality property, i.e., at least half $tx$ of each block would be from honest parties, though latency could be sacrificed. Moreover, the optimistic path  in \cite{cachin05} also satisfies our abstraction.}  
  then all parties send back their signatures on the proposed batch as their votes,
  once the leader  collects enough votes from distinct parties (i.e., $2f+1$), it uses the votes to form a quorum proof for its precedent proposal,
   and then repeats to multicast a new proposal of transactions (along with the proof). Upon receiving the new proposal and the precedent proof, the parties   output the precedent proposal and the proof (as a block), and then    vote  on the new proposal. Such   execution is   repeated until the abandon interface is invoked.



\vspace{-0.1cm}
\begin{figure}[h]
	\captionsetup{font={normalsize}}
	\begin{footnotesize}
		\vspace{-0.1cm}
		\fbox{%
			\parbox{8.2cm}{				
				
				let $\id$ be the session identification of $\tobc[\id]$, $\buf$ be a FIFO queue of input, $B$ be the batch parameter,  and  $\node_\ell$ be the leader (where $\ell=(\id\mod n) +1$)
				
				\vspace{0.1cm}
				$\node_i$ initializes $s=1$, $\sigma_0=\bot$  and runs the protocol in  consecutive slot number $s$ as:
				
				\begin{itemize}[leftmargin=0.3cm]			
					\item	\textbf{Broadcast}. if $\node_i$ is the leader $\node_\ell$
					\begin{itemize}[leftmargin=0.25cm]
						
						%\item	if $s = 1$ 	then:  multicast $\proposal(\id, s, \payload_s,\sigma_{s-1})$, where $\payload_s \leftarrow \buf[:B]$						
						
						\item	if $s > 1$ then: 
						\begin{itemize}[leftmargin=0.25cm]
							\item wait for $2f+1$ $\vote(\id, s-1,\sigma_{s-1,i})$ from distinct parties $\node_i$, where $\sigma_{s-1,i}$ is the valid partial signature signed by $\node_i$ for $\langle \id, s-1, \hash(\payload_{s-1}) \rangle$ 
							%{\color{orange}
							%// To be precise, $\vote$ carries $\sigma_{s-1,i}$, s.t. $\TSIG.\VrfyShare_{2f+1}(\langle \id, s-1, \hash(\payload_{s-1}) \rangle, (i,\sigma_{s-1,i})) =1$}
							
							\item compute $\sigma_{s-1}$,   the   full-signature for $\langle \id, s-1, \hash(\payload_{s-1}) \rangle$,
							by aggregating the $2f+1$ received valid partial signatures
							
							%{\color{orange}// To be precise, that means $\sigma_{s-1} \leftarrow\TSIG.\Combine_{2f+1}( \langle \id, s-1, \hash(\payload_{s-1}) \rangle,\{(i, \sigma_{s-1,i})\}_{2f+1} )$}
							
							
						\end{itemize}
						
						%where  $\TSIG.\VrfyShare_{2f+1}(\langle e, s-1, \hash(\payload_{s-1}) \rangle, (i,\sigma_{s-1,i})) =1$, $ \sigma_{s-1} \leftarrow\TSIG.\Combine_{2f+1}( \langle e, s-1, \hash(\payload_{s-1}) \rangle, $ $\{(i, \sigma_{s-1,i})\}_{2f+1} )$
						
						\item multicast $\proposal(\id, s, \payload_s,\sigma_{s-1})$, where $\payload_s \leftarrow \buf[:B]$ %{\color{orange}// Here it selects the first $B$-sized transactions at the front of $\buf$}
						
					\end{itemize}			
					
					\item	 \textbf{Commit and Vote}. upon receiving    $\proposal(\id, s, \payload_s,\sigma_{s-1})$ from   $\node_\ell$ 
					\begin{itemize}[leftmargin=0.3cm]
						
						%\item	if $s = 1$ then: send $\vote(e, s, \sigma_{s,i})$ to the leader $\node_l$, where $\sigma_{s,i} \leftarrow \TSIG.\SignShare_{2f+1}(sk_i, \langle e, s,  \hash(\payload_s) \rangle)$, then let $ s\leftarrow s+1$
						
						\item	if $s > 1$ then:
						
						\begin{itemize}[leftmargin=0.25cm]
							\item  proceed only if $\sigma_{s-1}$ is valid full signature that aggregates $2f+1$ partial signatures for $\langle \id, s-1, \hash(\payload_{s-1}) \rangle$,  otherwise abort
							
							%{\color{orange}// To be precise,  that means a valid $\proposal$ message shall carry $\sigma_{s-1}$ s.t. $\TSIG.\Vrfy_{2f+1}(\langle \id, s-1, \hash(\payload_{s-1}) \rangle, \sigma_{s-1}) = 1$}
							
							\item  output $\block$:=$ (\id, s-1, \payload_{s-1}, \prf_{s-1})$, where $\prf_{s-1}:=\langle \hash(\payload_{s-1}), \sigma_{s-1} \rangle$
							
							
						\end{itemize}			
						
						\item  send $\vote(\id, s, \sigma_{s,i})$ to the leader $\node_\ell$, where $\sigma_{s,i}$ is the partial signature for $\langle \id, s,  \hash(\payload_s) \rangle$, then let $ s\leftarrow s+1$
						
						%{\color{orange}// To be precise,  that means the $\vote$ message to send carries $\sigma_{s,i} \leftarrow \TSIG.\SignShare_{2f+1}(sk_i, \langle \id, s,  \hash(\payload_s) \rangle)$}
						
					\end{itemize}
					
					\item \textbf{Abandon}. upon $\abandon(\id)$ is invoked then:   abort the above execution
					
				\end{itemize}
				\vspace{-0.1cm}
			}
		}
		\vspace{-0.3cm}
		\caption{$\tobc$ from sequential multicasts ($\mathsf{Bolt}$-$\mathsf{sCAST}$). The external functions are presented in Fig. \ref{fig:external}.}% (which might be viewed as HotStuff that is specifically simplified for stable leader and no view-change).}
		
		\label{fig:multicast}
	\end{footnotesize}
	 \vspace{-0.2cm}
\end{figure}





\ignore{
\begin{lemma}	
	The algorithm in Figure \ref{fig:multicast} satisfies the {\em total-order}, {\em notarizability}, {\em abandonability} and {\em optimistic liveness} properties   of $\tobc$  except with negligible probability.
	\label{abc1}
\end{lemma}


{\em Proof}: Here we prove the three properties one by one:

{\em For total-order}: First, we prove at same position, for any two honest parties $\node_i$ and $\node_j$ return $\block_i$ and $\block_j$, respectively, then $\block_i = \block_j$. It is clear that if the honest party $\node_i$ outputs $\block_i$, then at least $f+1$ honest parties did vote for $\block_i$ because $\TSIG.\Vrfy_{2f+1}$ passes verification. So did  $f+1$ honest parties vote for $\block_j$. 
That means at least one honest party votes for both blocks, so $\block_i = \block_j$.

{\em For notarizability}: Suppose a party $\node_i$ outputs   $\blocks[j]:=\langle \id, j, \payload_j, \prf_j \rangle$, it means at least $f+1$ honest parties   vote  for $\block[j]$, according to  the pseudocode,  at least those same $f+1$ honest parties already output $\blocks[j-1]$ and  received the $\payload_j$, hence,  those honest parties can further use the valid $\prf_j$ to extract $\blocks[j]$ from the received protocol messages.

{\em For abandonability}: it is immediate to see from the pseudocode of the abandon interface.

{\em For optimistic liveness}: suppose that the optimistic condition is that the leader is honest, then any honest party would output $\block[1]$ in three asynchronous rounds after entering the protocol
and   would output     $\out[j+1]$ within two asynchronous rounds after outputting $\out[j]$ (for all $j\ge1$).
$\hfill\square$ 

}








 \smallskip
\noindent
{\bf $\mathsf{Bolt}$ from sequential reliable broadcast}.
As shown in Fig. \ref{fig:prbc}, we can also use sequential $\rbc$ instances   to implement $\tobc$.
In the implementation, a designated fastlane leader can reliably broadcast its proposed transaction batches one by one.
For each party receives a batch from some $\rbc$, it signs the   batch and  $\rbc$'s identifier, and multicasts the signature as vote, 
then wait for $2f+1$ valid votes to form a quorum proof, such that the batch and the proof assemble  an output block, and the party  proceeds into the next $\rbc$.
%\subsection{$\mathsf{Bolt}$-$\mathsf{sRBC}$ from sequential reliable broadcasts}
Note that a $\RBC$ implementation \cite{honeybadger} can use the technique of verifiable information dispersal \cite{cachin2005asynchronous} for communication efficiency as well as balancing network workload, such that the leader's bandwidth usage is at the same order of other parties'.
In contrast, $\mathsf{Bolt}$-$\mathsf{sCAST}$ might cause the  leader's bandwidth usage   $n$ times more than the other parties', 
unless an additional mempool layer is implemented to further decouple the dissemination of transactions from $\Bolt$.
%, hence, it is heavy for the leader unless the leader obtains more resources.
%This can restrict each block's   batch size and becomes the throughput bottleneck, 
%unless  the leader has significant  physical resources or implement additional mempool layer. 
%We therefore present an alternative $\tobc$ implementation  to remove the   bottleneck.

%borrowed from   to balance the communications over the whole network .
%For  $\tobc$'s notarizability property, we can  follow \cite{guo2020dumbo} to augment $\RBC$ by threshold signature,   resulting in   provable reliable broadcast ($\prbc$) that can   output  publicly verifiable proof attesting   $\RBC$'s termination besides    output.
%Moreover, when a $\rbc$ module delivers some transaction batch to some honest party, it also attaches a succinct proof along with the output, which attests at least $f+1$ honest parties did participate into this $\prbc$ and further proves  that at least those same parties already output in the immediately precedent $\prbc$ module, thus making another simple $\tobc$ construction that we call $\mathsf{Bolt}$-$\mathsf{RBC}$.
%Moreover, when an honest party delivers some transaction batch $\payload$ along with a succinct proof, which attests at least $f+1$ honest parties did participate into this $\tobc$, and by the pseudocode, the proof also further implies  that at least those same parties already received the same $\payload$, thus making another simple $\tobc$ construction that we call $\mathsf{Bolt}$-$\mathsf{sRBC}$.


	


\begin{figure}[h]
	\vspace{-0.15cm}
	\captionsetup{font={normalsize}}
	\begin{footnotesize}		
		\fbox{%
			\parbox{8.2cm}{				
				%, $\pending \leftarrow \emptyset$.								
				let $\id$ be the session identification of $\tobc[\id]$, $\buf$ be a FIFO queue of input, $B$ be the batch parameter,  and  $\node_\ell$ be the leader (where $\ell=(\id\mod n) +1$)
				
				\vspace{0.1cm}
				$\node_i$ initializes $s=1$, $\sigma_0=\bot$ and runs the protocol in  consecutive slot number $s$ as:
				
				\begin{itemize}[leftmargin=0.3cm]
					
					\item	\textbf{Broadcast}. if $\node_i$ is the leader $\node_\ell$,   activates $\rbc[\left \langle \id,s \right \rangle]$ with input $\payload_s \leftarrow \buf[:B]$; else activates $\rbc[\left \langle \id,s \right \rangle]$ as non-leader party
					
					\item  \textbf{Vote}.  upon $\rbc[\left \langle \id,s \right \rangle]$ returns $\payload_s$ %$(\payload_s, \prf_s)$:
					
					
					\begin{itemize}[leftmargin=0.25cm]
						
						\item  send $\vote(\id, s, \sigma_{s,i})$ to all, where $\sigma_{s,i}$ is the partial signature for $\langle \id, s,  \hash(\payload_s) \rangle$
						
						%{\color{orange}// To be precise,  that means $\vote$ message to send carries $\sigma_{s,i} \leftarrow \TSIG.\SignShare_{2f+1}(sk_i, \langle e, s,  \hash(\payload_s) \rangle)$}
						
					\end{itemize}			
					
					\item  \textbf{Commit}.  upon receiving $2f+1$  $\vote(\id, s,\sigma_{s,i})$ from distinct parties $\node_i$, where
					$\sigma_{s,i}$ is the valid partial-signature signed by $\node_i$ for $\langle \id, s, \hash(\payload_{s}) \rangle$
					%i.e., $\TSIG.\VrfyShare_{2f+1}(\langle e, s, \hash(\payload_{s}) \rangle, (i,\sigma_{s,i})) =1$
					
					\begin{itemize}[leftmargin=0.25cm]
						
						\item  output $\block$:=$ ( \id, s, \payload_{s}, \prf_{s})$, where $\prf_{s}:=\langle \hash(\payload_{s}), \sigma_{s} \rangle$ and $\sigma_{s}$ is the valid full signature that aggregates the $2f+1$ partial signatures for $\langle \id, s, \hash(\payload_{s}) \rangle$,  then let $ s\leftarrow s+1$ %{\color{orange} // To be precise, $ \sigma_{s} \leftarrow\TSIG.\Combine_{2f+1}( \langle e, s, \hash(\payload_{s}) \rangle,\{(i, \sigma_{s,i})\}_{2f+1} )$}
						
					\end{itemize}			
					
					\item \textbf{Abandon}. upon $\abandon(\id)$ is invoked then:   abort the above execution
					
				\end{itemize}
                \vspace{-0.1cm}	 
			}
		}
		\vspace{-0.3cm}
		\caption{$\tobc$ from sequential $\rbc$s ($\mathsf{Bolt}$-$\mathsf{sRBC}$). The external functions are presented in Fig. \ref{fig:external}.}% (where the  $\prbc$  \cite{guo2020dumbo} can be implemented by adapting the communication-efficient $\RBC$ in \cite{honeybadger}).}
		\label{fig:prbc}
	\end{footnotesize}
	\vspace{-0.4cm}
\end{figure}



\begin{figure}[h]
	\vspace{-0.2cm}
	\captionsetup{font={normalsize}}
	\begin{footnotesize}		
		\fbox{%
			\parbox{8.2cm}{				
				{\color{orange}// Validate $\prf_{s}$ to check whether at least $f+1$ honest parties   output the $s$-th $\block$ or can extract it (according to the next $\Extract$ function)}
				
				\textbf{external function} $\LogVerify(\id, s, \prf_{s})$:  %{\color{orange} ~~~ // {\bf external} function would not read any internal states of the $\tobc$ instance}
				
				~~~~  \hspace{1em}parse $\prf_{s}$ as $\langle h_s, \sigma_s\rangle$
				
				~~~~  \hspace{1em}return $\TSIG.\Vrfy_{2f+1}(\langle \id, s, h_s\rangle, \sigma_s)$ %($\TSIG.\Vrfy_{2f+1}(\langle e, s, h\rangle, \sigma)$ if $s > 0$) or (0 if $s \le 0$) 	
				
				\dotfill
				
				{\color{orange}// Leverage the valid $\prf_{s}$ to extract the $s$-th $\block$ from some received protocol messages (though the block was not output yet).}
				
				\textbf{external function} $\Extract(\id, s, \prf_{s})$: % {\color{orange} ~~~ // {\bf external} function would not read any internal states of the $\tobc$ instance}
				
				~~\hspace{0.8em} if $\LogVerify(\id, s, \prf_{s})=1$, then parse $\prf_{s}$ as $\langle h_s, \sigma_s\rangle$
				
				~~~~ \hspace{1em}if $\payload_{s}$ was received during executing $\tobc$ s.t. $ h_s=\hash(\payload_{s})$, then: 
				
				~~~~~~~~\hspace{2em}return $\block$:=$ ( \id, s, \payload_{s}, \prf_{s})$, where $\prf_{s}:=\langle h_s, \sigma_s\rangle$
				
				~~~~ \hspace{1em}return $\block$:=$ ( \id, s, \bot, \bot)$ 
				\vspace{-0.1cm}
			}
		}
		\vspace{-0.3cm}
		\caption{Invocable external functions for $\tobc$ instantiations}
		\label{fig:external}
	\end{footnotesize}
	\vspace{-0.2cm}
\end{figure}



\smallskip
\noindent
{\bf Analysis of the $\mathsf{Bolt}$ constructions}.
The security  analyses of $\mathsf{Bolt}$-$\mathsf{sCAST}$ and $\mathsf{Bolt}$-$\mathsf{sRBC}$ are simple by nature (cf. Appendix \ref{append:bolt}).
Their  complexities   can be easily counted as well (cf.  Appendix \ref{sec:complex}).






==> CCS 22 long-version/formulation.tex <==
%!TEX root = main.tex

% \medspace
\section{Problem Formulation}
\label{sec:def}


%\subsection{Nicknames}

%As briefly mentioned, our novel fastlane is centered around a new  broadcast primitive called notarized weak atomic broadcast ($\mathsf{nw\textnormal{-}ABC}$), and we let $\tobc$ to be its nickname;
%Our novel pace-sync  mechanism is nicknamed by $\trans$, at the core of which is a variant of binary agreement called two-consecutive-value Byzantine agreement ($\tcvba$); For the pessimistic path, %it can be reduced to any asynchronous consensus, and
%we nickname it by $\dumbo$ as instantiating it via the state-of-the-art asynchronous  protocol --- $\dumbo$.

 


 
%\subsection{Some terminology}
 
\smallskip
\noindent{\bf Transaction}. Without loss of generality, we let a transaction denoted by $\tx$ to represent a string of $|m|$ bits. %Through the paper, we will omit the detailed syntax of the transactions.

\smallskip
\noindent{\bf Block structure}. 
A block is a tuple in form of
$\block:= \langle epoch, $ $slot,  \payload,  \prf \rangle$, 
where $epoch$ and $slot$ are natural numbers, 
%$\Sigma_{-1}$ is called the notarization of the previous block,
$\payload$ is  a sequence of transactions also known as the payload.  Throughout the paper, we assume  $|\payload|=B$, %is $\mathcal{O}(B)$, 
where $B$
%$B=\Omega (\lambda n^2\log n)$ 
be the batch size parameter. The batch size can be chosen to saturate the network's available bandwidth in practice.
$\prf$ is a %threshold signature 
quorum proof
  attesting that at least $f+1$ honest parties indeed vote the $\block$ by signing it.
%the previous block have been received by at least $f+1$ honest parties.
%For presentation simplicity, we also define $\emptyset.epoch = 0$ and $\emptyset.slot = 0$.

\begin{figure}[h] 
	\vspace{-0.3cm}
	\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=7cm]{fig/block.pdf}\\
		\vspace{-0.5cm}\caption{Block and  output log due to our terminology.}	\label{fig:block}
	\end{center}
	\vspace{-0.4cm}
\end{figure}

\smallskip
\noindent{\bf Blocks as output $\out$}.
Throughout the paper, a $\out$ (or interchangeably called as $\blocks$) refers to an indexed sequence of blocks. For   $\out$ with length $L:=|\out|$, 
we might use hereunder  notations.
%\begin{itemize}
	%\item 
(1) $\out[i]$ denotes the $i$-th block in $\out$. For example, $\out[1]$ is the first block of $\out$, 
	 $\out[-1]$ is the alias of the last block in $\out$,  and $\out[-2]$ represents the  second-to-last  block in $\out$, and so forth.
%	\item $\out[i:j]$ denotes     all blocks from $\out[i]$  to $\out[j]$. Both $\out[i]$ and $\out[j]$ are inclusive for pretension simplicity.
(2)  $\out.append(\cdot)$  can append some $\block$ to   $\out$. For example, when $\out.append(\cdot)$ takes a $\block \ne \emptyset$ as input, $|\out|$  increases by one and $\out[-1]$ becomes this newly appended $\block$; when $\out.append(\cdot)$ takes a sequence of non-empty blocks $[\block_{x+1}, \dots , \block_{x+k}]$ as input, $|\out|$ would increase by $k$, and $\out[-1]=\block_{x+k}$, $\out[-2]=\block_{x+k-1}$ and so on after the operation; when $\out.append(\cdot)$ takes  an empty block   $\emptyset$ as input, the $append$ operation does nothing.
%\end{itemize}






\smallskip
\noindent{\bf Consecutive output $\out$}.
 %
 An output  $\out$ consisting of $L$ blocks is said to be consecutive if it %and a boolean function $\LogVerify$ 
 satisfies: for any two successive blocks $\out[i]$ and $\out[i+1]$ included by $\out$, either of the following two cases is satisfied: (i) 
 $\out[i].epoch = \out[i+1].epoch$ and $\out[i].slot  + 1 = \out[i+1].slot$; or (ii) $\out[i].epoch + 1 = \out[i+1].epoch $ and $\out[i+1].slot = 1$. Without loss of generality,
 we let all   $\out$s to be {\em consecutive}  throughout the paper for presentation simplicity.
 %\item For any block $\chain[i] \in \chain$, $\chain[i].\Sigma_{-1} \in \{0,1\}^{\poly(\lambda)} \cup \burro$, where $\burro$ is a special symbol, and  $\{0,1\}^{\poly(\lambda)}$ represents the output domain of $\TSIG.\Combine$ minus the symbol $\bot$.
%\begin{itemize}
	%\item For any $\block:= \langle epoch, slot,  \payload,  \prf \rangle\in\out$, %shall be anchored to an imaginary $\genesis$ block, i.e., $\out[1].h_{-1} = \hash (\genesis)$,  
	 %there satisfies $\LogVerify(\langle epoch, slot, \payload\rangle, \prf)=1$;
%	where $\genesis$ is pre-specified and $\hash \rightarrow \{0,1\}^{\lambda}$ is a cryptographic hash function;
%	\item For any two successive blocks $\out[i]$ and $\out[i+1]$ in $\out$,  $\out[i+1].h_{-1} = \hash(\out[i])$, namely, any block in $\out$ shall be anchored to its previous block;
	%\item For any $i \in [1, L]$, $\out[i].epoch \in \N$ and $\out[i].slot \in \N$, i.e., 
	%the  $epoch$ and  $slot$ must be integers greater than 0;%or equal to 1;
	%\item For any two successive blocks $\out[i]$ and $\out[i+1]$ included by $\out$, either of the following two cases shall be satisfied: (i) $\out[i].epoch = \out[i+1].epoch$ and $\out[i].slot  + 1 = \out[i+1].slot$; or (ii) $\out[i].epoch + 1 = \out[i+1].epoch $ and $\out[i+1].slot = 1$.
	%\item For any block $\chain[i] \in \chain$, $\chain[i].\Sigma_{-1} \in \{0,1\}^{\poly(\lambda)} \cup \burro$, where $\burro$ is a special symbol, and  $\{0,1\}^{\poly(\lambda)}$ represents the output domain of $\TSIG.\Combine$ minus the symbol $\bot$.
%\end{itemize}

%\medskip
%\noindent{\bf Other terms}. We might use the following terms in some parts of the remaining paper:
%\begin{itemize}
%	\item $\out[-1]$ is the last block in $\out$ and is also called $\pending$ block.
%	\item $\out[-2]$ is the 2nd to the last block in $\out$ and is also called $1$-$\notarized$ block.	
%	\item $\out[-3]$ is the 3rd to the last block in $\out$  and is also known  $2$-$\notarized$ block.
%	\item $\out[:-4]$ is called the $\finalized$ part of $\out$.
%\end{itemize}




%\section{Problem}

\subsection{Modeling the system and threats}
We consider the  standard  asynchronous message-passing  system   with trusted setup,
%It consists of $n$ parties $\{\node_i\}_{i \in [n]}$ interconnected via asynchronous point-to-point (p2p) channels, where $n \in \N$ represents the number of parties and $[n]$ is short for $\{1,\cdots,n\}$. %The adversary can fully control all p2p channels and   statically corrupt up to $f$ parties.
%
which can be detailed as follows.

%\begin{itemize}
%	\item {\bf Public key infrastructure (PKI).} There are $n$ designated parties, each of which has a unique identity (i.e. $\node_1$ through $\node_n$) that is known by everyone. Moreover, through existing PKI, each party $\node_i$ % \in \{\node_i\}_{i \in [n]}$
	% is bounded to a unique secret-public key pair 
	%of digital signature scheme $\SIG$. Thus, for each $\node_i$, it can use its secret key to generate a digital signature $\sigma$ for the message $m$ (e.g., denoted by  $\sigma \leftarrow \SIG.\Sign(sk_i, m)$), and  anyone can use  $\node_i$'s public key to verify whether $\sigma$ is deemed as a valid signature generated by $\node_i$ for the message $m$ (e.g., denoted by $\{0, 1\} \leftarrow  \SIG.\Vrfy(pk_i, m,\sigma)$). 
	
%	\item {\bf Other trusted setups.}
	%Besides the already-established PKI, we assume all involved threshold cryptosystems such as $\TSIG$ and $\TPKE$ have been properly set up, such that all participating parties can get and only get their own secret keys in addition to public keys. The above setups can be done either via a trusted dealer, or through some distrusted key generation protocols (that might rely on timing assumptions merely during the setup phase \cite{boldyreva2003threshold}). In particular, we require the establishments of $(2f+1,n)$-$\TSIG$ scheme, $(f+1, n)$-$\TPKE$ scheme, and $(f+1, n)$-$\coin$ scheme, where $f=\lfloor n/3 \rfloor$.
%	\footnote{Remark that it is also fine to use $(2f+1, n)$-$\coin$ scheme instead of $(f+1, n)$-$\coin$ scheme through the paper.}

	\smallskip
	 \noindent{\bf  Known identities and trusted setup}. There are $n$ designated parties, each of which has a unique identity (i.e., $\node_1$ through $\node_n$)  known by everyone else. 
	%Moreover, through an existing PKI, each party $\node_i$ % \in \{\node_i\}_{i \in [n]}$
	%is bounded to a unique secret-public key pair 
	%of a digital signature scheme $\SIG$. %Thus, for each $\node_i$, it can use its secret key to generate a digital signature $\sigma$ for the message $m$ (e.g., denoted by  $\sigma \leftarrow \SIG.\Sign(sk_i, m)$), and  anyone can use  $\node_i$'s public key to verify whether $\sigma$ is deemed as a valid signature generated by $\node_i$ for the message $m$ (e.g., denoted by $\{0, 1\} \leftarrow  \SIG.\Vrfy(pk_i, m,\sigma)$). 
	%	\item {\bf Other trusted setups.}
	All involved threshold cryptosystems   are properly set up, so all   parties  can get and only get their own secret keys in addition to   relevant public keys. The setup   can be done by  a trusted dealer or distributed key generation   \cite{pedersen1991threshold,gennaro1999secure,kate2009distributed,gao2021efficient,renavss,kokoris2020asynchronous,abraham2021reaching,das2022practical}. % (that might rely on timing assumptions merely during the setup phase \cite{boldyreva2003threshold}). In particular, we require the establishments of $(2f+1,n)$-$\TSIG$ scheme, $(f+1, n)$-$\TPKE$ scheme, and 	$(f+1, n)$-$\coin$ scheme, where $f=\lfloor n/3 \rfloor$.
	%\footnote{Remark that it is also fine to use $(2f+1, n)$-$\coin$ scheme instead of $(f+1, n)$-$\coin$ scheme through the paper.}
	

\smallskip
	 \noindent{\bf  Byzantine corruptions}.  %The adversary can fully control $f$   out of  $n$ parties. In addition, we restrict to static corruptions, namely, 
	The adversary can  choose up to $f$    parties to   fully control   before the protocol starts. Our instantiations focus on   static corruptions, which is same to all recent {\em practical} asynchronous atomic broadcast \cite{honeybadger,beat,guo2020dumbo,guo2022speeding,yang2021dispersedledger}. %\rev{EPIC \cite{liu2020epic}}. We   also remark that since our BDT framework is generic, adaptive security is easy to obtain if we instantiate building blocks with adaptively secure ones, just that their efficiency is not favorable \rev{(e.g., EPIC  has  a  degraded throughput less than half of its static counterpart for moderate  scales $\sim$50 nodes)}.  
	Also, no asynchronous BFT can tolerate more than $f = \lfloor (n-1)/3 \rfloor$ Byzantine corruptions.
	Through   the paper, we stick with this optimal resilience. %Therefore,   $f+1$ and $n-2f$ are interchangeable, so are $2f+1$ and $n-f$.
	%, and we are essentially targeting the optimal resilience (in case of static corruptions).
	%After all, recall that the adversary can arbitrarily schedule message deliveries sent over the network.
	%Once the protocol begins, the adversary cannot adaptively corrupt any honest parties, even if she has not controlled up to $\lfloor n/3 \rfloor$.
	%Also remark that static Byzantine fault can simulate adaptive crash fault, indicating BFT in such static corruption setting still subjects to FLP impossibility and must be randomized.
	
	\smallskip
	 \noindent{\bf  Fully-meshed reliable asynchronous network}.
	There exists a reliable asynchronous  peer-to-peer channel between any two   parties.
	%though the adversary must be consulted to approve message deliveries over any p2p channels. 
	%
	%Explicitly speaking, 
The adversary can arbitrarily delay or reorder messages, % deliveries,
	 but cannot drop or modify   messages sent among honest parties. %Such reliable asynchronous channels can be implemented via TCP 
	 
	
	\smallskip
	 \noindent{\bf  Computationally-bounded adversary}.
	We  consider  computationally bounded adversary that can   perform  some  probabilistic computing steps
	bounded by   polynomials	in the number of message bits generated by honest parties, which is standard cryptographic practice in the asynchronous network.	
	
 
	\smallskip
	 \noindent{\bf  Adversary-controlling local ``time''}. 
	%Remark that 
	It is impossible to implement  global time   in the   asynchronous model. Nevertheless,  we do not require any global wall-clock for securities.
	Same to  \cite{cachin2002asynchronous,kursawe05}, it is still feasible to  let each party keep an adversary-controlling local ``clock'' that elapses at the speed of the actual network delay $\delta$:
	each party sends a  ``tick'' message      to itself via the adversary-controlling network, then whenever  receiving a ``tick'', it increases its local ``time'' by one and resends a new ``tick'' to itself via the adversary.	
	Using the adversary-controlling  ``clock'', each party can     maintain a  timeout mechanism, for example,	let $timer(\tau).start()$ to  denote that a local timer is initialized and  will ``expire''  after $\tau$ clock ticks, 	and let $timer(\tau).restart()$  denote to  reset the timer.	
	%This ``timeout'' notion     shows that the timeout parameter $\tau$ used in our optimistic fastlane is essentially a function of the actual network delay instead of the  upper bound of delay.
	
	%\item  {\em Miscellany.} In addition, all system parameters, such as $n$, are (probably unfixed) polynomials in   security parameter $\lambda$ due to  the standard cryptographic practice \cite{cachin01,ittai19,lu2020dumbo}.
	
%\end{itemize}



%Clearly, the above model is essentially the well-accepted standard asynchronous, static corruption model with a few moderate cryptographic assumptions \cite{ittai19, honeybadger, cachin01}.


\subsection{Security goal: async. atomic broadcast}% $\mathsf{ABC}$}
 
%\noindent
%{\bf  Asynchronous atomic broadcast.}
Our  primary goal is to develop an asynchronous atomic broadcast protocol defined as follows
to attain high robustness against   unstable or even hostile   network environment.
%
%In particular,  
%the correct parties can continuously receive transactions as their inputs, and 
%Even if we relax the requirement for high performance in benign cases, 
%That means, the proposed   protocol  shall    satisfy the following security properties of  atomic broadcast. %, such that the payloads of these blocks can solicit and include their input transactions. 
%In details, the atomic broadcast can be defined as: %(for block-wise setting):
%(which is slightly tailored for the block-wise setting and is equivalent to the conventional notion \cite{cachin01}):


\begin{definition}\label{def:abc}
	In {\bf atomic broadcast} ($\mathsf{ABC}$),  %with an identification $\id$, %:=(e, h_{\genesis})$ 
	%It is joined by $n$ parties that continuously receive a sequence of transactions as input, and each correct participating node might output a sequence of $\blocks$. 
	each party is with  an implicit  queue  of input transactions (i.e., the input backlog)  and  outputs a  $\out$ of blocks.
	%
	Besides the   syntax, the $\mathsf{ABC}$ protocol shall  satisfy the  following properties with all but negligible probability:
	\begin{itemize}[leftmargin=0.5cm]
		\item {\em Total-order}. If an honest party outputs a $\out$, and another honest   party outputs another $\out'$, then $\out[i]=\out'[i]$ for every $i$ that $1 \le i \le \min\{|\out|,|\out'|\}$.
		
		\item {\em Agreement}. If an honest party adds a $\block$ to its $\out$,   all honest parties would eventually add the   $\block$ to their $\out$s.
		
	
		%\item {\em Censorship-resilience}. If $n-f$ honest parties take a transaction $\tx$ as input,  $\tx$ would eventually included by   an honest party's $\out$. Remark that the censorship-resilience can also be translated to a couple of mutually complement notions called validity and fairness in \cite{cachin01,kursawe05}, which essentially corresponds to   liveness.
		\item {\em Liveness} (adapted from \cite{cachin01}). If all honest parties input a transaction $\tx$,  
		$\tx$ would    output   within some   asynchronous rounds (bounded by   polynomials in   security parameters). 
		

		%This directly implies the eventual output of the transaction $\tx$.
		
		
		 %Also note that in the block-wise setting,   $\tx$ is outputted in the form of an element of a block's payload. 
	\end{itemize}
\end{definition}

 
\noindent
{\em Remarks on the definition of $\mathsf{ABC}$.} 	
Throughout the paper, 	we  let safety   refer to the union of total-order and agreement. Besides,
we   insist on the   liveness notion from \cite{cachin01} to ensure  that each input transaction can output reasonably quickly instead of eventually. 
%Such strong liveness  is needed for the end security goal of guaranteeing   fast confirmation of input transactions even in  the worst adversary-influencing case, i.e., it resolves the denial-of-service attacks.
This reasonable aim can   separate  some   studies that have {\em exponentially} large confirmation latency \cite{ben1983another}.
%This is  quintessential for the next reasons:   (i) it highlights the end goal of liveness, namely, to ensure the fast confirmation of input transactions even in   worst cases; for example, it    separates this reasonable aim from some studies having  exponentially large confirmation latency \cite{ben1983another}; 
%(ii) the protocol must have polynomial-bounded execution rounds to bound the computing power of   adversary in our model, otherwise  the underlying cryptographic primitives are potentially insecure  \cite{cachin01,ittai19}.
%and  was also known as censorship-resilience in HoneyBadger BFT \cite{honeybadger}. % and  once was interpreted as a couple of mutually complement notions called validity and fairness in \cite{cachin01,kursawe05}.	
Moreover, the protocol must terminate in polynomial number of   rounds to restrict the computing steps of   adversary in the computationally-secure model  \cite{cachin01,ittai19,pass2017sleepy}, otherwise      cryptographic primitives are potentially insecure.


\subsection{Performance  metrics and preliminaries}


%\noindent
%{\bf Performance  metrics.}
%\subsection{Performance  metrics}
We are particularly interested in   {\em practical} asynchronous protocols, and therefore, %focus on a few standard performance metrics about {\em block-wise} atomic broadcast:
%\begin{itemize}
% \item {\bf Block-quality.} Suppose the input transaction buffers of all honest parties are sufficiently full $\Omega(n,\lambda)$ and their sizes dominate both the system size $n$ and the security parameter $\lambda$ (e.g. hash length and/or signature length), we require that each delivered block must include a constant (or nearly constant) number  of distinct transactions sent from honest parties on average. Intuitively, the requirement of block-quality ensures many honest parties deliver transactions that are actually chosen from their input buffers.	 
% Remark that this block-quality requirement was implicitly proposed and realized in \cite{honeybadger}, which we believe is needed to rule out an asynchronous adversary who intends to degrade the actual throughput by creating ``bogus'' blocks.
% \footnote{For many (partial-)asynchronous protocols, what is both intriguing and unsatisfying is that: if many of them (e.g. \cite{hotstuff,libra}) are trivially executing in asynchronous network without particular enhancements, a dominating number of outputs (if there are any) could be ``bogus'' proposed by only corrupted parties. 
%Imagine a simple attack on \cite{hotstuff,libra}:	whenever an honest leader is designated to a ``view'', the  asynchronous network adversary delays all messages  to drive the protocol skip into the next view; nevertheless while the adversary  controls a leader, she prepares some ``junk'' messages to let the quorum agree.
%As such, even if these (partial-)asynchronous protocols make progress without grinding to halt, their liveness can be dramatically harmed, as the actual effective throughput becomes rare. Clearly, if our optimistic path suffers from the similar vulnerability, the average throughput can be significantly dropped by the asynchronous adversary.}
%\end{itemize}
%\noindent Rooting from the above block-quality, 
 consider the following critical efficiency metrics:

\begin{itemize}[leftmargin=0.5cm]
	\item {\em Communication complexity}. We primarily focus on the (average) bits of all messages associated to output each block. 
	Because the communicated bits per block essentially reflects the (amortized) communication per delivered transaction, % (a.k.a. the efficiency defined in \cite{honeybadger}), 
	in particular when   each block   includes   $\mathcal{O}(B)$-sized transactions, where  $B$ is a specified batch-size  parameter.%  specified for the block payload size.% to specify the payload size in each block.
	%Therefore we adopt communication complexity per   block as an important notion to characterize the maximum system throughput.
	
	%\item {\em Each party's bandwidth usage}. This is similar to per-block communication complexity, but it does not count the overall message bits that are exchanged for generating each block. Instead, this metric counts a certain party's bandwidth usage (including both incoming and outgoing messages) amortized for each output block.
	
	\item {\em Message complexity}. This characterizes     the   number of messages exchanged among  honest parties to produce a block.
	%sending/receiving messages over communication channels   and is one of the important factors related to system scalability.
	%communication channels that need to be built/maintained. 
	%It normally relates to system scalable.
	
	
	\item {\em Asynchronous  round complexity}. 
	The eventual delivery in   asynchronous network    causes   the protocol execution   independent to ``real time''.
	Nevertheless, it is still needed to characterize the   running time, and 
	a standard way  to do so  is    counting  asynchronous ``rounds'' as in \cite{canetti1993fast,cachin01}.
	%: for each message the adversary  assigns a virtual round number $r$, subject to the condition that any $(r-1)$-th round messages between any two correct parties must be delivered before any $(r+1)$-th round message is sent \cite{canetti1993fast}.
	%
	%so it becomes straightforward  to measure the running time %any transaction's confirmation latency    
	%by . 
	
	%Following this rationale, we might need our designs to meet the following requirements in order to realize highly responsive atomic broadcast: (i) the  ``time'' of generating each block  shall be on average $\bigO(1)$   rounds and (ii) any transaction lying in the honest parties' input backlogs would  output in a polynomial number of rounds.
	
	
	
	%Note that communication complexity per output block shall be asymptotically same to , which essentially characterizes the maximum system throughput.
\end{itemize}

%\noindent Last but not least, we consider the running time of outputting any transactions in standard asynchronous, static corruption model (with overwhelming latency), which is an important indicator to characterize the robustness of liveness \cite{honeybadger,cachin01}. For example, finite confirmation delay indeed corresponds sorta robust liveness/censorship-resistance notion. In details,  
%\begin{itemize}

%\item {\bf Transaction delay.}
%Suppose the adversary passes a transaction $\tx$
%to all honest parties'   input buffers. Say   $T$ represents the
%total number of transactions that are input to any honest party's input buffer before $\tx$ but not delivered yet. The so-called transaction delay becomes the running time before $\tx$ is output by every honest party with overwhelming probability, which is
%a function of $T$ and security parameters \cite{attiya1994bounds}. This notion has been recognized as a key factor to characterize {\em the responsiveness of liveness} \cite{pass2017hybrid, thunderella}.
%We emphasize on a (nearly) linear function w.r.t. $T$  \cite{honeybadger}, for the sake of highly responsive liveness.
%\end{itemize}

%Note that the above performance metrics can be leveraged to measure whether a hybrid design rea

%\subsection{Preliminaries}

\noindent{\bf Cryptographic abstractions}. $\hash$ denotes a collision-resistant hash function. 
$\TSIG$ and $\TPKE$ denote threshold signature  and  threshold encryption, respectively. Established $\TSIG$ is a tuple  of algorithms $(\SignShare_t, \VrfyShare_t,\Combine_t, \Vrfy_t)$,  and throughout the paper, we call the signature share output from $\SignShare_t$ the {\em partial signature}, and   call the output of $\Combine_t$  the {\em full signature}. Established $\TPKE$ consists  three algorithms $(\Enc_t, \DecShare_t, \Dec_t)$. In all notations, the subscript $t$ represents the threshold, cf. some classic literature such as \cite{honeybadger}. The cryptographic security parameter is denoted by $\lambda$,   capturing the bit-length of signatures and hashes.



\medskip
 \noindent
{\bf Building blocks}. We might use the following asynchronous broadcast/consensus protocols in the black-box manner.

\vspace{-0.1cm}
\begin{definition}{\bf Reliable broadcast ($\mathsf{RBC}$)} has a designated sender who aims to send its input to all parties,  %and an identifier $\id$ 
	%is a broadcast   
	and satisfies the  next properties  except with negligible probability:
	%is a protocol running among a set of $n$ nodes %\cite{bracha1987asynchronous} in which there is a node called sender whose aim is to broadcast a value to all the other nodes. More formally, an $\mathsf{RBC}$ protocol satisfies the following properties:
	%
	%\begin{itemize}
		%	
		%\item 
		(i) {\em Validity}. If the sender is honest and inputs $ v $, then all honest parties output $ v $;
		%	
		%\item 
	    (ii) {\em Agreement}. The outputs of any two honest parties are same;
		%
		%\item 
		(iii) {\em Totality}. If an honest party outputs $ v $, then all honest parties output $ v $.
	%\end{itemize}
\end{definition}

\vspace{-0.2cm}
\begin{definition}{\bf Asynchronous binary  Byzantine agreement ($\ABA$)}  \cite{MMR15,cachin00,canetti1993fast}  has a syntax that  each party inputs and outputs a single bit $b$, where $b$ ranges over $\{0,1\}$, 
% input, and their goal is to output a common bit
and  
%In an asynchronous binary agreement ,. In particular, a protocol $\ABA$ running among $n$ parties with identification $\id$ is said to be asynchronous binary agreement, if it 
shall guarantee the following properties except with negligible probability:
%\begin{itemize}
	%\item
	(i) {\em Validity}. If any honest party outputs $ b $, then at least one honest party takes $ b $  as input;	
	%\item
	(ii) {\em Agreement}. The outputs of any two honest parties are same;
	%\item 
	(iii) {\em Termination}. If all honest parties activate the protocol with taking a bit as input, then all honest parties would output a bit in the protocol.
%\end{itemize}
\end{definition}

%\smallskip



\vspace{-0.2cm}
\begin{definition}{\bf Asynchronous common subset ($\acs$)} \cite{benor} has a syntax that 
%We follow the elegant prior art to let the pessimistic path center around asynchronous common subset  ($\acs$). 
%In the  $\acs$ protocol 
each party input a value and output a set of values, where $n$ parties participate in this protocol and up to $f$  corruption parties.
%
It      satisfies   the next properties   except with negligible probability:
%\begin{itemize}
	%\item 
	(i) {\em Validity}. The output set $\bf S$ of an honest party     contains the inputs of at least $n - 2f$ honest parties;
	%\item 
	(ii) {\em Agreement}. The outputs of any two honest parties are same;
	%\item 
	(iii) {\em Termination}. If all honest parties activate the protocol,  then all honest parties would output.
%\end{itemize}
\end{definition}


%\noindent\rev{{Consistent broadcast} ($\mathsf{CBC}$) is similar to $\mathsf{RBC}$, but it does not provide {\em Totality}.}



\ignore{

\smallskip
\begin{definition}  {\bf Strong Provable  reliable broadcast ($\prbc$)}   with   a designated sender, a predicate  $\prbc.\Verify$  and an identifier $\id$ is a broadcast   that satisfies the  next properties  (in presence of $f$       corruptions) except with negligible probability:

\begin{itemize}
	\item {\em Validity}. If all honest parties invoke $\prbc[\id]$ and the sender is honest and inputs a message $ m $, all honest parties  will output $m$   with some string $\sigma$  s.t. $\prbc.\Verify(\id, \sigma)=1$.
	
	\item {\em Agreement}. If two honest parties output $ m $ and $ m' $  in $\prbc[\id]$ respectively, then  $ m = m' $.
	
	\item {\em Totality}. If any (probably malicious) party outputs $ m $ and $\sigma$ in $\prbc[\id]$ s.t. $\prbc.\Verify(\id, \sigma)=1$, then all honest parties eventually output some value attached with a proof $\sigma$  s.t. $\prbc.\Verify(\id, \sigma)=1$ in $\prbc[\id]$.
	
	\item {\em Unforgeability}.  If $f+1$ or more honest parties do not activate $\prbc[\id]$, it computationally infeasible for any   party to produce a string $\sigma$ 
	s.t. $\prbc.\Verify(\id, \sigma)=1$.
\end{itemize}
\end{definition}
 
We remark that strong $\prbc$ adds a unforgeability to the $\prbc$ introduced in \cite{guo2020dumbo} to ensure enough parties have activated  $\prbc[\id]$ when seeing the proof, it can be easily obtained from $\RBC$ by adding one round of threshold signature.

}






%\noindent{\bf Other notations}. $\langle x, y \rangle$   denotes a string concatenating  two strings $x$ and $y$. Any message between two parties is in the form of $\textsc{MsgType}(\id, \cdot, \cdot, \cdots)$, where $\textsc{MsgType}$ specifies the message type and  $\id$  is the identifier tagging the protocol instance. We might omit the $\id$ field in messages for brevity if there is a clear context, and also let ``A {multicasts} $\textsc{Msg}$''  denote that a party A sends a message $\textsc{Msg}$ to all parties, and let ``B aborts''  denote that a party B quits the protocol execution. The pseudocode of our protocol   follows the conventional way to describe asynchronous protocols \cite{cachin01,ittai19,lu2020dumbo}: we let ``{\em wait for}'' to represent that the protocol is blocking until a certain event; sometimes, we omit an implicit ``{\em wait for}'' handler for   the incoming messages and use ``{\em upon receiving}'' to describe how to process  an applicable message; ``{\em multicast}'' means to send a message to all parties; ``{\em output}'' means to return some value without halt; ``{\em return W}'' means to output {\em W} and then halt; Moreover, $\Pi[\id]$ refers to an instance of some protocol $\Pi$ with an identifier $\id$, and $y\leftarrow\Pi[\id](x)$ means to invoke $\Pi[\id]$ on input $x$ and wait for its  output $y$.
%





==> CCS 22 long-version/fsacs.tex <==
%!TEX root=main.tex

\section{Fast Asynchronous Common Subset}



\subsection{Definition of asynchronous common subset}


In particular, we follow the elegant prior art of HoneyBadger BFT to let the pessimistic path center around asynchronous common subset  ($\acs$), which can be defined hereafter.

\begin{definition}{\bf asynchronous common subset  ($\acs$).}
	An asynchronous common subset $\acs$ with identification $\id$ is denoted by $\acs[\id]$, and satisfies the following properties except with negligible probability:
	\begin{itemize}
		\item {\bf Validity}. If a correct node outputs a set $\bf v$, then $|{\bf v}| \ge n - f$ and ${\bf v}$ contains the inputs of at least $n - 2f$ correct nodes.
		\item {\bf Agreement}. If a correct node output a set $\bf v$, then every node outputs the same set $\bf v$.
		\item {\bf Termination}. If $n-f$ correct nodes receive an input, then every correct node delivers an output.
	\end{itemize}
\end{definition}

{\em Remark}. We emphasize that this paper will not focus on designing new concrete construction of asynchronous common subset to improve the pessimistic path, as it actually targets to design an efficient way to grafting a super-efficient optimistic path into existing fully asynchronous BFT protocols. We might adopt the best performing constructions of $\acs$ so far due to \cite{honeybadger}. More importantly, due to our modular  protocol design and analysis, any $\acs$ construction (e.g. from MVBA \cite{cachin01}) can be adopted.



\subsection{Constructing fast asynchronous common subset ($\fACS$)}

Observation of the HoneybadgerBFT, we notice that the protocol concurrently invoke $ N $ instances of RBC and $N$ instance of ABA, it dominates the message complexity to $\mathcal{O}(N^3)$ for each committed ACS. The heavy message complexity restricts the performance of latency significantly. 

Hence, we hope to improve the message complexity. We present a new $\acs$, called $\fACS$. It's a trade-off compare with HoneybadgerBFT's $\acs$, since it have
message complexity to $\mathcal{O}(CN^2)$ and the communication complexity to $\mathcal{O}(CN^2|m|)$; however, the HoneybadgerBFT's $\acs$ have message complexity to $\mathcal{O}(N^3)$ and the communication complexity to $\mathcal{O}(N^2|m|)$. The $\fACS$ protocol algorithm is described in Algorithm \ref{alg:fsACS} with $f<N/a$ byzantine failures, suppose $a \geqslant 3$ and $C$ are constants. In our main protocol, it still will invoke the sub-protocols RBC, leader-election and ABA, but it concurrently runs only $ C $ instances of RBC and $ C $ instances of ABA per epoch (instead of $N$). 

 In the $\fACS$, the leader-election sub-protocol is a important tool. We choose a small number $C$ because the size of leaders determines the costs of our protocols, however it also affects the security. We need to ensure that there will be at least one honest node in the leader set, otherwise the \textit{termination} of the $\fACS$ is not guaranteed.  In the $\fACS$, We make sure that the probability of at least one honest node in $C$ with overwhelming probability regarding security parameters.

Generally speaking, trivially setting $ C $ to $ f+1 $ is OK. If the number of Byzantine node is very small, or when the system scale is small, we can set $ C $ to $ f+1 $ to ensure safety. However it is not always the best solution. In large-scale system, it is sufficient to ensure safety choosing a much smaller $C$ via random algorithm when the number of Byzantine node is linear with the $N$.

Hence, we consider if the number of Byzantine node is independent of the $N$ (when $f$ is chosen to be a very small number), we will choose the simple round-robin leader election algorithm. If the number of Byzantine node is linear with the $N$, we will choose the random leader election algorithm to select $C$ leaders. 

As illustrated in Figure 3, the $\fACS$ protocol can be decomposed in four logical phases. The detailed protocol process as follows:
\begin{itemize}
	\item \textbf{First}, for consecutive epoch $i$, all nodes invoke leader-election protocol to elect $C$ leader;
	
	\item \textbf{Second}, all nodes send their message $\{V_i,\sigma_i\}$ to all leader;
	
	\item \textbf{Third}, for each leader $P_j$: Upon delivery $N-f$ valid message from distinct $N-f$ node, then collect these messages into a set $S$, the broadcast the set $S$ with RBC$_j$ protocol;
	
	\item \textbf{Fourth}, for any node, upon delivery $S_j$ from RBC$_j$, if input has not yet been provided to ABA$_j$, then provide input 1 to ABA$_j$; if upon delivery value 1 from any ABA$_{j}$ instance, then input 0 to other ABA instances if input has not yet been provided.
	
	\item \textbf{Fifth}, Upon all $C$ ABA instance have completed, then if the ABA of $P_{j}$ output 1, then put the $S_j$ add into the set $S$. Finally output $\cup _{V \in S}V$. 
	
\end{itemize}



\begin{figure}[H]
	\begin{footnotesize}
	\centering
	\label{alg:fsACS}
	\fbox{%
		\parbox{\linewidth}{%
			\begin{center}
				{\bf the $\fACS$ algorithm (for party $ P_{i} $) in consecutive epoch $ r $} 
			\end{center}	
			\begin{flushleft}
					\item Let RBC$ _{j} $ refer to an instance of the reliable broadcast protocol of the block-proposing stage where $ P_{j} $ is the leader.
				
				\item Let ABA$ _{j} $ refer to an instance of the asynchronous binary byzantine protocol correspond to the leader $ P_{j} $. Let $\{ABA_i\}_C$ refer to $ C $ BA instances.
				
				\begin{itemize}[noitemsep,topsep=0pt]
					\item Invoke leader-election protocol to elect $C$ leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$; {\color{cyan} // Leader election}
			
					\item Send message $\{V_i,\sigma_i\}$ to all leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$; {\color{cyan} // All node broadcast}
						
						
					\item if $P_i$ is leader then {\color{cyan} // Leader broadcast}
					\begin{itemize}[noitemsep,topsep=0pt]
							\item 	Upon delivery $N-f$ valid message $\{V_j,\sigma_j\}$ from distinct $N-f$ node $P_j$; then
							\item   Input the set $S_i=\{\{V^{'}_1,\sigma_{1}^{'}\},\{V^{'}_2,\sigma_{2}^{'}\},\cdots,\{V^{'}_{N-f},\sigma_{N-f}^{'}\}\}$ to RBC$_i$ protocol;						
					\end{itemize} 
						
					\item Upon delivery $S_j$ from RBC$_j$, if input has not yet been provided to ABA$_j$, then provide input 1 to ABA$_j$;
						
					\item Upon delivery of value 1 from any ABA instance, then input 0 to other ABA instances if input has not yet been provided.
						
					\item Upon  all C ABA instances have completed, then if the ABA of $P_{j}^{'}$ output 1, where $P_{j}^{'}$ is a leader, then put the $S_j$ add into the set $S$;				
					
		    		\item Return $\cup _{V \in S}V$.  	
						
					\end{itemize} 
				
			\end{flushleft}
		}
	}
	\caption{$\fACS$}
	\end{footnotesize}
\end{figure}


\begin{comment}

\begin{breakablealgorithm}
	\caption{the $\fACS$ algorithm (for party $ P_{i} $) in consecutive epoch $ r $}
	\label{alg:fsACS}
	\begin{algorithmic}[1] 
		

		\State Let RBC$ _{j} $ refer to an instance of the reliable broadcast protocol of the block-proposing stage where $ P_{j} $ is the leader.
		
		\State Let ABA$ _{j} $ refer to an instance of the asynchronous binary byzantine protocol correspond to the leader $ P_{j} $. Let $\{ABA_i\}_C$ refer to $ C $ BA instances.
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	-----------------Step1: Leader election-----------------}\vspace*{0.1 cm}
		\end{center}
		
		\State \textbf{Invoke} leader-election protocol to elect $C$ leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$;
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{------------------Step2: All node Broadcast------------------}\vspace*{0.1 cm}
		\end{center}
		
		\State \textbf{Send} message $\{V_i,\sigma_i\}$ to all leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$;
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{------------------Step3: Leader Broadcast------------------}\vspace*{0.1 cm}
		\end{center}
		
		\If{$P_i$ is leader}
		
		\State \textbf{Upon} delivery $N-f$ valid message $\{V_j,\sigma_j\}$ from distinct $N-f$ node $P_j$;
		
		\State \textbf{then} input the set $S_i=\{\{V^{'}_1,\sigma_{1}^{'}\},\{V^{'}_2,\sigma_{2}^{'}\},\cdots,\{V^{'}_{N-f},\sigma_{N-f}^{'}\}\}$ to RBC$_i$ protocol;
		
		\EndIf
		
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{---------------------Step4: Decision---------------------}\vspace*{0.1 cm}
		\end{center}
		
		\State \textbf{Upon} delivery $S_j$ from RBC$_j$, if input has not yet been provided to ABA$_j$, then provide input 1 to ABA$_j$;
		
		\State \textbf{Upon} delivery of value 1 from any ABA instance, then input 0 to other ABA instances if input has not yet been provided.
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{-----------------------Step5: Output--------------------}\vspace*{0.1 cm}
		\end{center}
		
		\State\textbf{Upon} all C ABA instances have completed, then if the ABA of $P_{j}^{'}$ output 1, where $P_{j}^{'}$ is a leader, then put the $S_j$ add into the set $S$;
		
		
		\State\textbf{Finally} output $\cup _{V \in S}V$.  
		
	\end{algorithmic}
\end{breakablealgorithm}

\end{comment}

\subsection{Analyzing $\fACS$ construction}

In here, we prove the construct of the $\fACS$ satisfies all properties of $\acs$ with overwhelming probability regarding security parameters.

\begin{lemma}
	\emph	{\bf Termination}. If $n-f$ correct nodes receive an input, then every correct node delivers an output.
\end{lemma}	

\begin{proof}

According election-leader protocol, after invoke the protocl, all honest can terminate and receive the same leader set. Since $n-f$ correct nodes receive an input, so the leaders can receiving at least $n-f$ valid message. Besides, there are at least one honest node in the leader set, so at least one ABA instance can finished, in this case, all node will have a input to all instance, according to the termination properties of ABA, all node can completed the all ABA instance, hence, according to the algorithm \ref{alg:fsACS}, every correct node delivers an output.


	$\hfill\blacksquare$ 
\end{proof}

\begin{lemma}
	\emph	{\bf Agreement}. If a correct node output a set $\bf v$, then every node outputs the same set $\bf v$.
\end{lemma}	

\begin{proof}
	 Suppose two correct node $P_i$ and $P_j$ output different $\bf v$ and $\bf v^{'}$, respectively. Then according to the algorithm \ref{alg:fsACS}, $P_i$ and $P_j$ must received different value from a same ABA instance. But it's contradiction with the agreement properties of ABA. Hence, every node outputs the same set $\bf v$.

	
	$\hfill\blacksquare$ 
\end{proof}

\begin{lemma}
	\emph{\bf Validity}. If a correct node outputs a set $\bf v$, then $|{\bf v}| \ge n - f$ and ${\bf v}$ contains the inputs of at least $n - 2f$ correct nodes.
\end{lemma}	

\begin{proof}
	Suppose a correct node outputs a set $\bf v$, according to the algorithm \ref{alg:fsACS}, It's clear that $|{\bf v}| \ge n - f$. Besides, here at most have $f$ byzantine node, hence, it also clear that ${\bf v}$ contains the inputs of at least $n - 2f$ correct nodes.
	
	$\hfill\blacksquare$ 
\end{proof}




\subsection{Cost of the $\fACS$}

In this part, we analysis the message complexity and communication complexity of $\fACS$ protocol. From section 2 we know: The RBC messages complexity is $\mathcal{O}(n^2)$ and communication complexity is $\mathcal{O}(n|m|)$. The ABA messages complexity is $\mathcal{O}(N^2)$ and communication complexity is $\mathcal{O}(n^2)$.

According to the pseudocode of algorithm \ref{alg:fsACS}, the message exchange appears in the next seven place:	
\begin{itemize}		
	\item \textbf{1:} all node participate the leader-election instance;
	\item \textbf{2:} all node multicast message to all leader;
	\item \textbf{3:} the leaders boardcast messages to all node with RBC;
	\item \textbf{4:} all node participate the $C$ ABA instance;

\end{itemize}


\noindent \textbf{The $\fACS$ message complexity:} in place 1, the messages complexity is $\mathcal{O}(n^2)$, in place 2, the messages complexity is $\mathcal{O}(Cn)$, in place 3, the messages complexity is $\mathcal{O}(Cn^2)$. in place 4, the messages complexity is $\mathcal{O}(Cn^2)$. Hence, the $\fACS$ messages complexity is $\mathcal{O}(Cn^2)$.
\vspace{0.2cm}

\noindent \textbf{The $\fACS$ communication complexity:} in place 1, the communication complexity is $\mathcal{O}(Kn^2)$; in place 2, the communication complexity is $n*C*\mathcal{O}(|m|+K)$=$\mathcal{O}(Cn(|m|+K))$; in place 3, the communication complexity is $C*n*\mathcal{O}(n(|m|+K))$=$\mathcal{O}(Cn^2(|m|+K))$; in place 4, the communication complexity is $C\mathcal{O}(n^2)$=$\mathcal{O}(Cn^2)$. Hence, the $\fACS$ communication complexity is $\mathcal{O}(Kn^2)$+$\mathcal{O}(Cn(|m|+K))$+$\mathcal{O}(Cn^2(|m|+K))$+$\mathcal{O}(Cn^2)$=$\mathcal{O}(Cn^2(|m|+K))$, where the length of a threshold signature and a signature share at most is $K$ bits. It's rasonable consider $|m|>>nK$. So the $\fACS$ communication complexity is $\mathcal{O}(Cn^2|m|)$.


==> CCS 22 long-version/hybrid-intro.tex <==
%!TEX root = main.tex

\section{Efficiency Bottleneck of Prior Art and Our Solution in a Nutshell}\label{sec:prior}

%The above issues correspond to a fundamental ``dilemma'' lying in the  design space of BFT consensus protocols suitable for the open Internet: the cutting-edge (partially) synchronous protocols can optimistically work very fast,  but lack  liveness guarantee in adversarial networks;
%on the contrary, the fully asynchronous protocols  are robust even in malicious networks, but  suffer from poor latency performance in the normal case. 



%\medskip
\noindent
{\bf Efficiency obstacles in prior art}.
%One natural question arises: can we  resolve the  ``dilemma'' to design a new atomic broadcast protocol achieving the best of both synchronous and asynchronous paradigms, such that it is super fast on the normal Internet and remains robust all the time (even if in an asynchronous network)?
%Regarding the question,
As briefly mentioned, pioneering works of Kursawe-Shoup \cite{kursawe05} (KS02)  and a following improvement of Ramasamy-Cachin \cite{cachin05} (RC05)
initiated the study of {\em optimistic asynchronous atomic broadcast} by adding a deterministic fastlane to fully asynchronous atomic broadcast, and they adopted multi-valued {\em validated} Byzantine agreement ($\mathsf{MVBA}$) to facilitate fallback once the fastlane fails to progress. 



Nevertheless, these prior studies are theoretical in   asynchronous networks, as they rely on heavy $\mathsf{MVBA}$ or even heavier full-fledged state-machine replication for fallback.
Serious efficiency hurdle remains in such cumbersome fallback, thus failing to harvest the best of   both paths in practice. 
%
Let us first overview the remaining   hurdles and  design challenges.
%
%As Fig. \ref{fig:ks02} illustrates, they initially run a deterministic protocol as ``fastlane'' to quickly progress in the optimistic case of good networks. But if the fastlane does not   progress in time (e.g., because of a potential asynchronous adversary), a fallback mechanism then is triggered to first clean any possible disagreement caused by the failed fastlane (through a pace-synchronization mechanism analog to view-change) and then ensure liveness (via a robust pessimistic path consisting of a full-fledged asynchronous protocol).
%The fastlane might luckily progress very fast in good network conditions, but a potential asynchronous adversary might   cause it grind to a halt,
%so a fallback mechanism is brought in worse cases to switch a stuck fastlane into a robust pessimistic path that runs fully-fledged randomized asynchronous protocol.
%
%The goal is to leverage the fastlane to enhance the performance on  good days, while using asynchronous protocols as the pessimistic path to maintain   robust liveness on bad times. 
%
%The rationale behind the  paradigm  is straight:
%the realistic  Internet might become unstable or even adversarial sometimes, but usually there are   sufficient optimistic periods, during which the network stays in good conditions to deliver messages synchronously and thus a deterministic fastlane can be utilized to    improve the normal-case  performance. In this way, the ``amortized'' latency of such an asynchronous protocol can be closer to the deterministic fastlane  instead of always suffering from the slow   pessimistic path.




%
%\footnote{Sometimes,   fastlane is also   called as   optimistic path or Bolt in the paper.} 
%to a  randomized pessimistic path  through a fallback mechanism (that was called {\em recover} in \cite{kursawe05,cachin05} and is similar to ``view change'' in many     partially synchronous protocols such as PBFT  but with a slightly more general purpose).  %\footnote{Several other works consider how to get a higher tolerance in optimistic (synchronous) case, while we focus on harvesting the best efficiency without giving up liveness. See Related Work for more careful comparisons.}. 


%If optimistic case are common enough, the amortized latency would be close to 
% frequently.
%\footnote{Note that it is arguably appropriate to assume that the network might optimistically hold synchrony. Actually many partially synchronous protocols   adopt an even heavier assumption that synchrony must hold for a while to argue the    liveness property. Same to why partially synchronous protocols can be live, the optimistic path of hybrid protocols can  progress in   benign cases. }


% \cite{kursawe05, cachin05}. 


%for us to look back how earlier studies leveraged the ``hybridization'' art%We realize the general ``hybridization'' idea behind these studies is still meaningful nowadays. 
%
%These pioneering studies %The aim of hybridization then becomes to squeeze the most performance out of   optimistic synchrony via deterministic executions, while remains a ranzdomized pessimistic path to preserve high robustness against potential adversarial networks.
%
%Such that, when optimistic conditions  actually hold (e.g., synchrony and honest leader), the concrete performance could be optimal (e.g., linear communications/messages, constant running rounds, and responsiveness). 
%
%These results hint a promising approach to boost the concrete performance of asynchronous protocols.
%
%The above ``hybridization'' idea  becomes  enticing to practicalize asynchronous BFT to meet both robustness and performance demands. 
%
%Especially, 
%if there is a way to efficiently and safely hybridizing an optimal optimistic path and any robust fully asynchronous protocols, 

%At first glance, it is appealing to realize the best of both paths through hybridization, that is: 

%\footnote{Remark that for many partial-synchronous BFT protocols,   they might also offer high performance when the time assumption  holds, but might lose liveness when the network becomes unstable. However, the goal of hybrid protocol in our context can offer similar high performance when network is in good condition and still ensure liveness when the network becomes arbitrarily unstable. Moreover, it is arguably that the optimistic path can be prevalent in practice, otherwise the partially synchronous model cannot be justified.}


\ignore{%%%%%%
	
	From a high-level, such a ``hybrid" structure proceeds as follows:
	(i) when the network stays in good conditions, %(say, with some constant probabilities),% {and the leader is honest}, 
	the deterministic optimistic path can succeed to offer high performance similar to the cutting-edge (partially) synchronous protocols, and (ii) when the optimistic path fails to progress (e.g., within a chosen time parameter), it can enable parties to jointly fallback into the robust pessimistic path with randomized executions, so it can tolerate arbitrarily delayed networks to restore liveness and recover to the optimistic case as soon as possible.
	
	More interestingly,    this ``hybrid'' paradigm for asynchronous BFT might  bring more practical merits. Recall that when deploying deterministic (partially) synchronous protocols in the open Internet, the engineers have to conservatively choose the timeout parameter (or to adaptively increase it) %during the deterministic executions trying 
	in order to ensure the synchrony assumption to hold. This in turn leaves a chance to degrade the performance. Now, the fallback mechanisms ensures that liveness can be safeguarded by the asynchronous protocols in the worst case, so engineers can aggressively set the timeout parameter according to their optimistic estimation about benign network conditions for good days only,  making the optimistic path to be unchained and run in full horse-power to be even responsive.
}%%%%%

%, thus is unchained from . 
%While at the same time,  the protocol is from  adversary-influencing performance degradation.



%really responsive and


%without worrying fragile liveness,

% other than simply pooling the best of both paths  together.
%Since now the 


 
%\medskip
%\noindent
%{\bf Bottleneck of optimistic asynchronous atomic broadcast.} Although the high-level idea of  the above optimistic asynchronous atomic broadcast    appears to be enticing in theory,  the actual design was complicated since the whole fallback mechanism shall be guaranteed to work in fully asynchronous network.
%
%In particular, if we aim to harvest the best of   both paths of optimistic asynchronous  $\mathsf{ABC}$  in practice, serious efficiency hurdle  remains.
%. to make the cumbersome fallback mechanism simpler and more efficient.
%
%
%The first immediate issue is that asynchronous BFT protocols themselves were with large communications, e.g., cubic to the number of nodes $n$. But even if we replace the pessimistic path with the recently improved randomised protocols such as \cite{honeybadger,guo2020dumbo},  the asynchronous fallback mechanism itself is also complicated and heavy. 
%
%
%Though  ``hybridization'' is a promising approach to  high-performing asynchronous BFT protocols, 
%The main technical barrier of making   ``hybridization'' practical is how to efficiently switch to the randomized pessimistic path when the fast deterministic path fails.
%behind the methodology is also clear, that is how to make the fallback mechanism secure as well as efficient. 
%
%without relying on any timing assumptions.
% even if the communication among parties can be arbitrarily delayed. 




\smallskip
\noindent
\underline{\smash{\em Challenge  and effiency bottleneck lying in pace-synchronization}}.
%
As Fig. \ref{fig:ks02} illustrates, the fastlane of KS02 and RC05
  directly employs a sequence of some broadcast primitives (the output of which is also called a block for brevity). %e.g., reliable broadcasts in KS02 \cite{kursawe05} and a stronger variant of consistent broadcasts in RC05 \cite{cachin05},
%(i.e., a primitive that emulates an ideal broadcast channel from a designed leader to all parties)
%always ensures that one honest node receives a value, all others will receive the same value, but without liveness if leader/sender is malicious) 
If a party does not receive a block within a period (defined by a timeout parameter), then it  requests   fallback by informing other parties about the index of the block that it just received. 
When the honest parties receive a sufficient number of fallback requests (e.g., $2f+1$ in the presence of $f$ faulty parties), 
%all honest parties will do so.
%Nevertheless, different parties might have distinct local views about the progress of the failed fastlane.
%So they 
they execute the {\em pace-synchronization} mechanism    to decide where to continue   the pessimistic path.


%The output of pace-synchronization will confirm the  progress of fastlane, such that the parties can agree on an index of some broadcast instance that has been delivered, 
%from which the parties can continue to run a full-fledged asynchronous protocol to ensure the critical liveness against adversarial asynchronous network.
%Noticeably, the pace-synchronization is similar to the view-change in many partial synchronous protocols (e.g., that of PBFT's), 
%(i.e., the index of a broadcast instance which they synchronize up to)
%it has to be fully asynchronous .
%even if the synchrony assumption fails temporarily.
%, so they will synchronize their outputs up to the index and then continue to. %(and also synchronize the missing outputs to the current progress), 
%Those decisions need to be made even when the synchrony assumption fails temporarily. 
%
Since different honest parties may have different progress in the fastlane when they decide to fall back, e.g., some are now at block 5, some at block 10, thus {pace-synchronization} needs to ensure: (i) all honest parties can eventually enter the pessimistic path from the same block; and (ii) all the ``mess-ups'' (e.g., missing blocks) left by the fastlane can be properly handled. Both requirements should be satisfied in an asynchronous network! These requirements hint that all the parties may need to {\em agree} on a block index that is proposed by some honest party, 
otherwise they might decide to sync up to some blocks that were never delivered. Unfortunately, directly implementing such a functionality 
requires one-shot asynchronous (multi-valued) Byzantine agreement with strong validity
%(can be considered as a single-shot version of atomic broadcast) 
(that means the output must be from some honest party), which is   infeasible because of inherent exponential communication \cite{fitzi2003efficient}.





\begin{figure}[h]
	\vspace{-0.4cm}
	%\captionsetup{font={normalsize}}
	\begin{center}
		\includegraphics[width=8.5cm]{fig/ks02-rc05.pdf}\\
		\vspace{-0.2cm}
		\caption{Execution flow of KS02 \cite{kursawe05} and RC05 \cite{cachin05}. Both rely on cumbersome asynchronous MVBA  to do pace-sync.}	\label{fig:ks02}
	\end{center}
	\vspace{-0.3cm}
\end{figure}




%is at the core of  optimistic asynchronous atomic broadcasts, as it ensures:
%(i) If a broadcast instance in  fastlane did output to enough parties, 
%it must be considered as ``delivered'' after pace-synchronization, otherwise, the fastlane becomes useless because its output can be revoked;
%(ii) If distinct parties made varying progresses in the fastlane, e.g., someone outputs in 5 broadcasts while another one outputs in 6 broadcasts, it will clean such mess-up and ensure agreement.

%and it can be analog to view-change in many partial synchronous protocols (e.g., PBFT's),
%but it requires stronger security guarantees to further ensure liveness in asynchronous network.
%similar to the view-change in many partial synchronous protocols (e.g., that of PBFT's), 
As depicted in Fig. \ref{fig:ks02}, both KS02 and RC05 smartly implement  {pace-synchronization} through asynchronous multi-valued {\em validated} Byzantine agreement ($\mathsf{MVBA}$) to get around the infeasible strong validity.  An $\mathsf{MVBA}$ is a weaker  and implementable form of asynchronous multi-valued Byzantine agreement, the output of which is allowed to be from a malicious party but has to satisfy a predefined predicate. Still, $\mathsf{MVBA}$ is a  cumbersome building block (and can even construct full-fledged asynchronous atomic broadcast directly \cite{cachin01}). 
%
What's worse, KS02 and RC05 invoke this heavy primitive for both pace-synchronization and pessimistic path, causing at least  $\bigO(n^3)$-bit communication and dozens of rounds. Although we may reduce the $\bigO(n^3)$ communication to $\bigO(n^2)$ by some very recent results (e.g.,  Dumbo-MVBA   \cite{lu2020dumbo}), however, they remain costly in practice due to a large number of extra execution rounds and additional computing costs (e.g., erasure encoding/decoding).

\smallskip
\noindent
\underline{\smash{\em \rev{Slow pace-sync remains in a more general framework  \cite{700aublin}}}}. \rev{Later, \\Aublin et al. \cite{700aublin} studied a   more general framework that is flexible to assemble optimistic fastlanes and  full-fledged BFT   protocols,
	as long as   the underlying modules all satisfy a defined $\mathsf{Abstract}$ functionality.
	To facilitate fallback  when the fastlane fails due to network asynchrony or corruptions, 
	\cite{700aublin} used a stronger version of $\mathsf{Abstract}$ variant with guaranteed liveness (called $\mathsf{Backup}$).
	$\mathsf{Backup}$ can guarantee all parties to output exact $k$ common transactions \cite{700aublin}, 
	so   it can handle fallback by first finishing pace-sync, then deciding some output transactions (i.e., running as the pessimistic path), and finally restarting the fastlane.
}

\rev{ Aublin et al. \cite{700aublin} also pointed out that $\mathsf{Backup}$ (with guaranteed progress) can be obtained from full-fledged BFT protocols. 
	For example, \cite{700aublin} gave exemplary $\mathsf{Backup}$ instantiations based on PBFT \cite{castro2002practical} and Aardvark \cite{clement2009making} in the partially synchronous setting. 
	This indicated another feasible way to implement asynchronous fallback, i.e., implement $\mathsf{Backup}$ by full-fledged  asynchronous BFT protocols.}
	%
	
\rev{Unfortunately, when $\mathsf{Backup}$ is implemented via full-fledged  asynchronous BFT, it would be  as heavy as $\mathsf{MVBA}$ (or even heavier), since  most existing   performant asynchronous BFT protocols are either constructed from $\mathsf{MVBA}$ \cite{guo2020dumbo,guo2022speeding} or have implicit $\mathsf{MVBA}$ \cite{gelashvili2021jolteon}. 
	That said, though the framework presented in \cite{700aublin} is more general than KS02 and RC05, 
	it is not better than KS02 and RC05 with respect to the efficiency of pace-sync  (and thus has the same efficiency bottleneck lying in pace-sync).}

\rev{	
In contrast, we identify an extra simple property    (not covered by $\mathsf{Abstract}$ \cite{700aublin}), so the new fastlane abstraction (1) enables us to utilize a much simpler asynchronous pace-synchronization, and (2) still can be easily obtained with highly efficient instantiations.}

%\rev{	However, although the framework from Aublin et al. \cite{700aublin} is very general and intuitive, the efficient implementation of  $\mathsf{Backup}$ is unclear in the fully asynchronous setting, because their key primitive for fallback---$\mathsf{Backup}$ relies on full-fledged  asynchronous BFT, which is not cheaper than .
%	As a seeming alternative, one might   suggest to  leverage full-fledged  state-machine replication ($\mathsf{SMR}$, which can be thought of $\mathsf{ABC}$ with clients) instead of $\mathsf{MVBA}$  to realize pace-sync as   in \cite{700aublin}.
%Intuitively, every party can submit to $\mathsf{SMR}$  a  fallback proposal (carrying a  proposed fastlane block index   to continue the pessimistic path) when its fastlane fails to progress.
%Now, $\mathsf{SMR}$ can   eventually output all honest parties' fallback proposals and therefore allow the parties to decide a common fastlane position   to continue the pessimistic path. 
%Thus, the ($f+1$)-th smallest or ($f+1$)-th largest fallback proposal must be from an honest party, from which the pessimistic path can   start.
%But, unfortunately, asynchronous $\mathsf{SMR}$ is  as heavy as $\mathsf{MVBA}$ (or even heavier), since  most existing   performant asynchronous $\mathsf{SMR}$ protocols are either constructed from $\mathsf{MVBA}$ \cite{guo2020dumbo,guo2022speeding} or have implicit $\mathsf{MVBA}$ \cite{gelashvili2021jolteon}.}


%\footnote{Although   $\bigO(n^3)$ may be reduced to $\bigO(n^2)$ by some very recent results (e.g.,  MVBA from \cite{lu2020dumbo}), they remain costly in practice due to a large number of execution rounds and additional computing costs. In contrast, we present a much simpler fallback that can  be realized by a binary agreement.}  
%
%(including the recent \cite{ittai19} when input size depends on $n$, where $n$ is the number of peer parties) 
%(details to be given in next subsection).%Both KS02 and RC05 need to invoke several cumbersome MVBA  protocols 
%while doing pace-synchronization and running pessimistic path.
%Unfortunately, each MVBA would  incur   at least $\bigO(n^3)$   communicated bits 
%(including   the recent  construction in \cite{ittai19}) 
%\footnote{We note that the $\bigO(n^3)$ communication may be reduced to $\bigO(n^2)$ by some very recent results including the optimal extension protocol for    MVBA   \cite{lu2020dumbo} and the MVBA-based fallback in \cite{spiegelman2020search}. But they remain costly in practice due to the large amount of execution rounds and additional computing cost. In contrast, we present a much simpler fallback that does not need the advanced MVBA component and can   be realized by the basic  binary agreement.}  
 %Let alone very large size inputs were fed into the already cumbersome MVBA protocols for pace-synchronization \cite{kursawe05} and for  asynchronous consensus \cite{kursawe05, cachin05}.
 
%It follows that the pace-synchronization is at least as slow as the pessimistic path, which is  dozens of time slower than deterministic fastlane.
%which relax the validity requirement 




%It is possible that some honest node was running ahead and already committed block $s+k$ (where $k$ is some parameter determined by the protocol in \cite{kursawe05}). To avoid influencing the safty, the nodes will again execute MVBA protocols block-by-block trying to catch up with him to reach block $s+k$.


%a natural question arises: whether such protocols could really achieve {\em the best of both fastlane and pessimistic path} in practice?  I.e., as asynchronous atomic broadcast protocols, can they be as fast as the state-of-the-art (partial) synchronous protocols (e.g., $\mathsf{HotStuff}$) on good days, and also perform same to the best-possible asynchronous protocols (e.g., $\dumbo$) if encountering adversarial asynchronous networks?

%


%  in these earlier fallback designs \cite{kursawe05, cachin05}. 
%nearly  by  one single binary agreement (BA) instance, which is much more practical than all known MVBA constructions in terms of concrete running rounds.}


%which is an advanced   asynchronous agreement building block that can directly imply almost all flavors of asynchronous BFT protocols from complex atomic broadcasts to basic binary agreements \cite{cachin01,guo2020dumbo,cachin2002asynchronous}.
 




%{\em Prior technique}. 
%In the optimistic case, when messages are delivered within a guessed time parameter $\tau$ and the fastlane leader is honest, 
%It is intuitive as in \cite{kursawe05,cachin05} to directly deploy a stable leader version of a (partially) synchronous broadcast protocol for the optimistic path. When sufficient parties feel that the optimistic path is not making fast enough progress (or no progress at all), they could start the pace synchronization
%
%In the optimistic asynchronous BFT protocols, ``pace'' synchronization is the key  to enable the parties who quit from the optimistic path to cooperatively decide
%to jointly determine how many blocks  are indeed optimistically outputted  so they can sync  up to here, and more importantly, 
%this shall not rollback too many optimistic outputs;
%otherwise,  the confirmation of optimistic paths would be slowed down. For example, if $k$ optimistic blocks could be rolled back at worst, then an optimistic block can be finalized   only after $k$ more optimistic blocks are outputted.

%To bound the rollback of optimistic blocks,
%prior studies let the honest parties sign and   broadcast their current ``paces'' in the optimistic path, 
%then each party can wait $n-f$ such pace-signature pairs and take them as input to invoke an MVBA instance. 
%A set of $n-f$ valid pace-signature pairs would   be chosen by   MVBA and returned to all honest parties.
%Since each signed pace is also attached with a small proof attesting that at least $n-2f$ honest parties indeed output its precedent blocks,  
%the parties can choose the maximum pace out of the output set of MVBA minus one as the final common pace of optimistic path to sync up, 
%which would simply bound the rollback of optimistic path because the MVBA result contains at least one honestly signed pace that is at most one block earlier than the latest block outputted by the optimistic path.



%=====
\ignore{%%%%%
	Intuitively, when the fastlane cannot make  progress in time, 
	a fallback mechanism  must be activated to ensure all honest parties to: 
	(i) make an  agreement on the need of fallback since   enough parties have sensed the    fastlane failure;  
	(ii)   reach a consensus on the current fastlane progress such that all parties can realize common states from which to continue; 
	then (iii)  continue the execution by running some randomized  asynchronous protocols  in case   the fastlane completely fails, or re-enter the fastlane otherwise. The  fallback mechanism   must be safe and live in   fully {\em asynchronous} networks to ensure robust liveness of the entire protocol.
	
	====
	
	%<<<<<<< HEAD
	Earlier studies \cite{kursawe05, cachin05} demonstrated the theoretic feasibility of implementing the needed asynchronous fallback through   using  asynchronous multi-valued Byzantine agreement with external validity  (MVBA) \cite{cachin01}, which is an advanced   asynchronous agreement building block that can directly imply almost all flavors of asynchronous BFT protocols from complex   atomic broadcasts to   primitive   binary agreements \cite{cachin01,guo2020dumbo,cachin2002asynchronous}.
	% which can be used to directly construct an asynchronous BFT \cite{cachin01}. 
	%
}%%%%%




%=======
%Earlier studies \cite{kursawe05, cachin05} demonstrated how it is feasible to implement the fully asynchronous ``pace'' synchronization from the advanced building block of multi-value validated Byzantine agreement (MVBA) but   are suffering from  overall $\bigO(n^3)$   communications  and at least several tens of asynchronous rounds.\footnote{Remark that the $\bigO(n^3)$ communication of ``pace'' synchronization  might be reduced to $\bigO(n^2)$ by the recent improvement of optimal MVBA construction \cite{lu2020dumbo}, but the construction remains costly due to the large number of running rounds. In contrast, we present a ``pace'' synchronization nearly  by  one single binary agreement (BA) instance, which is much more practical than all known MVBA constructions in terms of concrete running rounds.}
%The high cost of ``pace'' synchronization can be further amplified by frequent fallbacks due to unpredictable wide-area network environments, 
%causing prohibitive overhead that greatly sacrifices the practicality of dual-path switches and further fails us in reaching the best of both paths.
%>>>>>>> c852c7212ba6bd73d6c17c16d6250e9cdf4e5ed4

\smallskip
\noindent
\underline{\smash{\em Consequences of slow pace-synchronization.}}   %Given the recent progress on practical asynchronous atomic broadcast, we may replace the pessimistic path easily with, say, $\dumbo$ protocols \cite{guo2020dumbo}. 
%
%
The inefficient pace-sync   severely harms the practical effectiveness of adding fastlane.
In particular, when  the network   may  fluctuate as in the real-world Internet, the pace-sync   phase  might be triggered frequently, 
and its high cost   might eliminate the benefits of adding fastlane.


\begin{figure}[h] 
	\vspace{-0.4cm}
		%\captionsetup{font={normalsize}}
	\begin{center}
		%\includegraphics[width=8cm]{fig/bottleneck.pdf}\\
		\includegraphics[width=8cm]{fig/fluctuate.pdf}\\
		\vspace{-0.4cm}	\caption{Consequence of slow fallback in KS02/RC05 in fluctuating networks. The length of each phase denotes   latency.}	\label{fig:bottleneck}
		%\caption{KS02/RC05 v.s. our new framework in case of frequent fallbacks. Our core technique of simplifying pace-sync into binary agreement becomes the crux to harvest of the best of both fastlane and pessimistic path.}	\label{fig:bottleneck}
	\end{center}
	\vspace{-0.4cm}
\end{figure}

%
To see the issue,  
consider the heavy pace-sync  of existing work   that is as slow as the asynchronous pessimistic path
%  is at least two  times 
%slower than the underlying asynchronous protocol, 
and dozens of times slower than the fastlane.\footnote{Actual situation might be much worse in RC02 \cite{kursawe05} because several more MVBA invocations with much larger inputs are executed in the pace-sync.}
%
As Fig. \ref{fig:bottleneck} (a) exemplifies,
although the network stays  in good conditions for the majority of  time, the overall average latency of the protocol is still way larger than its  fastlane. One  slow fallback could ``waste'' the gain of dozens of optimistic blocks,  and it essentially renders the optimistic fastlane ineffective. In the extreme case shown in Fig. \ref{fig:bottleneck} (b), the fallback  is always triggered because the fastlane leaders are facing adaptive denial-of-service attack,  
%using the slow fallback mechanism along with the fastlane  not only becomes ineffectiveness to save nothing, but actually 
it even doubles the cost of simply running the pessimistic asynchronous protocol alone.
 

%(smaller latency, say 40 times from our experimental estimation, e.g., Table \ref{table:summary}), 
%As shown in Fig. \ref{fig:bottleneck} (a), let us do a rough estimation about how bad it affects the overall performance: suppose the randomized asynchronous pessimistic path produces one third of all outputs, while the other two thirds of the outputs are generated by the optimistic deterministic  fastlane. This may not be rare when the underlying communication network is fluctuating, 
%the fastlane can interleave  to progress or completely fail, 
%causing the inefficient fallback frequently triggered once in three blocks (on average). 
%
%Now as illustrated in Fig. \ref{fig:bottleneck} (a), the overall protocol has a latency at least 2/3 of the underlying asynchronous protocol, which is still a dozen times slower than the deterministic path.
%actually has no performance improvement comparing with the asynchronous protocol 
%even though the deterministic fastlane has been executed for the most  time.
%









It follows that in the wide-area Internet,    {\em inefficient pace synchronization} in previous theoretical protocols   likely eliminates the potential benefits of    optimistic fastlane, and thus their applicability is limited.  
So a fundamental practical challenge remains to minimize the overhead of pace-sync, such that we can harvest the  best of both paths  in optimistic asynchronous atomic broadcast.
%Another simpler example  is the extreme case 
\ignore{%%%%%%
	\footnote{Different from the challenging fallback to the pessimistic path, making all parties to restart the fastlane nearly simultaneously can be   trivial  if the underlying network is indeed  synchronous.
		Imagine  the next simple ``synchronizer'' to handle this trivial task:  each party   multicasts a ``{\textsc{TryBolt}}'' message to announce the termination of its pessimistic path; in addition, it waits for $f+1$ ``{\textsc{TryBolt}}''     to    multicast ``{\textsc{StartBolt}}''; it also waits for $n-2f$ ``{\textsc{StartBolt}}'' and multicasts the message if not sending it yet; so everyone can       receive $n-f$ ``{\textsc{StartBolt}}'' messages nearly at the same time to  re-enter the fastlane.
		%  during the actually synchronous periods. 
		%Imagine  the next ``synchronizer'' to handle this simple task: each party   multicasts a  signature to announce the termination of its pessimistic path; in addition, it waits for enough such valid signatures   to    multicast a set of them to the network; at the same time, it waits for such a set of signatures to transfer it to all parties; so everyone can immediately re-enter the fastlane upon receiving the valid set of signatures, which 
		%can fix clock drift and thus make all parties   restart the fastlane nearly simultaneously if the underlying network is indeed  synchronous.
		%Moreover, many asynchronous BFT might   incorporate similar tricks for ensuring termination and hence already bound the drift upon . 
		We omit the    trivial process throughout the paper.}
}%%%%%

%The high cost of existing fallback can be further amplified by frequent fallbacks due to unpredictable wide-area network environments, 
%causing prohibitive overhead that greatly sacrifices the practicality of dual-path switches and further fails us in reaching the best of both paths.
%What's worse, bearing above worry in mind, the engineers may again become conservative trying to avoid the expensive fallback, thus increasing the timeout parameter $\tau$, 
%\medskip



%Hence it is fair to say that all prior studies \cite{hotstuff, pala} cannot realize practical dual-path hybridization to really enjoy the best of both worlds,
%In particular, when their optimistic path fails, the "view-change" subprotocol to fallback into the asynchronous BFT brings prohibitive asymptotic complexities. This issue is even amplified in the scenario of   wide-area Internet, since the network might frequently become unstable and subsequently cause many costly fallbacks.
%
%followed by the open problem down below: 

%\smallskip
%{\centering \em How to design an asynchronous BFT protocol that achieves: (i) high-performance  in the benign network environments as if the state-of-the-art synchronous protocols and (ii)  robust worst-case performance   similar to the cutting-edge asynchronous protocols?}
%\smallskip
%\smallskip
%\begin{center}
%	{\em 
				%Can we minimize the overhead of pace-sync in optimistic asynchronous atomic broadcast, such that we can harvest the \\ best of both paths in  the real-world Internet environment?
		%Can we have an asynchronous atomic broadcast \\(with an optimistic deterministic fastlane), 
%		such that \\the overhead of its fallback is minimal  to harvest the best of both paths in  the real-world Internet environment?
		%such that it is ``as fast as'' the state-of-the-art deterministic protocols in the real-world networks? Additionally, can we , such that it can perform same to the currently most efficient asynchronous protocols in the worst-case?
%	}
%\end{center}
%\smallskip

%\input{overview}


%{\em }
%\footnote{Remark  that all styles of hybridized synchronous and partial-synchronous protocols \cite{sbft, zyzzyva,sync-hotstuff,thunderella} cannot answer this challenging open problem, as their ``view-change'' sub-protocols to switch between dual modes explicitly admit timing assumptions, which clearly causes the lack of liveness in fully asynchronous environment.}



==> CCS 22 long-version/hybrid.tex <==
%!TEX root=main.tex

\newpage

\section{The Hybrid BFT for atomic broadcast}

The hybrid protocl proceed in sequential round numbered $r$ for each consecutives epoch $e$. For each epoch $e$, consiting of an optimistic phase and recovery phases. A leader was designated for each epoch $e$ in the optimistic phase, it is responsible to broadcast the $n-f$ incoming message to all partys. If the leader don't follow the protocol or when network delay is unexpected, the protocol will swithches to the recovery phase. In fact, the optimistic phase guarantees the agreement and total order properties, but not the liveness property; however, the protocol can effectively determine if the liveness are potentially threatened, the hybrid BFT can get guarantees the liveness by the recovery phase.  The recovery phases can help all party make progress on same checkpoint, and guarantee to obtain some progresss on each epoch. After which all correct nodes will in a consistent state, the optimistic phase starts again with a new leader by \liang{round-robin} election.

\subsection{The optimistic phase of the Hybrid BFT}
In the optimistic phase of epoch $e$, the party of number $(e ~mod ~n)+1$ as the current epoch's leader. Every party have one initial queue, in this quene, the last three block is the $\pending$ block, $1$-$\notarized$ block and $2$-$\notarized$ block.  
%where $\pending$ block stores received message from leader but not yet delivered; $D$ stores all delivered message. 
Every party also maintains an array log of size $B$ that acts as a buffer for all message to deliver in the current epoch. 

\textbf{Details of the optimistic phase:} The optimistic phase algorithm is described in Algorithm \ref{alg:optimistic}. 

For a leader party, in every round, it will wait for receive some valid message from $n-f$ distinct party, upon received $n-f$ valid message, it will forward these message to all node and into next rounds, a new leader will continue this process after $N$ round.

For a non-leader party, it will send message to leader in every round, and wait for receive leader's message, upon the received message is valid after verify, it will into next round and repeat this work until $N$ rounds, and then, change leader to start next epoch.


\begin{breakablealgorithm}
	\caption{The optimistic phase of protocol H-BFT for party $P_{i}$ in epoch $e$(Proceed in sequential round numbered $r$ for each consecutive epoch $e$;):}
	\label{alg:optimistic}
	\begin{algorithmic}[1] 
		
		\noindent\textbf{Initialization}:  
		
		\textbf{B} is the batch size parameter;
		
		$buf$ = [ ] is a FIFO queue of input message;
		
		$D$=$\emptyset$; \hfill \{Delivered\}
		
		$P$=$\emptyset$;\hfill \{Pending\} 
		
		%	\noindent$PP$=$\emptyset.$\hfill \{Pre-pending\}
		
		$e=1$;\hfill\{current epoch\}
		
		$r=1$;\hfill\{current round\}
		
		$s=r-1$;\hfill\{$s$ is the pending sequence numbe\}
		
		$c=0$;\hfill\{the number of current complain partys\}
		
		$l=(e~mod~n)+1$;\hfill\{current leader number\}
		
		$proof_{r}=Hash(P)$\hfill\{$P$ is the pending block\}
		
		$start(T)$;\hfill\{$T$ is the static time parameter\}
		
		complain=false;\hfill\{current party's complaint status\}
		
		recovery=false;\hfill\{current party's recovery status\}
		
		\vspace*{0.2 cm}
		\If{ party $P_i$ \textbf{is} current epoch's leader}	
		\If{$(r>B)$ or (timeout(T))}
		\State complain();
		\Else
		\State \textbf{wait for} receipt valid message $\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}$ from $n-f$ distinct party such that $m_{j}\notin D\bigcup P$;
		\If{ received  $n-f$ valid message}
		\State stop(T);
		% \State  put these message and correspond signature into a set;
		\State  \textbf{send} $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_i}$ to all party;
		\State  put $P$ add into $D$;
		\State empty(P);
		\State  put $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_i}$ add into $P$; 
		\State   $ r=r+1$;
		\State  start(T);
		\EndIf
		\EndIf
		\EndIf
		
		
		\vspace*{0.2 cm}
		\If{party $P_i$ \textbf{is not} current epoch's leader}
		\If{$(r>B)$ or (timeout(T))}
		\State complain();
		\Else
		\State \textbf{send} message $\{m_i,proof_{r},\{e,r,Hash(m_i,proof_{r})\}_{\sigma_i}\}$ to leader $P_{l}$ and $m_{i}\notin D\bigcup P$;
		\If{received a message $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_l}$ from leader $P_l$}
		\State stop(T);
		\State  input the message into verify(); 
		\If{verify()=1}
		\State  put $P$ add into $D$; 
		\State  empty(P); 
		\State  put $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_l}$ add into $P$;
		% \State  buf= buf-$D$;
		\State  $r=r+1$;
		\State  start(T);
		\EndIf	
		\If{verify()=0}
		\State complain();  
		\EndIf
		\EndIf
		\EndIf     
		\EndIf
		
		
		\vspace*{0.2 cm}
		\If{ received $(e,complain)_{\sigma_j}$ from $P_{j}$ for the first time}
		\State set $c=c+1$;
		
		\If{$c=f+1~ and ~\neg complain()$}
		\State complain();
		\EndIf
		
		\If{$c=2f+1$}
		\State complain=false;
		\State recovery=true;
		\State  recovery();
		\EndIf			
		\EndIf
	\end{algorithmic}
\end{breakablealgorithm}


\textbf{Switching to the Recovery Phase:} A correct party will switch to complain mode when one of the conditions happened as follows: 

(1) If the network conditions is unexpected, that is to say, the party can not received message from the leader after time $T$;

(2) the leader is not functioning properly, that is to say, the party verify the message invalid which received from the current leader;

(3) when B round has been finished.

When a party into complain mode, it will invoke the function $complain()$ to told all other party that he was in complain. If a party is in complain mode, he will reject accept any message expect the complain messages.  

The Hybird protocol from the optimistic phase of protocols switches to recovery phase need at least $t+1$ party was in complain mode. If the $t+1$ complaint party was correct party, in this case, the complain mode will amplify which can made all party into complaint mode. Hence, every correct party can receive enough complain message from the $n-f$ distinct party, thereby the optimistic phase will switch to the recovery phase of protocols.




\begin{breakablealgorithm}
	\caption{The function components for party $P_i$:}
	\begin{algorithmic}[1] 
		
		\noindent\textbf{function help$(r_i,S)$}
		\If{$r_i<S$}
		\State\textbf{send} $(help, r_i, S)$ to all party;
		\State\textbf{For} each  value $r \in \{r_i, r_{i}+1,\cdots,S\}$ wait for $N-2f$ valid  VAL$(r;h;b_j;s_j)$ messages such that $b_j$ is a valid Merkle branch for root $h$ and leaf $s_j$; %$\{block[r+1],\cdots, block[S]\}$; 
		\State\textbf{Upon} received $N-2f$ valid messages with same $r$ and $h$,  then decode block[r];
		\State\textbf{then} add $\{block[r_i], block[r_i+1], \cdots, block[S]\}$ into $D$ by increasing order;
		\EndIf
		
		
		
		
		
		
		
		
		
		\vspace*{0.2 cm}\noindent\textbf{function complain()}
		\State complain=true;
		\State \textbf{Send} $(e,complain)_{\sigma_i}$ to all party;
		
		\vspace*{0.2 cm}\noindent\textbf{function verify()}
		
		\State \textbf{input} $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_l}$;
		
		\If {for all $m_{j}: m_{j}\notin$ $ D\bigcup P$ \textbf{and}  verifysig$(\{(m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}, {\sigma_l})$=1   \textbf{and}  verifysig$(e,r,Hash(m_j,proof_{r}), \sigma_j)$=1   \textbf{and} the value  $proof_{r}$ from $2f+1$ distinct party is the same}
		
		\State \textbf{return} 1;
		\Else
		\State \textbf{return} 0;
		\EndIf
		
		
	\end{algorithmic}
\end{breakablealgorithm}





\subsection{The fully asynchronous phase}


In the recovery phase of epoch $e$, all party first






the party of number $(e ~mod ~n)+1$ as the current epoch's leader. Every party have two initial queue $P$ and $D$, where $P$ stores received message from leader but not yet delivered; $D$ stores all delivered message. A party also maintains an array log of size $B$ that acts as a buffer for all message to deliver in the current epoch. 

\textbf{Details of the recovery phase:} The recovery phase algorithm is described in Algorithm \ref{alg:recovery}. 

The protocol of recovery phase is a leaderless BFT in this phase, it consists of three parts: firstly, all nodes need to agreement on the checkpoint; and then, 



For a leader party, in every round, it will wait for receive some valid message from $n-f$ distinct party, upon received $n-f$ valid message, it will forward these message to all node and into next rounds, a new leader will continue this process after $N$ round.

For a non-leader party, it will send message to leader in every round, and wait for receive leader's message, upon the received message is valid after verify, it will into next round and repeat this work until $N$ rounds, and then, change leader to start next epoch.















\begin{breakablealgorithm}
	\caption{The recovery phase of party $P_i$:}
	\label{alg:recovery}
	\begin{algorithmic}[1] 
		
		\noindent\textbf{function recovery():}
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	--------Step1: Agree on checkpoint--------}\vspace*{0.1 cm}
		\end{center}
		
		\If{$s=0$}
		\State \textbf{send} $\{recovery, e, 0, \emptyset\}_{\sigma_i}$ to all;\hfill// s is the pending sequence number; %is the complain's round number  
		\Else
		\State \textbf{send} %$(recovery, e,r,\{(proof_{r+1})_{\sigma_j}\}_{2f+1})_{\sigma_i}$to all;
		$\{recovery, e, s, \{\{e,s,Hash(m_j,proof_{s})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_i}$ to all;
		\EndIf
		
		\State \textbf{wait for} received $n-f$ valid recevory messages %$\{recovery,e,s,\{(e,s)_{\sigma_{j^{'}}}\}_{2f+1}\}_{\sigma_j}$ or $\{recovery, e, 0, \emptyset\}_{\sigma_j}$ 
		from $n-f$ distinct party $P_j$;% such that these messages verify is valid and $e$ is the current epoch;
		
		
		
		\If{ received  $n-f$ valid message}
		\State Let $R=Max(s^{'}_{1},s^{'}_{2},\dots,s^{'}_{n-f})$;
		\State Propose $R$ to $TCBA$;
		\State $S\leftarrow TCBA-1$;
		\State\textbf{Return} S;
		\EndIf 
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	--------Step2: Make sure to obtain progress--------}\vspace*{0.1 cm}
		\end{center}
		\If{$S\leqslant 0$}
		\State Honey-badger();
		\Else
		
		\If{$r=S$}
		\State put $P$ add into $D$; 
		\EndIf
		
		
		\If{$r<S$}
		\State help$(r,S)$;
		\EndIf
		
		
		
		\If{received $(help, r_j, S)$ from party $P_j$}
		\If{$r>r_j$}
		\While {$r>r_j$ and $r_j \leqslant  S$}
		\State \textbf{let} $\{b_k\}_{k \in  [N]}$ be the blocks of an $(N-2f; N)$-erasure coding scheme applied to $block[r_j]$;
		\State \textbf{let} $h$ be a Merkle tree root computed over $\{b_k\}$;
		\State \textbf{send} $VAL(r_j;h;b_i;s_i)$ to  party $P_j$, where $b_i$ is the $i^{th}$ Merkle tree branch;					
		%	\State\textbf{then send} $\{block[r_j], block[r_j+1],\cdots,block[r_i]\}$ to $P_j$;		 
		\State $r_j=r_j+1$;		
		\EndWhile	
		\Else	
		\State discard;
		\EndIf
		\EndIf
		
		
		
		\EndIf
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	------------Step3: Start the next epoch------------}\vspace*{0.1 cm}
		\end{center}
		
		
		
		\State$e=e+1$;
		\State$c=0$;
		\State$empty(P)$;
		\State$buf = buf-D$;
		\State enter the optimistic phase;
		
		
	\end{algorithmic}
\end{breakablealgorithm}








\newpage

\section{The cost of the hybrid BFT}


\begin{table}[htbp]
	
	\centering  
	%	\fontsize{6.5}{8}\selectfont  
	\caption{\bf \large Asymptotic performance comparison for atomic broadcast}  
	\label{tab:performance_comparison}  
	\begin{tabular}{|c|c|c|c|c|c|c|c|}  
		\hline  
		\multirow{2}{*}{Protocol}&\multirow{2}{*}{Async?}&\multicolumn{2}{c|}{Communication Complexity}&\multicolumn{2}{c|}{Message Complexity}\cr
		\cline{3-6}  
		& &Optim.&Worst&Optim.&Worst\cr  
		\hline  
		\hline  
		PBFT&No&$\mathcal{O}(N)$&$\infty$&$\mathcal{O}(N^2)$&$\infty$ \cr
		\hline 
		CKPS01&Yes&$\mathcal{O}(N^3)$&$\mathcal{O}(N^3)$&$\mathcal{O}(N^2)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		KS02&Yes&$\mathcal{O}(N^2)$&$\mathcal{O}(N^3)$&$\mathcal{O}(N^2)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		RC05&Yes&$\mathcal{O}(N)$&$\mathcal{O}(N^3)$&$\mathcal{O}(N)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		HoneyBarger&Yes&$\mathcal{O}(N)$&$\mathcal{O}(N)$&$\mathcal{O}(N^2)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		\multirow{2}{*}{Hybrid}&\multirow{2}{*}{Yes}&\multirow{2}{*}{$\mathcal{O}(N)$}&\multirow{2}{*}{$\mathcal{O}(N)$}&\multirow{2}{*}{$\mathcal{O}(N)$\multirow{2}{*}}&$\mathcal{O}(N^2)$(determistic) \cr
		\cline{6-6}  
		& &&&&$\mathcal{O}(N)$(probability)\cr  		
		
		\hline  
	\end{tabular}  
\end{table}  


==> CCS 22 long-version/mule.tex <==
%!TEX root = main.tex







%\medspace\medspace
%\medskip
\section{$\sys$ framework}
\label{sec:bdt}




%Now we  present     $\sys$ ($\mathsf{BDT}$) in details, as having the critical $\mathsf{nw\textnormal{-}ABC}$ and $\mathsf{tcv\textnormal{-}BA}$ ingredients at hand.  
%$\mathsf{BDT}$ is a generic framework with as-simple-as-possible pace synchronization (nicknamed by $\trans$)   centered around  $\mathsf{tcv\textnormal{-}BA}$, which allows to run any $\mathsf{nw\textnormal{-}ABC}$  instantiation such as $\tobc$ as the optimistic fastlane, and naturally can   use many     asynchronous consensus protocols (e.g., $\dumbo$ \cite{guo2020dumbo}, VABA \cite{ittai19}, Dumbo-MVBA \cite{lu2020dumbo}, DispersedLedger \cite{dl}) as its pessimistic path. 

%\medskip
%\noindent
%{\bf Overview}. 
As Fig. \ref{fig:hybrid} outlines, the fastlane of $\mathsf{BDT}$   is a $\tobc$ instance wrapped by a timer.
If honest parties can   receive a new $\tobc$ block in time, they would restart the timer to wait for the next $\tobc$ block.
Otherwise, the timer   expires, and the honest parties   multicast a fallback request containing the latest $\tobc$ block's quorum proof that they can see. %according to their local views.



\begin{figure}[htbp]
	%\captionsetup{font={small}}
	\vspace{-0.2cm}
	\begin{center}	
		\includegraphics[width=8cm]{fig/abstractHybrid.pdf}
		%\vspace{-0.25cm}
	\end{center}
	\vspace{-0.25cm}
	\caption{The execution flow of $\sys$ %When $\ABA$ returns 0 or   $\RB$ recovers invalid value, $\eoVABA$ goes to $\IDE$ and randomly elects another dispersal to recover.
	}	
	\label{fig:hybrid}
	\vspace{-0.2cm}
\end{figure}



After timeout, each party   waits for $n-f$   fallback requests with valid $\tobc$ block proofs, and enters pace-sync.
They invoke $\mathsf{tcv\textnormal{-}BA}$ with using the maximum block index (slot) in the received fallback requests as input.
Eventually, the honest parties enter the $\mathsf{tcv\textnormal{-}BA}$ and decide to either retry the fastlane or start the pessimistic path. As we briefly mentioned before, the reason we can use such a simple version of {\em binary} agreement is that via a careful analysis, we can find that \nwabc\/ prepares all honest parties will enter $\tcvba$ with one of neighboring indices as input.

%output the same slot number to all honest  parties, such that they can tentatively continue another fastlane or   run the pessimistic path according to the $\mathsf{tcv\textnormal{-}BA}$ output.


%After that, every honest party either has the globally latest $\tobc$ block's slot number or one less than that, so they can invoke $\mathsf{tcv\textnormal{-}BA}$ 
%to pick up one out of these two numbers, from which they either 

The remaining non-triviality is that $\mathsf{tcv\textnormal{-}BA}$ cannot  ensure its output to always be the larger number out of the two possible inputs,
that means the globally latest $\tobc$ block can be revoked after pace-sync. Hence, the latest fastlane block is marked as ``pending'', 
and a ``pending'' block is finally output until the fastlane returns another new block.
This pending fastlane block ensures safety in $\mathsf{BDT}$.
 




%Though it seems straight to,
%there are still a few non-trivialities to construct  $\mathsf{BDT}$ from $\mathsf{nw\textnormal{-}ABC}$  and $\mathsf{tcv\textnormal{-}BA}$





\begin{figure*}[!b]
	\vspace{-0.2cm}
	\captionsetup{font={normalsize}}
	\begin{footnotesize}
		\centering
		\fbox{%
			\parbox{17.5cm}{%
				%Let  $e$ be the  epoch number, $Esize$ be the epoch size parameter, $\tau$ be the timeout parameter of optimistic paths, $T$ be a time parameter to check suspicious transaction censorship, and $\buf$ be a FIFO queue of input transactions 				
				
				%\vspace{0.1cm}
				{\color{orange}// {\bf Optimistic Path} (also the BDT protocol's main entry)}					
				
				Every party $\node_i$ runs the protocol in  consecutive epoch numbered $e$ (initialized as 1) as follows:
				\begin{itemize}
					\item initialize: $p_e\leftarrow 0$, $\prf_{e}\leftarrow\bot$,  $\mathsf{Paces}_e\leftarrow\{\}$,	$\notarized_e\leftarrow\emptyset$ %and $1$-$\notarized_e\leftarrow\emptyset$
					\item activate $\tobc[e]$ instance, and start a timer that expires if not being restarted after $\tau$ clock ``ticks'' (i.e., invoke $timer(\tau).start()$)
					\item upon $\tobc[e]$ delivers a $\block$: 
					\begin{itemize}
						\ignore{
							\item parse $\block$:=$ \langle e, p, \payload_{p}, \prf_{p} \rangle $, where $p$ is the ``slot'' number
							\item $\out.append(\notarized_e)$, $\buf\leftarrow\buf \setminus \{\payload \textrm{ in } \notarized_e\}$ {\color{orange} ~~~//  the elder pending fastlane block becomes finalized, thus being output}
							\item 
							%$2$-$\notarized_e\leftarrow$ $1$-$\notarized_e$, $1$-
							$\notarized_e\leftarrow \block$, $p_e\leftarrow p$, $\prf_{e}\leftarrow\prf_{p}$ {\color{orange} ~~~//  the newly output fastlane block becomes the pending block}
							\item $timer(\tau).restart$ {\color{orange} ~~~//   $\tobc[e]$ makes progress in time, so restart the ``heartbeat'' timer}
						}
						
						\item parse $\block$:=$ \langle e, p, \payload_{p}, \prf_{p} \rangle $, where $p$ is the ``slot'' number
						\item $\out.append(\notarized_e)$, $\buf\leftarrow\buf \setminus \{\payload \textrm{ in } \notarized_e\}$, $\notarized_e\leftarrow \block$ {\color{orange} ~~~//finalized  the elder pending block, pending the newly fastlane block}
						%\item $\notarized_e\leftarrow \block$, $p_e\leftarrow p$, $\prf_{e}\leftarrow\prf_{p}$ {\color{orange} ~~~//  the newly output fastlane block becomes the pending block}
						\item  $p_e\leftarrow p$, $\prf_{e}\leftarrow\prf_{p}$, $timer(\tau).restart$ {\color{orange} ~~~//   $\tobc[e]$ makes progress in time, so restart the ``heartbeat'' timer}
						
					\end{itemize}
					%or $p_e=Esize$ 
					\item upon $timer(\tau)$ expires  or the front $\tx$ in the backlog $\buf$ was buffered   $T$ clock ``ticks'' ago:
					\begin{itemize}
						\item invoke  $\tobc[e]$.$\abandon()$  and multicast $\view(e, \pace_e, \prf_{e})$ {\color{orange} ~~~ // the fastlane is probably stucking or censoring certain transactions}
					\end{itemize}					
					
					\item upon receiving  message $\view(e, \pace_{e}^j, \prf_{e}^j)$ from  $\node_j$ for the first time:
					\begin{itemize}
						\item if $\LogVerify(e, \pace_{e}^j, \prf_{e}^j) = 1$: $\mathsf{Paces}_e \leftarrow \mathsf{Paces}_e\cup \pace_{e}^j$
					\end{itemize}
					
					\begin{itemize}
						\item if $|\mathsf{Paces}_e|=n-f$:  {\color{orange} ~~~// enough parties have already quitted the fastlane}
						
						\begin{itemize}
							\item invoke  $\mathsf{\textbf{Transformer(e)}}$ and wait for its return to continue {\color{orange} ~~~// enter into the pace-synchronization phase}
							\item proceed to the next epoch $e \leftarrow e + 1$  {\color{orange} ~~~// restart the fastlane of next epoch}
						\end{itemize}					
					\end{itemize}			
				\end{itemize}	
				
				\vspace{-0.1cm}
				\dotfill
				
				{\color{orange}// \bf Pace Synchronization}
				
				\textbf{internal function} $\trans$($e$): {~~~\color{orange}// {\bf internal} function shares   all internal states of the BDT protocol}
				
				\begin{itemize}
					\item let $\maxview_e \leftarrow \max(\mathsf{Paces}_e)$ and then $\mathsf{syncPace}_e  \leftarrow \tcvba[e]$($\maxview_e$)  {~~~\color{orange} // see Fig. \ref{fig:tcvba} or \ref{fig:blackaba} for concrete implementations of $\tcvba$}
					
					\item  if $\mathsf{syncPace}_e > 0$:  %{~~~\color{orange}//  where $\mathsf{syncPace}_e$ is the $\tcvba[e]$ output }
					\begin{itemize}
						\item send $\view(e, \mathsf{syncPace}_e, \prf)$ to all if  $\mathsf{syncPace}_e\in\mathsf{Paces}_e$, where $\LogVerify(e, \mathsf{syncPace}_e, \prf) = 1$
						
						\item if $\mathsf{syncPace}_e = \pace_e$: $\out.append(\notarized_e)$ and $\buf=\buf \setminus \{\payload \textrm{ in } \notarized_e\}$ % {~\color{orange} //   $\out.append(\emptyset)$   appends nothing to $\out$}
						
						\item if $\mathsf{syncPace}_e = \pace_e+1$:
						
						\begin{itemize}
							\item wait for a valid $\view(e, \mathsf{syncPace}_e, \prf)$, %s.t. $\LogVerify(e, \mathsf{syncPace}_e, \prf) = 1$, 
							then $\block'\leftarrow\Extract(e, \mathsf{syncPace}_e, \prf)$ {\color{orange} // try to extract the missing block}%$\mathsf{syncPace}_e$-th block from the received fastlane messages}
							\item if $\block'$ is in form of $ ( e, \mathsf{syncPace}_e, \bot, \bot)$, then:  
							$\block'\leftarrow \gethelp(e, \pace_e, 1)$ {\color{orange} // failed to extract, have to rely on other   parties to fetch, cf. Fig. \ref{fig:help}}%the missing block from the fastlane, so have to rely on other   nodes to fetch it (because at least $f+1$ honest nodes do have the block), cf. Fig. \ref{fig:help}}%\mathsf{syncPace}_e - \pace_e)$
							
							\item $\out.append(\notarized_e).append(\block')$ and $\buf=\buf \setminus \{\payload \textrm{ in } \notarized_e \textrm{ and } \block'\}$
							
						\end{itemize}
						
						\item if $\mathsf{syncPace}_e > \pace_e+1$:   $\blocks \leftarrow \gethelp(e, \pace_e, \mathsf{syncPace}_e - \pace_e)$      {\color{orange} // contact other parties to fetch   missing fastlane blocks, cf. Fig. \ref{fig:help}}
						\begin{itemize}
							\item $\out.append(\notarized_e).append(\blocks)$ and $\buf=\buf \setminus \{\payload \textrm{ in } \notarized_e \textrm{ and } \blocks\}$  
						\end{itemize}
						\item continue \textbf{Optimistic Path} with $e \leftarrow e+1$
					\end{itemize}
					
					\item if $\mathsf{syncPace}_e=0$: 
					invoke  $\mathsf{\textbf{Pessimistic(e)}}$  and wait for  its return, then continue \textbf{Optimistic Path} with $e \leftarrow e+1$
				\end{itemize}
				
				\vspace{-0.1cm}
				\dotfill
				
				{\color{orange}// {\bf Pessimistic Path}}
				
				\textbf{internal function} $\Pessimistic$($e$): {~~~\color{orange}// {\bf internal} function shares   all internal states of the BDT protocol}
				
				\begin{itemize}			
					\item $\txs_i$ $\leftarrow$  randomly select $\lfloor B/n \rfloor$-sized transactions from the first $B$-sized transactions at the top of $\buf$
					\item $x_i \leftarrow \TPKE.\Enc(epk, \txs_i)$, namely, encrypt $\txs_i$ to obtain $x_i$  %{\color{orange}~~~ // threshold encryption}
					\item $\{x_j\}_{j \in S } \leftarrow  \ACS[e](x_i)$, where $S \subset [n]$ and $|S|\ge n-f$ %then wait to receive $\{x_j\}_{j \in S }$ from $\ACS[e]$, where $S \subset [n]$ %{\color{orange}~~~ // Dumbo2-ACS}
					\item %$\payload=\bigcup_{j \in S} \txs_j\leftarrow \{\TPKE.\Dec(epk, x_j)\}_{j \in S } $, namely, 
					For each $j\in S$, jointly decrypt the ciphertext $x_j$ to obtain $\txs_j$, so the payload $\payload=\bigcup_{j \in S} \txs_j\leftarrow \{\TPKE.\Dec(epk, x_j)\}_{j \in S } $
					
					\item let $\block := \langle e, 1, \payload, \bot \rangle$, then $\out.append(\block)$ and $\buf=\buf \setminus \{\payload \textrm{ in } \block\}$ 
					
				\end{itemize} 
				%{\color{orange} // This pessimistic path might be replaced by many asynchronous consensus protocols, e.g., ACS and MVBA. Throughout the paper, the pessimistic path is instantiated by Dumbo, i.e.,   using a reduction to ACS (Honeybadger \cite{honeybadger}) and an ACS implementation from Dumbo \cite{guo2020dumbo}. Essentially, the underlying    ACS   \cite{guo2020dumbo} can   be replaced by any improved implementation.}
			}
		}
		\vspace{-0.4cm}
		\caption{The $\sys$ (BDT) protocol}
		
		\label{fig:mule}
	\end{footnotesize}
	  \vspace{-0.1cm}
\end{figure*}




\begin{figure*}[!b]
	\captionsetup{font={normalsize}}
 	\vspace{-0.1cm}
	\begin{footnotesize}
		\centering
		\fbox{%
			\parbox{17.5cm}{%
				
				{\color{orange}// {\bf The $\help$ daemon process}}\\
				$\help$: It is a daemon process that can read the finalized output $\out$ of $\sys$, %as well as the $\notarized_e$ block of current epoch,  
				and it listens  to the down below event:
				\begin{itemize}
					\item  upon receiving message $\ghlp(e, \tip, \gap)$ from party $\node_j$ for the first time:
					\begin{itemize}
						\item assert $1 \leq \gap \le Esize$
						\item wait for $\out$ containing the $\block := \langle e, \tip + \gap, *, * \rangle$
						%\item wait for the last block in $\out$ having a slot number equal or greater than $\tip + \gap$
						%\item $\out_e$ $\leftarrow$ retrieve all blocks in $\out$ where the  epcoh field is $e$ 
						\item let $M \leftarrow$ retrieve all blocks in $\out$ from $\block := \langle e, \tip + 1, *, * \rangle$ to $\block := \langle e, \tip + \gap, *, * \rangle$
						
						
						\begin{itemize}
							%	\item let $M \leftarrow \out_e[\tip+1:\tip+\gap]$
							\item let $\{m_k\}_{k \in [n]}$   be the fragements of a $(n-2f, n)$-erasure code   applied to $M$  and $h$   be a Merkle tree root computed over $\{m_k\}_{k \in [n]}$ 
							%\item let $h$ to be the root of a Merkle tree computed over $\{m_k\}_{k \in [n]}$ 
							\item send $\hlp(e, \tip, \gap, h, m_i, b_i)$ to   $\node_j$ where $m_i$ is the $i$-th erasure-code fragement of $M$  and $b_i$ is the $i$-th Merkle tree branch %MT branch rooted from $h$
						\end{itemize}
					\end{itemize}
				\end{itemize}
				
				\vspace{-0.2cm}
				\hrulefill
				
				{\color{orange}// {\bf The $\gethelp$ function}}
				
				{\textbf{external function} $\gethelp(e, \tip, \gap)$:} 
				\begin{itemize}
					\item let $F\leftarrow[\ ]$ to be a dictionary structure such that $F[h]$ can store all leaves committed to Merkle tree root $h$ 
					\item multicast message $\ghlp(e, \tip, \gap)$
					\item upon receiving the message $\hlp(e, \tip, \gap, h, m_j, b_j)$ from party $\node_j$ for the first time:
					\begin{itemize}
						\item if $b_j$ is a valid Merkle branch for root $h$ and leaf $m_j$ then: $F[h] \leftarrow F[h] \cup (j, m_j) $;
						otherwise discard the   message
						\item if $|F[h]| = n-2f$ then:
						\begin{itemize}
							\item interpolate the $n-2f$ leaves stored in $F[h]$ to reconstruct $M$, then parse $M$ as a sequence of $\block s$ and return $\block s$
						\end{itemize} 
					\end{itemize}
					
				\end{itemize}
			}
		}
	\vspace{-0.4cm}
		\caption{$\help$ and $\gethelp$. $\help$ is a daemon process having access to the output $\out$, and $\gethelp$ is a function   to call   $\help$}
		\label{fig:help}
	\end{footnotesize}
	 \vspace{-0.1cm}
\end{figure*}

 





\smallskip
\noindent
{\bf Protocol details.}
$\mathsf{BDT}$   is formally illustrated in Fig. \ref{fig:mule}.
It  employs a  reduction to $\mathsf{nw\textnormal{-}ABC}$, $\tcvba$, and some asynchronous consensus (e.g., $\ACS$). 
%The state variables for any party  are as follows in table \ref{table:variables}.
Informally, it proceeds as follows by successive epochs: %Each epoch might invoke three phases, i.e., $\tobc$, $\trans$ and $\Pessimistic$, 
%and each epoch can be briefly described as follows:
\begin{enumerate}[leftmargin=0.6cm]
	\vspace{-0.1cm}
	\item
	{\em $\tobc$ phase.} 
	When an honest party enters an epoch $e$, 
	it   activates a $\tobc[e]$ instance, and locally starts an adversary-controlling  ``timer'' that expires after $\tau$ clock ``ticks'' and resets once hearing the ``heartbeat'' of $\tobc[e]$ (e.g., $\tobc[e]$ returns a new block). If one party receives a new   $\tobc[e]$ block in time without ``timeout'', it  temporarily records the block as  $\notarized$, finalizes the previous (non-empty) $\notarized$ block   as $\mathsf{BDT}$'s output, and sets its ``pace'' $p_e$ 	to the new block's slot number. Otherwise, the ``timeout'' mechanism interrupts, %(it could be the current leader is corrupted or the network failed to keep synchronous), 
	and the party   abandons $\tobc[e]$. %and broadcast the proof of latest $\tobc[e]$ block (i.e., for the current pace $p_e$)
	%to request fallback.
	%
	%Namely, every $\tobc[e]$  block is   confirmed once one more    $\tobc[e]$  block is appended to it.
	%
	Beside the above ``timeout'' mechanism to ensure $\tobc$ progress in time, we also consider   that some transactions are probably censored: if the oldest transaction (at the top of the input backlog) is not   output  for a  duration $T$, an interruption is also raised to abandon $\tobc[e]$.
	%Finally, it is optional that the parties might raise an interruption to quit from the fastlane if  $\tobc[e]$  has finalized enough ($Esize$) optimistic blocks.
	%
	Once a party  abandons $\tobc[e]$ for any    above reason, it immediately    multicasts   latest ``pace'' $p_e$   with  the corresponding block's proof  via  a $\view$ message. 
	%
	
	\item
	 {\em $\trans$ phase.} 
	If an honest party receives   ($n-f$) valid $\view$ messages from distinct parties w.r.t.  $\tobc[e]$,    it enters   $\trans$. 
	In the   phase, the party chooses the maximum ``pace'' $\maxview$ out of the $n-f$  ``paces'' sent from distinct parties,
	and it would use this $\maxview$ as input to invoke the  $\tcvba[e]$ instance. 
	%
	When $\tcvba[e]$ returns a value $\mathsf{syncPace}$,  all parties 
	agree to continue from the $\mathsf{syncPace}$-th block in $\tcvba[e]$.
	%the fastlane in this epoch $e$ has finalized $\mathsf{syncPace}$ optimistic blocks.
	In some worse case that a party did not yet receive all blocks up to $\mathsf{syncPace}$,  it can fetch  the missing blocks from other  parties by calling  the
	 $\gethelp$ function    (cf. Fig. \ref{fig:help}).
	
	\item
	 {\em $\Pessimistic$ phase.} This phase may not be executed unless the optimistic fastlane of the current epoch $e$ makes no   progress at all, i.e,  $\mathsf{syncPace}=0$. 	In the worst case,  %$\tobc[e]$ essentially contributes nothing to the actual output, and 
	 $\Pessimistic$ is invoked to guarantee that some blocks (e.g., one) can be generated despite an adversarial   network   or   corrupt leaders, which becomes   the last line of defense   to ensure the critical liveness.
	
\end{enumerate}



 
\noindent
{\bf $\help$ and $\gethelp$.} %We make some remarks about the execution procedures of the $\sys$ framework:
%
%\begin{itemize}
	  %First, for   concrete instantiations of $\tobc$, there are various choices to cater for varying demands. $\mathsf{Bolt}$-$\mathsf{sCAST}$ is from pipelined multicasts, 	which could be low latency in practice for its simplest communication pattern. $\mathsf{Bolt}$-$\mathsf{sRBC}$ can better  shift the communication load from the leader side to all parties, so it might subject to better performance if larger batch sizes are used for  higher throughput.
	%
	 %We elaborate the $\help$ service and the $\gethelp$ function shown in Figure \ref{fig:help}.
	 Besides the above main protocol procedures,
	 a party might  invoke the 	$\gethelp$ function to broadcast a $\ghlp$ message, when it realizes that some fastlane blocks are missing. 
	As Fig. \ref{fig:help} illustrates,   $\ghlp$ messages specify which blocks to retrieve,
	and every party also runs a $\help$ daemon   to  handle  $\ghlp$ messages.
	%The $\help$ service is a daemon process activated once every party is initialized and takes care of $\ghlp$ messages.
	Actually, any honest party that invokes  $\gethelp$ can eventually retrieve the missing  blocks, because at least $f+1$ honest parties indeed   output   the  blocks under request. The $\help$ daemon can also use the  techniques of erasure-code and Merkle commitment tree in verifiable information dispersal \cite{cachin2005asynchronous,honeybadger},  such that it only  responds with a coded fragment of the requested blocks, thus saving the overall communication  cost by an $\bigO(n)$ order.
	
	%\item It  is possible to further strengthen the $\help$ service and the $\gethelp$ function to dismiss the seemingly mandatory $Esize$ parameter from the $\mathsf{BDT}$  framework at the price of communication. For example, we can let every honest party to actively multicast the index (e.g., epoch and slot) of its latest  block in $\out$ ``periodically'' via checkpoint messages. Upon receiving enough checkpoint messages  including some block indices higher than the latest block in its local $\out$, an honest party can   learn how many blocks that it is currently missing, and thus it can ask others to fetch these missing blocks. This strengthened method for syncing  would allow us to remove the $Esize$ parameter, because the fastlanes   now no longer have to compulsorily end  ``periodically'' to invoke   $\trans$ for syncing up the missing fastlane blocks. Nevertheless, we still advocate to follow the current design to use the optional $Esize$ parameter and set it not too large, since this can give each party a   fair chance to be the leader of fastlanes, and more importantly, the periodic $\trans$ execution is cheap since it is a highly efficient module.
	
	 	%Moreover, once any  $\tobc$ block is placed into any honest party's final output $\out$, it is indeed finalized in the sense that no matter how does the pace synchronization phase execute, it would not be revoked. But the last one block of each $\tobc$ instance may not be included in the output $\out$,  since the $\notarized$  block   have a chance of not becoming part of the final output. We therefore advocate a strategy  that: in each fastlane, the  $Esize$-th block (i.e., the last one $\tobc$ block) can   include zero payload.
	
	%Though in our  protocol description,  we let the $\Pessimistic$ phase to agree only one block once it is invoked, we remark that there could be some global heuristic algorithms that can estimate how many pessimistic blocks to output during the $\Pessimistic$ phase according to the known public information (e.g., how many times the fastlane instances have completely failed to output nothing in a stream). Designing such a heuristic to better fit the real-world Internet environments could be an interesting engineering question to explore in the future  but   does not impact any security analysis in this paper.
	

%\end{itemize}




%\noindent{\bf Remarks on alternative fastlane strategies.} The exemplary fastlane instantiation in Figure \ref{fig:mule} is a parameterized by $Esize$ to specify that each $\tobc$ instance is terminated to run pace-synchronization after $Esize$ fastlane blocks are output. When the fastlane is built from some $\tobc$ instantiation such as $\mathsf{Bolt\textnormal{-}sCAST}$, it is possible that up to $f$ honest parties might be much slower than the else honest parties (which can even be intentionally caused by malicious fastlane leader). The strategy of ``periodically'' stopping fastlanes to invoke $\trans$ can enable all parties to quickly sync up any missing blocks. Nevertheless, this $Esize$ parameter is essentially optional. For example, it is possible to   tweak the $\help$ service and the $\gethelp$ function to dismiss the  $Esize$ parameter: every   party  simply multicast the  epoch and slot  of its latest fastlane block   ``periodically'' via some checkpoint messages,  so that an honest party can learn how many blocks   it is currently missing after receiving enough checkpoint messages,  and thus   can ask others to fetch them. Nevertheless, we   advocate  the current design of using $Esize$ parameter and set $Esize$ not too large, since this can give each party a   fair chance to be the leader of fastlane, and more importantly, the periodic $\trans$ execution is essentially cheap for its   high  efficiency.

\smallskip
\noindent
{\bf Alternative pessimistic path.}
The exemplary $\Pessimistic$ path invokes $\dumbo$ to output one single block. %only if  the $\trans$ phase reveals the fastlane outputs nothing. 
Nonetheless, this is not the only design choice. First, \rev{$\BDT$ is a generic framework, and thus it is compatible with many recent asynchronous BFT protocols such as   DispersedLedger \cite{yang2021dispersedledger} and not restricted to $\dumbo$}. Second, there could be some global heuristics to estimate how many  blocks needed to generate during the pessimistic path according to some public   information (e.g., how many times the fastlane completely fails   in a stream). Designing such  heuristics to better fit   real-world Internet environments could be an interesting engineering question to explore in the future  but   does not impact any security analysis.





==> CCS 22 long-version/overview.tex <==


%!TEX root = main.tex

%\subsection{Our contributions}
\medskip
\noindent{\bf Technical overview.}  The key observations and    basic ideas behind our new efficient asynchronous fallback mechanism
 can be briefly explained as follows.
%the $\sys$ framework consists of three key components:
%(i) a deterministic optimistic path, a.k.a. Bolt, supposed to be fast in benign cases but lack live assurance;
%(ii) a robust randomized pessimistic path, a.k.a. Dumbo, expected to progress in arbitrary bad networks but probably be slow;
%(iii) a pace synchronization module, a.k.a. transformer, designed to assist efficient fallback  to Dumbo in case that Bolt loses liveness. 











{\em Prior technique}. 
%In the optimistic case, when messages are delivered within a guessed time parameter $\tau$ and the fastlane leader is honest, 
It is intuitive as in \cite{kursawe05,cachin05} to directly deploy a stable leader version of a (partially) synchronous broadcast protocol for the optimistic path. When sufficient parties feel that the optimistic path is not making fast enough progress (or no progress at all), they could start the pace synchronization
%
%In the optimistic asynchronous BFT protocols, ``pace'' synchronization is the key  to enable the parties who quit from the optimistic path to cooperatively decide
to jointly determine how many blocks  are indeed optimistically outputted  so they can sync  up to here, and more importantly, 
this shall not rollback too many optimistic outputs;
otherwise,  the confirmation of optimistic paths would be slowed down. For example, if $k$ optimistic blocks could be rolled back at worst, then an optimistic block can be finalized   only after $k$ more optimistic blocks are outputted.

To bound the rollback of optimistic blocks,
prior studies let the honest parties sign and   broadcast their current ``paces'' in the optimistic path, 
then each party can wait $n-f$ such pace-signature pairs and take them as input to invoke an MVBA instance. 
A set of $n-f$ valid pace-signature pairs would   be chosen by   MVBA and returned to all honest parties.
Since each signed pace is also attached with a small proof attesting that at least $n-2f$ honest parties indeed output its precedent blocks,  
the parties can choose the maximum pace out of the output set of MVBA minus one as the final common pace of optimistic path to sync up, 
which would simply bound the rollback of optimistic path because the MVBA result contains at least one honestly signed pace that is at most one block earlier than the latest block outputted by the optimistic path.




{\em Our methodology}. We realize that the above ``pace'' synchronization  of using a whole set of $n-f$  pace-signature pairs as MVBA input is unnecessary.
At the core of the $\sys$ framework,
we provide a highly efficient alternative ``pace'' synchronization mechanism  as fast as binary agreement.
%which can avoid the costly and slow MVBA module as well as strictly bound the possible rollback of optimistic blocks.

Our main observation lies in the fact that: there are at least $n-2f$ honest parties that do output the latest two optimistic path blocks,
so once all parties receive $n-f$ valid pace-signature pairs,
they can simply compute the maximum among these paces. Thanks to the ``notarizability'' of our fastlane abstraction, the honest parties would get either the same value or two consecutive integers,
and our task of ``pace'' synchronization is therefore reduced to make the honest parties choose one common integer out of those two unknown consecutive values. 
To this end, we propose and construct a novel asynchronous Byzantine agreement primitive to solve the specific issue of agreeing between two uncertain consecutive values. The construction has  message patterns and execution flows exactly same to the state-of-the-art binary agreement protocol in \cite{guo2020dumbo} %(and its instantiation version \cite{guo2020dumbo}) 
and only has three different lines in pseudocode for checking  slightly updated ``if-else'' conditions.


%{\em Other design mindsets}.
For the   efficiency of this new pace synchronization,
we now can adopt some more aggressive  optimistic tactics as follows.
First, different from \cite{kursawe05} that keeps on running optimistic path until it becomes problematic, we can proactively and even frequently raise ``pace'' synchronizations once the optimistic path has made enough progresses, 
which is important to ensure ``fairness'' when the optimistic path is leader-based. 
%Without an efficient ``pace'' synchronization, proactive switches optimistic path leaders would cause extra overhead.
Second, different from \cite{kursawe05,cachin05} where the pessimistic path is always executed after ``pace'' synchronization, we now can invoke the pessimistic path only if the optimistic path is completely failed, i.e., even if the optimistic path seemingly goes problematic during the course of executing, 
we would keep on trying the optimistic path again after ``pace'' synchronization as long as it remains to return some minimal output (e.g.,   one single block).





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{

barrier. Essence of optimistic path compatible with efficient fallback.


Asynchronous safety is too broad to describe the  that are  with 




\yuan{todo:  seems it is worth to put forth the notion of optimistic liveness for the hybrid paper. The story can be more clean with it. 1. Liveness in async is inherently randomized and therefore suspiciously heavyweight; 2.  a notion called optimistic liveness}
We for the first time give a positive answer to the above open problem.
To characterize what we mean by “fast” or “instant confirmation”, we adopt the same notion of
responsiveness as proposed in the work by Attiya, Dwork, Lynch, and Stockmyer [2] and later
adopted by others [27, 41]. A consensus protocol is said to be responsive iff any transaction input
to an honest node is confirmed in time that depends only on the actual network delay, but not on
any a-priori known upper bound on the network delay. Henceforth in this paper, we use $\delta$ to denote
the actual network delay and use $\Delta $ to denote an a-priori known upper bound of the network’s
delay where $\Delta $ is possibly provided as input to the protocol.
As shown in [41], achieving responsiveness requires us to assume that 2/3 of the players are
honest. (Additionally, all known protocols that are responsive are very complicated, and thus hard
to implement.)
Towards overcoming this issue, we here instead consider a notion of optimistic responsiveness—where responsiveness is only required to hold whenever some “goodness conditions” are
satisfies. More precisely, we consider two sets of conditions:

{\bf Optimistic-case and pessimistic-case.}
\begin{itemize}
	\item Worst-case conditions.
	\item Optimistic-case conditions.
	\item Pessimistic-case conditions.
\end{itemize}


{\bf $\sys$ in a nutshell.}
%, and bridge the gap between the high demands of the consortium blockchain and the robust asynchronous BFT protocols. 
%
On the core of our protocol design, we provide an efficient asynchronous ``view-change'' subprotocol to 
graft a simple optimistic path to a heavier fully asynchronous pessimistic path, 
such that we can hope the best of both. 
In particular, when the optimistic path succeeds to progress, the cost is rather low due to the extreme simplicity of the optimistic path. Even if the optimistic path fails to be live (e.g. due to corrupted leader or unstable network), our ``view-change'' subprotocol allows all correct nodes smoothly fall back into the backup pessimistic path to ensure robust liveness with incurring merely little  overhead that is asymptotically small.

In greater detail, our protocol is repeating to proceed in epoch, and in each epoch, it consists of three critical ingredients hereafter:
\begin{itemize}
	\item {\bf Optimistic path.} 
	Every epoch will begin with trying a simple and highly efficient leader-driven optimistic path, which leverages the  ``pipelining'' idea that was initially hinted by  Lamport \cite{paxos}, and recently revived in the lens of blockchain \cite{hotstuff, sync-hotstuff, pala, casper}.
	The ``pipelining'' design through the lens of blockchain is deemed as the crux to realize the optimistically higher performance, and involves only two types of messages, namely, $\propose$ and $\decide$. The $\decide$ message is sent from the leader to nodes (along with the decided output), while $\propose$ messages are sent from nodes to the leader (along with some proposed input).
	
	
	Generally speaking, in each epoch, a leader node is  ``elected'' (or assigned) to drive the optimistic path to proceed by slots: (i) in each slot,
	the leader node collects $\propose$s from the network, and each $\propose$ contains a digital signature for the $\decide$ committed by the leader in the immediate  precedent slot; (ii) upon the leader receives $n-f$ $\propose$s, the leader can commit a new $\decide$ message for the current slot, and this new $\decide$ message shall include $n-f$ valid signatures for the previous slot's $\decide$; (iii) later, upon receiving the new $\decide$ from the leader, a node checks the message contains $n-f$ valid signatures for the precedent $\decide$, and then digitally signs this current $\decide$ to create a new $\propose$ sent back to the leader for the next slot; (iv) and so forth.
	%
	
	The above scheme follows the recent elegant results on ``pipelining'', and is intuitively high-performing in case both the leader is correct and the timing assumption holds. 
	%In our instantiation, we require the optimistic path of each epoch stop after .
	
	%More importantly, even for arbitrary malicious leader and network, we can observe that: upon receiving a new valid $\decide$ from the leader, a node can extract a string that we call notarization string\footnote{The notarization string might also known as the quorum certificate in the literature.} to attest that ``at least $n-2f$ correct nodes already voted for the same precedent $\decide$ that I voted for''. 
	
	%To interpret the above fact one step further, let a node call its recently received proposal as $\pending$, the immediate precedent proposal as 1-$\notarized$, and the second precedent proposal as 2-$\notarized$, which immediate helps us conclude: once a correct node can extract a notarization string to attest ``at least $n-2f$ correct nodes already voted for its 1-$\notarized$ proposal'', these $n-2f$ correct nodes can also produce notarization strings to attest ``''.
	% This fact further means
	
	\item {\bf View-change.} The view-change protocol is activated and then be terminated, as long as at least $n-2f$ correct nodes ``abandon'' the optimistic path. In our instantiation, a correct node abandons the optimistic path, either when it feels no progress made for a while, or when the optimistic epoch is supposed to be completed as the number of already delivered messages has reached a parameter called epoch size. As such, we indeed place the view-change subprotocol in the critical path of optimistic cases. Remark that such the choice will not introduce much overhead, as view-changes are optimistically rare, especially when we moderately tune up the parameter of epoch size to allow honest leaders drive an epoch for a while.
	
	The efficiency of our view-change component stems from the nice properties of the optimistic path, that are: even for arbitrary malicious leader and network, upon receiving a new valid $\decide$ message from the leader (for the current slot), a correct node can extract a string that we call notarization string\footnote{The notarization string might also known as the quorum certificate in the literature.} to attest that ``at least $n-2f$ correct nodes already voted for the same precedent $\decide$ that I voted for in the previous slot''; in addition, the notarization string can be easily public verified, as it is essentially a set of signatures (bounded to slot numbers); more importantly, if  $\decide$ was not received and voted by $n-2f$ correct nodes in the corresponding asynchronous slot, the notarization string for it cannot be forged by the adversary due to the security of digital signature.
	
	The above facts hint us a solution towards constructing the asynchronous view-change with $\bigO(n^2)$ communications. 
	The basic idea is to let each correct node simply multicast  a view-change message that includes the ``highest'' notarization string abstracted from the optimistic path. Such the view-change message essentially makes a trial to convince the network: ``which slot I am at'' (i.e., ``what is my view'').
	Then, each node simply waits for $n-f$ validly notarized view-change messages from distinct nodes, and count the highest ``view'' out of  the $n-f$ notarized ``views'' as an important intermediate result called by $\maxview$.
	%
	After the multicast of view-change messages, we catch up with another crucial observation   to make our asynchronous view-change asymptotically better than prior studies, which is: $\maxview$s of all correct nodes are already somehow weakly-agreed, say correct nodes' $\maxview$s must either be the same integer (i.e. corresponding the same slot), or two consecutive integers (i.e. corresponding two consecutive slots). These weakly-agreed $\maxview$s correspond the cornerstone to efficiently make the correct nodes agree on how the progress made during the abandoned optimistic path. In particular, we formalize the special Byzantine agreement problem that correct nodes input two consecutive integers, and propose a simple construction with $\bigO(n^2)$ messages and $\bigO(1)$ expected running time  (see more details about the two-consecutive-value Byzantine agreement in Section \ref{sec:tcvba}).
	
	After all, the correct nodes will agree on how many messages are already delivered during the just abandoned optimistic epoch. More importantly, the above view-change procedure ensures at least $n-2f$ correct nodes indeed deliver the output messages up to the agreed ``view'', indicating that the correct nodes who did not deliver these outputs yet can always trivially sync up to this agreed ``view''.
	
	\item {\bf Pessimistic path.} Once the ``view-change'' subprotocol is terminated, all correct nodes can reach an agreement on how much progress the optimistic path does. In case too less progress (e.g., smaller than a security parameter) has been done in the optimistic path of the epoch, a heavier but robuster asynchronous BFT protocol is activated and then terminated. This asynchronous path (or interchangeably called pessimistic path) is inspired by the breakthrough of HBBFT to center around asynchronous common subset (ACS). Once the asynchronous path is done, the protocol proceeds to the next epoch.
	
	Different from Ben-Or ACS, we design and provide an expectedly constant-round ACS called fast ACS ($\fACS$), which realizes $\bigO(1)$ running time without sacrificing the asymptotic complexity of communications; moreover, the total message complexity of ACS is reduced from $\bigO(n^3)$ to $\bigO(\kappa n^2)$ where $\kappa$ is a security parameter (e.g., $\kappa=21$).\footnote{It could be appealing at first glance to leverage the recent MVBA construction \cite{ittai19} due to Abraham {\em et al.} to construct constant-round ACS, but it is not clear how to make it without asymptotically increasing commutations. For example, when we adopt the reduction in \cite{cachin01} to construct ACS from MVBA and count an ACS input as a word, the input size of MVBA has already been $\bigO(n)$ words. Once the MVBA instantiation in \cite{ittai19} is applied, the total  communications of ACS becomes $\bigO(n^3)$ words, which is equivalent to $\bigO(n^2)$ communication  per delivered ACS input and clearly sacrifices the ``communication-optimal''.}
	%, since the MVBA in \cite{ittai19} brings $\bigO(n^2|m|)$ words where $|m|=n$ due to the ACS construction \cite{cachin01}.}
	
	
	The construction of $\fACS$ is highly inspired by Ben-Or ACS with a few exceptions to introduce a small committee consisting of $\kappa$ nodes. In high-level, $\fACS$ proceeds as: (i) call a simple randomized election subprotocol to elect a committee of $\kappa$ nodes; (ii) all correct nodes send their input-signature pairs to the $\kappa$ committee nodes; (iii) each committee node collects a set of $n-f$   input-signature pairs, and uses reliable broadcast to send the set of input-signature pairs to the network; (iv-1) every correct node executes $\kappa$ ABA instances, each of which corresponds a particular committee node; (iv-2) a correct node assigns the input of a certain binary agreement to 1, iff it receives the valid input-signature pairs from the corresponding committee node (through reliable broadcast); (iv-3) as soon as one binary agreement terminates (with output 1), $\fACS$ outputs the input-signature pairs reliably broadcasted by the corresponding committee node.
	
	Due to the above $\fACS$, the bandwidth usage (of each node) is slightly amplified by $\kappa$ times relative to Ben-Or construction. However, the $\log(n)$ running time is removed, as $\fACS$ only ``halts'' to wait the termination of constant ABAs. In addition, the message complexity is also reduced by a factor of $\bigO(n)$, because $\fACS$ only requires $\kappa$ reliable broadcasts and $\kappa$ ABAs (instead of $n$) where $\kappa$ is a constant security parameter.
	As such, we can slightly trade off the concrete bandwidth usage for asymptotically less running time and asymptotically fewer messages. 
	Remark that this new trade-off option becomes appropriate, when the system burden is small and/or the bandwidth is somehow abundant. 
	
\end{itemize}

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> CCS 22 long-version/preliminary.tex <==
%!TEX root=main.tex
\medskip
\section{Preliminaries}
\label{sec:pre}



 
\noindent{\bf Collision-resistance hash function.}
A hash function $\hash: \{0,1\} ^ {*} \rightarrow \{0,1\} ^ \lambda$ is said to be collision-resistant, if no probabilistic polynomial algorithm adversary can generate a couple of distinct values $x_1$ and $x_2$ subject to $\hash(x_1)=\hash(x_2)$ except with negligible probability. %Through the paper, we assume that there exists a hash function $\hash$ that is collision-resistant.
 
\smallskip 
\noindent{\bf Non-interactive threshold signature.}
A non-interactive $(t, n)$-threshold signature scheme  $\TSIG$ is a tuple of  algorithms/protocols involving $n$ parties $\{\node_i\}_{i\in[n]}$ hereunder:
\begin{itemize}
	\item $\TSIG.\Setup(1^\lambda, t, n) \rightarrow (pk, { vk}, { sk})$. Once this algorithm/protocol is completed, there generates a public key $pk$,  a vector of public verification keys ${vk} := (vk_1, \cdots, vk_n)$, along with a vector of private secret keys ${ sk} := (sk_1, \cdots, sk_n)$ where $\node_i$ gets $sk_i$ only.
	\item $\TSIG.\SignShare_t(sk_i, m) \rightarrow \sigma_i$. It takes   a message $m$ and a private key share $sk_i$ as input, and outputs a signature share $\sigma_i$. We also use $\SignShare_t(m)$ for short.
	\item $\TSIG.\VrfyShare_t(pk, { vk}, m, (i, \sigma_i)) \rightarrow \{0,1\}$. This is a deterministic algorithm taking a message $m$, the public key $pk$, the verification keys ${ vk}$, a ``partial'' signature $\sigma_i$ and an index $i$ as input. It outputs 1 or 0 depending on whether $\sigma_i$ is deemed as a valid ``partial'' signature share produced by party $\node_i$ or not. We also use  $\VrfyShare_t(m, (i,\sigma_i))$ for short.
	\item $\TSIG.\Combine_t(pk, { vk}, m, \{(i, \sigma_i)\}_{i \in [n]}) \rightarrow \sigma $. The algorithm takes  the public key $pk$, the verification keys ${ vk}$, a message $m$, along with $t$ partial signature-index pairs $(i, \sigma_i)$  as input. This algorithm either outputs a full signature $\sigma$ for message $m$, or $\bot$ when $\{(i, \sigma_i)\}_{i \in [n]}$ contains ill-formed $(i, \sigma_i)$. We might use $\Combine_t(m, \{(i,\sigma_i)\}_{i \in [n]})$ for short.
	\item $\TSIG.\Vrfy_t(pk, m,\sigma) \rightarrow \{0,1\}$. This is a deterministic algorithm that takes as input a message $m$, the public key $pk$ and an ``combined'' signature $\sigma$. It outputs 1 or 0 depending on whether $\sigma$ is the valid signature for message $m$ or not. The notation $\Vrfy_t(m, \sigma)$ can be used for short.
\end{itemize}


	Besides the  trivial {\em correctness} of enforcing all honestly produced signature shares and signatures to pass verification, we   require {\em robustness} and {\em unforgeability} for  $\TSIG$:
\begin{itemize}
	
	\item {\em Robustness}. No probabilistic polynomial time (P.P.T.) adversary can produce $t$ valid ``partial'' signature shares, s.t. running $\Combine$ to aggregate them does {\em not} produce a valid ``full'' signature, except with  negligible probability. % in $\lambda$. 
	%
	Intuitively, it ensures any $t$ valid ``partial'' signatures of a message must induce a valid ``full''  signature \cite{shoup2000practical}.
	
	\item {\em Unforgeability}. This can be defined by a threshold version Existential UnForgeability under Chosen Message Attack  game.
	%, which   means that  for any message $m$, it is computational infeasible for the adversary $\A$ (who can adaptively corrupt $f$ parties that $f < t$) to produce
	%a valid ``full'' signature for $m$, unless $\A$ submits signing requests  to $t-f$ distinct uncorrupted parties to sign $m$.
	%
	Intuitively, it ensures that no P.P.T. adversary $\A$ controlling $t-1$ parties   can produce a valid ``full'' signature except with  negligible probability, unless $\A$ receives a ``partial'' signature  produced by an honest party.  
	%See \cite{libert2012non} for the formal definition.
	
\end{itemize}

%Remark that we assume $\TSIG.\Setup$ has already been correctly executed before the start of protocols, i.e., the setup of $\TSIG$ is taken for granted. 

%Remark that through the paper, we let $(t, n)$-$\TSIG$ scheme's parameter $n$ to be same as the number of 
%threshold $t=2f+1$, where $f$ is the number of Byzantine faulty parties to tolerate.




\smallskip
\noindent{\bf Threshold public key encryption ($\mathsf{TPKE}$)}. A $(t, n)$-threshold public key encryption scheme $\mathsf{TPKE}$ is a tuple of  algorithms/protocols involving $n$ parties $\{\node_i\}_{i\in[n]}$:
\begin{itemize}
	\item $\TPKE.\Setup(1^\lambda, t, n) \rightarrow (epk, { esk})$. It generates a public encryption key $epk$, along with a vector of private keys ${ esk}:= (esk_1, \cdots, esk_n)$, each item of which $esk_i$ is the secret key held by the corresponding party $\node_i$.
	\item $\TPKE.\Enc(epk, m) \rightarrow c$. It   encrypts a message $m$ to a ciphertext $c$ with using the public encryption key $epk$.
	\item $\TPKE.\DecShare(esk_i, c) \rightarrow c_i$. It allows a party $\node_i$ to use its secret key $esk_i$ to produce a   decryption share $c_i$  for $c$ (or a special symbol $\bot$ in case $c$ is ill-formed).
	\item $\TPKE.\Dec(epk, \{(i, c_i)\}_{i \in  [n]}) \rightarrow m$. It combines a set of valid decryption shares $(i,c_i)$ from at least $t$ distinct parties to reconstruct the plaintext $m$.
\end{itemize}

The {\em  correction} requirement of $\mathsf{TPKE}$ is obvious, which is any $t$ honest parties can cooperate to decrypt a ciphertext $c$ to get the corresponding plaintext $m$, as long as $c$ is produced by an honest party to encrypt $m$. 
%
Informally speaking, we expect an established $(t, n)$-$\mathsf{TPKE}$ scheme to be {\em robust} and {\em IND-CCA secure} (see \cite{shoup1998securing, boneh2006chosen} for rigor definitions).

%\begin{itemize}
%	\item {\bf Robustness} essentially requires the consistency of decryptions, which means no computationally bounded adversary (who statically corrupts up to $t-1$ parties) can produce a ciphertext $c$, such that two or more distinct plaintexts can be reconstructed from $c$.
%	\item {\bf Threshold-version of IND-CCA security} essentially ensures the adversary (who statically corrupts $t-1$ parties and is given decryption oracle) shall learn negligible information from a ciphertext    as if she does not see the ciphertext at all (before calling the decryption oracle to decrypt it).
	%, which is known to be strictly stronger than IND-CPA security.
%\end{itemize}

%Remark that we assume $\TPKE.\Setup$ has already been correctly executed before the start of protocols, i.e., the setup of $\TSIG$ is taken for granted. 


%\subsection{Threshold public key encryption}
%A $(t, n)$-threshold public key encryption scheme $\TPKE$ is a tuple of following four algorithms:
%\begin{itemize}
%	\item $\TPKE.\Setup(1^\lambda, t, n) \rightarrow (epk, \{esk_i\})$
%	\item $\TPKE.\Enc(epk, m) \rightarrow c$
%	\item $\TPKE.\DecShare(esk_i, c) \rightarrow c_i$
%	\item $\TPKE.\Dec(epk, c, \{i, c_i\}_{i \in S}) \rightarrow m$
%\end{itemize}



%\smallskip 
%\noindent{\bf Threshold common-coin scheme ($\coin$).} A $(t, n)$-threshold common-coin scheme $\coin[\id]$  \cite{cachin00} is a protocol joined by $n$ parties and satisfies the following properties:
%\begin{itemize}
%	\item {\em Agreement}. If $t$ parties invoke $\coin[\id]. \getcoin()$, then all honest parties that activate $\coin[\id]. \getcoin()$ can receive a common value $r \in \{0,1\} $. 
	%More importantly, the value $r$ is uniformly sampled in the range $\{0,1\}^{\lambda}$ and cannot be biased by P.P.T. adversary (who statically corrupts up to $t$ parties) except with negligible advantage.
%	\item {\em Unpredictability}. The value $r \leftarrow \coin[\id].\getcoin()$ cannot be predicated by P.P.T. adversary (who can statically corrupt up to $t-1$ parties) except with negligible advantage, until  one honest party calls $\coin[\id]. \getcoin()$.
%\end{itemize}

%Note that it is well-known to realize the above $(t, n)$-threshold common-coin scheme from an  established non-interactive $(t, n)$-threshold signature scheme among $n$ parties \cite{cachin00, honeybadger}. The detailed construction is too trivial to mention, and it only requires $\bigO(\lambda n)$ communication cost per party, $\bigO(n)$ messages per party and one asynchronous round to run.








 
\smallskip
\noindent{\bf Asynchronous binary   agreement ($\ABA$).} In an asynchronous binary agreement \cite{MMR15,lamport1982byzantine}, each party has a single-bit input, and their goal is to output a common bit. In particular, a protocol $\ABA$ running among $n$ parties with identification $\id$ is said to be asynchronous binary agreement, if it guarantees the following properties except with negligible probability:
\begin{itemize}
	\item {\em Termination}. If all honest parties pass inputs to $\ABA[\id]$, then all honest parties output associated to $\id$.

	\item {\em Agreement}. If any honest party outputs a bit $ b $  associated to $\id$,  then  all honest parties  output  the same   $ b $  on $\id$.
	
	\item {\em Validity}. If any honest party outputs $ b $ (associated to $\id$), then at least one honest party takes $ b $    as input to $\ABA[\id]$.
\end{itemize}

%We defer the concrete constructions of $\RBC$ and $\ABA$ protocols to Appendix.
 

\ignore{
\medskip
\noindent{\bf $(\eta, \kappa, \epsilon)$-Committee election ($\ACE$).} In a $(\eta, \kappa, \epsilon)$-committee election protocol running among $n$ parties (identified from $1$ through $n$) \cite{kapron2010fast,abraham2018solida}, the parties aim to output a $\kappa$-sized committee set $C$, such that $C$ is a subset of $\{1, \cdots, n\}$ containing at least $\eta$ correct parties' identities. In particular, a protocol with identification $\id$ is said to be $(\eta, \kappa, \epsilon)$-committee election, if it satisfies the following properties  in the presence of $f$ statically corrupted parties except with probability $\epsilon+negl(\lambda)$, where $negl(\lambda)$ is a negligible function of security parameter:
\begin{itemize}
	\item {\bf Termination.} If $f+1$ correct parties activate the protocol  $\ACE[\id]$, then all correct parties output (associated to $\id$).
	\item {\bf Agreement.} If a correct party outputs a committee set $C$  (associated to $\id$), all correct parties output the same set $C$  (associated to $\id$).
	\item {\bf Validity.} If any correct party outputs $C$  (associated to $\id$), then $|C|=\kappa$ and $C$ contains the identities of at least $\eta$ correct parties.
\end{itemize}

We emphasize on $(1, \kappa, \epsilon)$-$\ACE$ through the paper, namely, to elect a $\kappa$-sized committee containing at least one correct party with probability $1-\epsilon$. So $\kappa$ is essentially a security parameter of the committee election protocol \cite{abraham2019communication}.
%, and we might thus use $\ACE[\id]$ or $\kappa$-$\ACE[\id]$ as abbreviated forms of $(1, \kappa)$-$\ACE[\id]$.  
%
Also note that conditioned on  static corruptions up to $f$ as well as the already established $(f+1, n)$-threshold common-coin scheme $\coin$, for any given $\epsilon$, a security parameter $\kappa$ can be determined, such that it becomes trivial to construct $(1, \kappa, \epsilon)$-$\ACE$. Remark that the computational cost of $(1, \kappa,\epsilon)$-$\ACE$ is essentially same to $\coin.\getcoin()$.}



 
\smallskip
\noindent{\bf Asynchronous common subset ($\acs$).}
%We follow the elegant prior art to let the pessimistic path center around asynchronous common subset  ($\acs$). 
In the  $\acs$ protocol among $n$ parties (including up to $f$ Byzantine faulty parties) with identification $\id$,
each party takes as input a value and outputs a set of values.
%
It   satisfies   the following properties except with negligible probability:
	\begin{itemize}
		\item {\em Validity}. If an honest party outputs a set of values $\bf v$, then $|{\bf v}| \ge n - f$ and ${\bf v}$ contains the inputs from at least $n - 2f$ honest parties.
		\item {\em Agreement}. If an honest party outputs a set of values $\bf v$, then every party outputs the same set $\bf v$.
		\item {\em Termination}. If $n-f$ honest parties receive an input, then every honest party delivers an output.
	\end{itemize}
 

%{\em Remark}. We emphasize that this paper will not focus on designing new concrete construction of asynchronous common subset to improve the pessimistic path, as it actually targets to design an efficient way to grafting a super-efficient optimistic path into existing fully asynchronous BFT protocols. We might adopt the best performing constructions of $\acs$ so far due to \cite{honeybadger}. More importantly, due to our modular  protocol design and analysis, any $\acs$ construction (e.g. from MVBA \cite{cachin01}) can be adopted.

 

\smallskip
\noindent{\bf Strong provable  reliable broadcast ($\prbc$).} A protocol among a set of $n$ parties with   a designated sender, a predicate function  $\prbc.\Verify$  and an identification $\id$ is said to be  $\prbc$, if it satisfies the  next properties  (in presence of $f$ static   Byzantine faults) except with negligible probability:

\begin{itemize}
	\item {\em Validity}. If all honest parties invoke $\prbc[\id]$ and the sender is honest with taking a message $ m $ as input, all honest parties eventually output $m$   with proof $\sigma$  s.t. $\prbc.\Verify(\id, \sigma)=1$.
	
	\item {\em Agreement}. If two honest parties output $ m $ and $ m' $  in $\prbc[\id]$ respectively, then  $ m = m' $.
	
	\item {\em Totality}. If any (probably malicious) party outputs $ m $ and $\sigma$ in $\prbc[\id]$ s.t. $\prbc.\Verify(\id, \sigma)=1$, then all honest parties eventually output a value attached with a proof $\sigma$  s.t. $\prbc.\Verify(\id, \sigma)=1$ in $\prbc[\id]$.
	
	\item {\em Unforgeability}.  If $f+1$ or more honest parties do not activate $\prbc[\id]$, it computationally infeasible for any   party to produce a proof $\sigma$ 
	s.t. $\prbc.\Verify(\id, \sigma)=1$.
	
\end{itemize}

%\noindent
Note that {\em strong} provable  reliable broadcast adds   unforgeability   to    provable  reliable broadcast introduced in \cite{guo2020dumbo}, 
so it ensures that  when a valid proof is generated, there are enough honest parties that did activate the protocol.
Existing provable reliable broadcasts can   trivially obtain this property. For example, one can either   use any reliable broadcast as black-box with adding one extra round of multicasting $(n-f,n)$ threshold signatures as in \cite{guo2020dumbo},
or modify  Bracha's reliable broadcast \cite{bracha1987asynchronous} (or its variant \cite{honeybadger}) with encapsulating $(n-f,n)$ threshold signatures in the last $\ready$ messages as if in \cite{cachin2002asynchronous}.
%The original Bracha's RBC requires $ O(N^{2}|v|) $ bits of communication in order to broadcast a value of size $ |v| $. HoneyBadgerBFT uses RBC from Cachin and Tessaro, with erasure coding to reduce the cost to $ O(N|v|+N^{2}LogN) $.




==> CCS 22 long-version/related.tex <==
%!TEX root = main.tex

\section{Other Related Work}
%\medskip
%\noindent
%{\bf Other related work}. 
In the past decades,   asynchronous BFT protocols are mostly theoretical results \cite{rabin1983randomized,ben1983another,canetti1993fast,bracha1987asynchronous,abraham2008almost,patra2009simple,patra2011error,ben2003resilient,benor,correia2006consensus}, 
%and no clear and convincing evidence was ever shown to demonstrate real-world feasibility  
until several recent progresses such as HoneyBadgerBFT \cite{honeybadger}, BEAT \cite{beat}, $\dumbo$ protocols \cite{guo2020dumbo,lu2020dumbo,guo2022speeding}, VABA \cite{ittai19},  DAG-based asynchronous protocols \cite{danezis2022narwhal,dag}, \rev{and DispersedLedger \cite{yang2021dispersedledger}}. %and DAG-rider \cite{dag}. %They do not rely on timing assumptions and enjoy robustness as well as responsiveness; Nevertheless,  to obtain these benefits, 
Nevertheless, they still have  a   latency much larger than that of good-case   partially synchronous protocols. % because of using dozens of rounds to terminate.
\rev{Besides the earlier   discussed optimistic asynchronous consensus \cite{kursawe05,cachin05} and more general framework \cite{700aublin}}, Spiegelman recently \cite{spiegelman2020search}  used
VABA \cite{ittai19} to instantiate  
pace-sync in optimistic asynchronous atomic broadcast. However,  it is still inefficient, especially when  fallbacks   frequently occur.
\rev{    $\BDT$ framework presents a generic and   efficient solution to add a deterministic fastlane to   most existing asynchronous consensus protocols (except the DAG-based protocols). 
	%Such that these asynchronous   protocols can enjoy much smaller  latency under certain optimistic conditions.
	For example, it is compatible with   two very recent results of DispersedLedger    \cite{yang2021dispersedledger} and $\mathsf{Speeding}$-$\dumbo$ \cite{guo2022speeding}, and can directly employ them to instantiate   more efficient pessimistic path.}
	%This is because DispersedLedger is still a sequence of asynchronous common subset protocols (with separated data dissemination and Byzantine agreement). 
	%It is currently unclear how to use the DAG-based asynchronous protocols (e.g., Tusk \cite{danezis2022narwhal} and DAG-rider \cite{dag}) in    $\BDT$ framework without further adaptions,
    %because $\BDT$     requires the underlying asynchronous protocol to hold a termination property: if an honest party halts in the pessimistic path after output a certain block, then all honest parties still can output the same pessimistic block. However, Tusk  and DAG-rider might require all honest nodes to forever run, for example, if an honest party outputs a block and halts, other honest parties (that   not   output the same block yet) might require the halted party to continue run to help them eventually output the same block.


%\rev{DispersedLedger \cite{yang2021dispersedledger} focuses on reducing bandwidth wasted during running the agreement phase, the rationale behind is that it separates the bandwidth-intensive transaction dissemination and the bandwidth-oblivious agreement. The techniques also can be applied to BDT as well. However, DispersedLedger essentially still has the same structure as HoneyBadgerBFT  \cite{honeybadger}. Hence, BDT framework will also be brought many practical benefits to DispersedLedger.}
%\rev{Tusk \cite{danezis2022narwhal} and DAG-rider \cite{dag} are DAG-based  asynchronous protocols, our BDT framework needs a termination property in each epoch from the pessimistic path such that we can successfully restart fastlane. On the contrary, the DAG-based protocol may not ensure all honest nodes output in the same epoch, but they can output it after running more epochs. In specific, suppose some honest nodes in epoch R satisfy the output conditions and output block[R], while other honest nodes did not satisfy, but once these honest nodes satisfy the output conditions in epoch R$'$ (> R), then they also will output block[R] before block[R$'$]. If an honest node terminates in some epoch R, this might hurt other honest nodes to terminate. The DAG-based protocol is unclear to us whether it can work as an asynchronous protocol in the pessimistic path.}

\ignore{
Aforementioned KS02 \cite{kursawe05} and RC05 \cite{cachin05} demonstrated  theoretical feasibility of developing optimistic
asynchronous atomic broadcast to reduce the latency of asynchronous protocols in the benign network environments.
But they suffer from slow pace-sync instantiated by $\mathsf{MVBA}$ \cite{cachin01} in the fluctuating networks as earlier discussed.
Recently, Spiegelman \cite{spiegelman2020search}  leveraged
VABA \cite{ittai19} to instantiate  
pace-sync in optimistic asynchronous atomic broadcast. However,  it is still inefficient, especially when  fallbacks   frequently occur.
\rev{%Note that a slow asynchronous pace-synchronization could eliminate the benefits of fastlane in practice, and we reduce it to minimum --- binary BA (called $\tcvba$). 
	The general framework proposed by Aublin et al.   
	\cite{700aublin} provided an alternative idea.
	It defines a Backup primitive (i.e., a composable Abstract component with liveness guarantee to ensure the output of a certain number $k$ of transactions)   and thus can (i) decide  a common position representing where the fastlane fails and (ii) output a sequence of transactions. So Backup in   
	\cite{700aublin} can handle both pace-sync and pessimistic path in the optimistic asynchronous atomic broadcast.
	But  %,  is unclear how to be efficiently instantiated, 
	\cite{700aublin}  Backup was constructed via fully-fledged BFT protocols,
	which actually
	is not cheaper than  $\mathsf{MVBA}$   \cite{kursawe05,cachin05} in the fully asynchronous setting (since the state-of-the-art  asynchronous  BFT protocols are normally constructed from $\mathsf{MVBA}$).}
	In contrast to these prior studies \cite{kursawe05,cachin05,700aublin,spiegelman2020search} using asynchronous $\mathsf{MVBA}$ or heavier asynchronous $\mathsf{SMR}$ for pace-sync, we reduce pace-sync to only asynchronous {\em binary} agreement. \rev{It is possible because of our delicate formulation of a slightly stronger fastlane.}
	%because asynchronous $\mathsf{SMR}$ is known for its complexity \cite{miller2016honey}
	% performant asynchronous $\mathsf{SMR}$  can rely on $\mathsf{MVBA}$   to construct.
	%can be instantiated by 
	%and interestingly, this actually reduces to the fallback construction in .
	%In \cite{700aublin}, such $\mathsf{SMR}$ was Backup
	% \cite{700aublin} observed that liveness. 
	%\cite{700aublin} presented an Abstract in the fastlane, if we borrow the Abstract to our BDT, because the output (called abort history) of Abstract instance just has the property of abort order that it has the commit history as a prefix and different honest nodes could have different abort histories even if the length of all abort histories is the same. Besides, according to the properties of Abstract, it's also unclear to us how to extract the commit history from the abort history in Abstract. Hence, it is hard for us to decide the input of $\tcvba$ if we replace  $\mathsf{nw}$-$\mathsf{ABC}$ with Abstract \cite{700aublin}. In sum, we think Abstract is unsuitable for $\tcvba$. As stated previously,  \cite{700aublin} has to  leverage full-fledged $\mathsf{SMR}$ to realize pace-sync, but $\mathsf{SMR}$ is at least as heavy as $\mathsf{MVBA}$. Hence, the composition of Abstract and full-fledged $\mathsf{SMR}$ is more expensive than the composition of $\mathsf{nw}$-$\mathsf{ABC}$ and $\tcvba$.	Moreover, our BDT decouples pace-sync from the pessimistic path. If there is some progress in an epoch, it could directly switch back to the fastlane after pace-sync, thus completely avoiding the pessimistic path. The idea is difficult to achieve in the \cite{700aublin}.   
%Though,	it 	is still possible to suffer from large latency on the normal Internet where there are small network fluctuations.
}


It is well known that partially synchronous protocols \cite{yin2018hotstuff-full,pbft} can be responsive after GST in the absence of failures. Nonetheless,
if some parties are slow or even act maliciously, they might suffer from a worst-case latency related to the  upper bound of network delay. Some recent studies \cite{abraham2021good,abraham2020sync,thunderella,shrestha2020optimality,sbft,momose2020hybrid} also consider synchronous protocols with {\em optimistic responsiveness}, such that when some special conditions were satisfied, they can confirm transactions very quickly (with preserving optimal $n/2$ tolerance). Our protocol is {\em responsive} all the time, because it does not  wait for timeout that is set as large as the upper bound of network delay in all cases. 

Besides,  some literature \cite{blum2019synchronous,blum2021tardigrade,blum2020always,loss2018combining,momosemulti}  
studied how to combine synchronous and asynchronous protocols for stronger and/or flexible security guarantees in varying network environment.  
%This line of work might focus on  designing  protocols that can tolerate up to $n/2$  corruptions in the synchronous cases  and tolerate $n/3$ corruptions  in the asynchronous cases.  
We instead aim to harvest efficiency from the   deterministic protocols. %and   stick  with     $n/3$ tolerance (optimal in   asynchronous networks).

%\smallskip
\noindent\underline{\smash{\em Concurrent works}}. 
A concurrent work  \cite{gelashvili2021prepared} considers adding an asynchronous view-change to a variant of HotStuff. Very recently its extended version    \cite{gelashvili2021jolteon} was presented with implementations. They focus on a specific construction of asynchronous fallback tailored for HotStuff by opening up a recent MVBA protocol \cite{ittai19}, thus can have different efficiency trade-offs. On the other hand, they cannot inherit the recent progress of asynchronous BFT protocols to preserve the linear per transaction communication (as we do) in the pessimistic path, or future improvements (since BDT is generic).  Moreover, \cite{gelashvili2021jolteon} essentially still uses an MVBA to handle pace-sync, while we reduce the task to conceptual minimum---a binary agreement, which itself could have more efficient constructions. 

 
\ignore{
In the past decades, most  asynchronous BFT protocols are only theoretical results \cite{rabin1983randomized,ben1983another,canetti1993fast,bracha1987asynchronous,abraham2008almost,patra2009simple,patra2011error,ben2003resilient,benor,correia2006consensus}, and no clear and convincing evidence was ever shown to demonstrate real-world feasibility  until recent studies such as HoneyBadger BFT \cite{honeybadger}, BEAT \cite{beat}, $\dumbo$ BFT \cite{guo2020dumbo,lu2020dumbo} and VABA \cite{ittai19}. They do not rely on timing assumptions and enjoy robustness as well as responsiveness; nevertheless,  to obtain these benefits, they often have large latency (that is usually much larger than partially synchronous protocols under good network conditions) due to dozens of rounds to terminate.

The aforementioned KS02 \cite{kursawe05} and RC05 \cite{cachin05} demonstrated the theoretical feasibility of developing optimistic asynchronous atomic broadcast to reduce the latency of asynchronous protocols in the benign network environments. Very recently, Spiegelman \cite{spiegelman2020search} also studied this issue with using a recent MVBA construction \cite{ittai19} to instantiate the fallback.
However, as earlier discussed,   their frameworks and instantiations are still inefficient. 
In particular, the  fallback mechanisms invoke cumbersome MVBA to clean the mess of failed fastlanes.
In the realistic unstable networks, they may not guarantee the expected benefits of introducing the deterministic fastlanes, when frequent fallbacks are occurring.

It is well known that   partially synchronous protocols  can be responsive after $GST$ in the absence of failures. 
Nonetheless, if some parties are slow or even act maliciously, many of these protocols \cite{pbft,hotstuff} might suffer from a worst-case latency related to the network delay upper bound. Several other studies \cite{abraham2021goodcase,sync-hotstuff,thunderella,shrestha2020optimality,sbft,momose2020hybrid} consider synchronous protocols that achieve {\em optimistic responsiveness}, so the protocols can be responsive when some special conditions were satisfied while preserving   optimal  resilience against $n/2$ corruptions in other worse cases. In contrast, our protocol is {\em responsive} all the time  without relying on any optimistic condition. 

Besides, there is also some literature  \cite{blum2019synchronous,blum2020always,blum2020network,loss2018combining} that focuses on using the hybrid mechanism of synchronous and asynchronous protocols for stronger security guarantees, in particular for higher fault tolerance.  This line of work mainly aims to  design asynchronous protocols that can tolerate up to $n/2$  corruptions in the synchronous cases  and tolerate $n/3$ corruptions  in the asynchronous cases.  Our work instead aims to harvest efficiency from the deterministic protocols in practice.
}




%\noindent{\bf Outline of the paper.} Sections \ref{sec:pre} and \ref{sec:def} present the preliminary primitives and the problem definitions, respectively. After that, Section \ref{sec:fast} introduces the new fastlane formulation {\em notarizable weak atomic broadcast} and present two instantiations for it. Section \ref{sec:tcvba} then defines and constructs {\em two-consecutive-valued binary agreement}, which is the key ingredient for our new fallback mechanism. In Section \ref{sec:bdt}, we construct  our new generic practical framework $\sys$ for optimistic asynchronous atomic broadcast and analyze its security in details. We then implement the framework and demonstrate its high applicabilities by extensive real-world experiments across the globe in Section \ref{evaluation}.Complexity analysis and numerical estimations are  presented in Section \ref{sec:ca} to further discuss the applicability of $\sys$ in unstable network environments.


==> CCS 22 long-version/tcba.tex <==
%!TEX root = main.tex









\subsection{Two-consecutive-value BA}
%\section{Build the    AllSpark for our $\trans$: Two-Consecutive-Value Byzantine Agreement}
\label{sec:tcvba}

Another critical ingredient  is a variant of binary agreement that 
%As briefly mentioned in Introduction, our novel pace synchronization is created from a key component two-consecutive-value Byzantine agreement ($\tcvba$).
can help the honest parties to choose one common integer out of two unknown but consecutive numbers. % (i.e., agree on from which fastlane block to start fallback).
%thus implementing $\trans$ to   reach an agreement on how many blocks were indeed output in the optimistic fastlane.
%
Essentially, $\tcvba$ extends the conventional binary  agreement and can   be formalized as follows.




\begin{definition}  {\bf Two-consecutive-value Byzantine agreement}  ($\tcvba$) satisfies   termination, agreement and validity  (same to those of asynchronous binary agreement) with overwhelming probability, if all honest parties input a value in $\{v, v+1\}$ where $v \in \N$.
\end{definition}





%\vspace{-0.2cm}
\begin{figure}[h]
	%\vspace{-0.2cm}
	\captionsetup{font={normalsize}}
	\begin{footnotesize}
		\centering
		\fbox{%
			\parbox{8.2cm}{%
				For each party $\node_{i}$, make the following modifications to the $\ABA$ code in Alg. 7 of \cite{guo2020dumbo} (originally from \cite{MMR15} but with some adaptions to use Ethan MacBrough's suggestion  \cite{ababug} to fix the potential liveness issues of \cite{MMR15}):
				
				\vspace{0.1cm}
				Replace line 13-23 of  Algorithm 7 in \cite{guo2020dumbo} with the next instructions:			
				\begin{itemize}[leftmargin=0.3cm]
					\item $c\leftarrow \coin_r.\getcoin()$
					\begin{itemize}[leftmargin=0.25cm]
						\item if $S_r= \{v\}$ then:									
						
						\begin{itemize}[leftmargin=0.25cm]
							\item {\color{orange} if $v\%2 = c\%2$ }
							\begin{itemize}[leftmargin=0.25cm]
								\item  if $decided$ = false then: output $v$; $decided$ = true
								\item   else (i.e, $decided$ = true) then: halt						
							\end{itemize}									
							\item $\est_{r+1} \leftarrow v$
						\end{itemize}
						
						\item if $S_r= \{v_1, v_2\}$ then:
						\begin{itemize}[leftmargin=0.25cm]
							\item {\color{orange}if $v_1\%2 = c\%2$, then $\est_{r+1} \leftarrow v_1$}
							\item {\color{orange}else (i.e, $v_2\%2 = c\%2$), then $\est_{r+1} \leftarrow v_2$}
						\end{itemize}
						
					\end{itemize}
				\end{itemize}
				\vspace{-0.1cm}	 
			}
		}
		\vspace{-0.3cm}
		\caption{ $\tcvba$ protocol. Lines different to Alg. 7 in  \cite{guo2020dumbo} are    in {\color{orange} orange texts}.}
		\label{fig:tcvba}
		
	\end{footnotesize}
	\vspace{-0.2cm}
\end{figure}









To squeeze extreme performance of pace synchronization, we   give a non-black-box construction $\tcvba$ that only has to revise three lines of code of the practical $\ABA$ construction  adapted from \cite{MMR15}. This non-black-box construction basically reuses the protocol pseudocode 
except several if-else  checking (see Fig. \ref{fig:tcvba}) and hence has the same performance of this widely adopted   $\ABA$ protocol. 








In addition, $\tcvba$ can be constructed    from any  $\ABA$  with only one more    ``multicast'' round, cf. Figure \ref{fig:blackaba}. This black-box construction  provides us a convenient way to inherit any potential improvements of   underlying $\ABA$ primitives \cite{crain2020two, das2021practical}.
%especially when our non-black-box technique cannot be directly applied.




\vspace{-0.1cm}
\begin{figure}[h]
	\vspace{-0.1cm}
	%\captionsetup{font={normalsize}}
	\begin{footnotesize}
		\centering
		\fbox{%
			\parbox{8.2cm}{%				
				Let $\ABA$  be any asynchronous binary agreement, then   party $\node_{i}$ executes:				
				
				\vspace{0.1cm}Upon receiving input $R$ then: %initial $val_0 \leftarrow R$, $\values_r = \emptyset$ and $r \leftarrow 0$
				\begin{itemize}[leftmargin=0.3cm]
					%	\item $\values_r \leftarrow \{\}$
					\item multicast $\val(\id,R)$% to all,  $\values_r \leftarrow \values_r \cup \{val_r\}$
					%\item upon receiving $f+1$ $\val(e,v)$ messages with same number $v$ from distinct nodes then:
				
					\item { upon receiving $\val(\id,R')$ from $f+1$ parties containing the same $R'$}
				\begin{itemize}[leftmargin=0.25cm]
					\item  if $\val(\id,R')$ has not been sent before, then: multicast $\val(\id,R')$				
				\end{itemize}
					
					\item wait for receiving $2f+1$ $\val(\id,v)$ messages from distinct parties carrying the same $v$, and activate $\ABA[\id]$ with   $v\%2$ as input
					
					%\begin{itemize}[noitemsep,topsep=0pt]
					\item wait for $\ABA[\id]$ returns $b$:
					\begin{itemize}
						\item if $v\%2 = b$, then: return $v$
						\item else: wait for receiving $f+1$ $\val(\id,v')$ messages from distinct parties containing the same $v'$ such that $v'\%2=b$, then return $v'$
					\end{itemize}
					
				\end{itemize}
				\vspace{-0.1cm}	 
			}
		}
	\vspace{-0.3cm}
		\caption{ $\tcvba$ protocol built from any $\ABA$ ``black-box''}% of Algorithm 7 in  \cite{guo2020dumbo}.}
		\label{fig:blackaba}
	\end{footnotesize}
	  \vspace{-0.2cm}
\end{figure}




%\noindent
%{\bf Security and efficiency analyses}.
%.



\ignore{
\subsection{Analyzing $\tcvba$ construction}
\textbf{Details of the TCBA} The two consecutive value byzantine agreement algorithm is described in Algorithm \ref{fig:tcvba}.


If for any honest party, their input range is two consecutive value R and R-1, then, the TCBA guarantees achieve the following three properties:\:

\begin{lemma}
	\emph{\textbf{Agreement:} if any correct party outputs the value $\upsilon $, then every corrects party output $\upsilon $.}
\end{lemma}


\begin{proof}
	
	Suppose the  $P_i$ is the first correct party outputs the value $\upsilon $ which at round $r$. If the others correct nodes also have a output at round $r$, since all correct node have the same common coin at round $r$, hence, all correct nodes will output the same value $\upsilon $.
	
	Since $P_i$ have a output $\upsilon $, then $val_r = \{\upsilon\}$ at round $r$.  According to the protocol, we can know $P_i$ received the message $AUX[r](\upsilon^{})$ from at least $n-t$ different partys, sinces at most $f$ Byzantine party, it follows that $P_j$ has received $AUX[r](\upsilon^{})$ from at least $n -2f$ different correct party, but $n=3f+1$, hence $AUX[r](\upsilon^{})$ from at least $f+1$ correct party.
	
	Consider the other correct party $P_j$ have $val_r = \{\upsilon^{'}\}$ at round $r$, then $P_j$ received the message $AUX[r](\upsilon^{'})$ from at least $(n-f)$ different party. As $(n-f)+(f+1) > n$, it follows that one correct party sent $AUX[r](\upsilon^{'})$ to $P_j$ and $AUX[r](\upsilon^{})$ to $P_i$. But one correct party sent the same $AUX[r]$ message to all the party. Hence $\upsilon^{}=\upsilon^{'}$. 
	
	Hence, if the other correct party $P_j$ does not output at round $r$, then $P_j$ necessarily have $val_r = \{R, R-1\} $. It follows that such $P_j$ will execute line 17-23, and assigns the value of modular 2 equal the common coin to its estimate $est_{j+1}$.
	
	So, the estimates$_{r+1}$ of all the correct party  modular 2 are equal to the common coin$_r$, which is the ouput value $\upsilon$ at round $r$. In this case, all the correct party  have the same estimate value $\upsilon$ at beginning of round $r+1$, the set $values_{r+1}$ of every correct nodes $P$ only contains $\upsilon$ after execute line 1-6.
	
	Then, the other correct party $P_j$ continue looping until $random_{r^{'}}$ = $\upsilon\%2$ for some round $r^{'} > r$, in this time, $P_j$ also have a output $\upsilon$.$\hfill\blacksquare$ 
\end{proof}

\begin{lemma}
	\emph{\textbf{Validity:} if all correct party output the value $\upsilon $, then the value $\upsilon$ was input by at least one correct party.}
	\label{Validity}
\end{lemma}	

\begin{proof}
	Suppose the correct party $P_i$ have a output $\upsilon $ at round $r$ , then $val_r = \{\upsilon\}$.  According to the protocol line 7-9, we can know $P_i$ received the message $AUX[r](\upsilon^{})$ from at least $n-f$ different partys, hence, at least $n-f$ differents party have $\upsilon \in values_r$. In this case, according to the protocol line 1-6, the value $\upsilon$ was input by at least $f+1$ differents party. Sinces at most $t$ Byzantine party, then the value $\upsilon$ was input by at least one correct party.
	
	If the value $\upsilon$ nevers input by any correct party, sinces at most $t$ Byzantine party, it follows that $\upsilon \notin values_r$ for any correct nodes after execute line 1-6, hence, $\upsilon \notin val_r$. In this case, all correct party never output the value $\upsilon $. $\hfill\blacksquare$ 
	
\end{proof}

\begin{lemma}
	\emph{\textbf{Termination:} if all correct party have a input, then every corrects party output a value.}
\end{lemma}	

\begin{proof}
	Since for any honest party, their input range is two consecutive value R and R-1. Without loss of generality, $|R| >|R-1|$, in this case, $|R| >f+1$(maybe also have $|R-1| >f+1$ if the corrupted node also input value R-1), the line 3-5 will gurantee all correct node broadcast $Val_{r}(\upsilon)$. That is also gurantee all nodes can receive $Val_r(\upsilon )$ messages from $2f+1$ different nodes, hence, at least $2f+1$ differents node's $values_r\neq \emptyset$ is true. According the proof 3.1, we can know at the end of some round $r$, all correct node will have same estimate value, and $values_{r+1}$ only contain the same one value $\upsilon$. Then, all correct party $P$ will wait until $random_{r^{'}}$ = $\upsilon\%2$ for some round $r^{'} \geq r$, in this time, All correct party $P$ output a value $\upsilon$. $\hfill\blacksquare$ 
	
\end{proof}	

}








==> CCS 22 long-version/viewchange.tex <==
%!TEX root=main.tex

\section{View change}
\label{sec:viewchange}

\subsection{Strong Total-Order Broadcast(STOB)}

Definition 1


Strong Total-Order Broadcast

==> conclusion.tex <==
%!TEX root=main.tex

\section{Conclusion}

==> fsacs.tex <==
%!TEX root=main.tex

\section{Fast Asynchronous Common Subset}



\subsection{Definition of asynchronous common subset}


In particular, we follow the elegant prior art of HoneyBadger BFT to let the pessimistic path center around asynchronous common subset  ($\acs$), which can be defined hereafter.

\begin{definition}{\bf asynchronous common subset  ($\acs$).}
	An asynchronous common subset $\acs$ with identification $\id$ is denoted by $\acs[\id]$, and satisfies the following properties except with negligible probability:
	\begin{itemize}
		\item {\bf Validity}. If a correct node outputs a set $\bf v$, then $|{\bf v}| \ge n - f$ and ${\bf v}$ contains the inputs of at least $n - 2f$ correct nodes.
		\item {\bf Agreement}. If a correct node output a set $\bf v$, then every node outputs the same set $\bf v$.
		\item {\bf Termination}. If $n-f$ correct nodes receive an input, then every correct node delivers an output.
	\end{itemize}
\end{definition}

{\em Remark}. We emphasize that this paper will not focus on designing new concrete construction of asynchronous common subset to improve the pessimistic path, as it actually targets to design an efficient way to grafting a super-efficient optimistic path into existing fully asynchronous BFT protocols. We might adopt the best performing constructions of $\acs$ so far due to \cite{honeybadger}. More importantly, due to our modular  protocol design and analysis, any $\acs$ construction (e.g. from MVBA \cite{cachin01}) can be adopted.



\subsection{Constructing fast asynchronous common subset ($\fACS$)}

Observation of the HoneybadgerBFT, we notice that the protocol concurrently invoke $ N $ instances of RBC and $N$ instance of ABA, it dominates the message complexity to $\mathcal{O}(N^3)$ for each committed ACS. The heavy message complexity restricts the performance of latency significantly. 

Hence, we hope to improve the message complexity. We present a new $\acs$, called $\fACS$. It's a trade-off compare with HoneybadgerBFT's $\acs$, since it have
message complexity to $\mathcal{O}(CN^2)$ and the communication complexity to $\mathcal{O}(CN^2|m|)$; however, the HoneybadgerBFT's $\acs$ have message complexity to $\mathcal{O}(N^3)$ and the communication complexity to $\mathcal{O}(N^2|m|)$. The $\fACS$ protocol algorithm is described in Algorithm \ref{alg:fsACS} with $f<N/a$ byzantine failures, suppose $a \geqslant 3$ and $C$ are constants. In our main protocol, it still will invoke the sub-protocols RBC, leader-election and ABA, but it concurrently runs only $ C $ instances of RBC and $ C $ instances of ABA per epoch (instead of $N$). 

 In the $\fACS$, the leader-election sub-protocol is a important tool. We choose a small number $C$ because the size of leaders determines the costs of our protocols, however it also affects the security. We need to ensure that there will be at least one honest node in the leader set, otherwise the \textit{termination} of the $\fACS$ is not guaranteed.  In the $\fACS$, We make sure that the probability of at least one honest node in $C$ with overwhelming probability regarding security parameters.

Generally speaking, trivially setting $ C $ to $ f+1 $ is OK. If the number of Byzantine node is very small, or when the system scale is small, we can set $ C $ to $ f+1 $ to ensure safety. However it is not always the best solution. In large-scale system, it is sufficient to ensure safety choosing a much smaller $C$ via random algorithm when the number of Byzantine node is linear with the $N$.

Hence, we consider if the number of Byzantine node is independent of the $N$ (when $f$ is chosen to be a very small number), we will choose the simple round-robin leader election algorithm. If the number of Byzantine node is linear with the $N$, we will choose the random leader election algorithm to select $C$ leaders. 

As illustrated in Figure 3, the $\fACS$ protocol can be decomposed in four logical phases. The detailed protocol process as follows:
\begin{itemize}
	\item \textbf{First}, for consecutive epoch $i$, all nodes invoke leader-election protocol to elect $C$ leader;
	
	\item \textbf{Second}, all nodes send their message $\{V_i,\sigma_i\}$ to all leader;
	
	\item \textbf{Third}, for each leader $P_j$: Upon delivery $N-f$ valid message from distinct $N-f$ node, then collect these messages into a set $S$, the broadcast the set $S$ with RBC$_j$ protocol;
	
	\item \textbf{Fourth}, for any node, upon delivery $S_j$ from RBC$_j$, if input has not yet been provided to ABA$_j$, then provide input 1 to ABA$_j$; if upon delivery value 1 from any ABA$_{j}$ instance, then input 0 to other ABA instances if input has not yet been provided.
	
	\item \textbf{Fifth}, Upon all $C$ ABA instance have completed, then if the ABA of $P_{j}$ output 1, then put the $S_j$ add into the set $S$. Finally output $\cup _{V \in S}V$. 
	
\end{itemize}



\begin{figure}[H]
	\begin{footnotesize}
	\centering
	\label{alg:fsACS}
	\fbox{%
		\parbox{\linewidth}{%
			\begin{center}
				{\bf the $\fACS$ algorithm (for party $ P_{i} $) in consecutive epoch $ r $} 
			\end{center}	
			\begin{flushleft}
					\item Let RBC$ _{j} $ refer to an instance of the reliable broadcast protocol of the block-proposing stage where $ P_{j} $ is the leader.
				
				\item Let ABA$ _{j} $ refer to an instance of the asynchronous binary byzantine protocol correspond to the leader $ P_{j} $. Let $\{ABA_i\}_C$ refer to $ C $ BA instances.
				
				\begin{itemize}[noitemsep,topsep=0pt]
					\item Invoke leader-election protocol to elect $C$ leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$; {\color{cyan} // Leader election}
			
					\item Send message $\{V_i,\sigma_i\}$ to all leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$; {\color{cyan} // All node broadcast}
						
						
					\item if $P_i$ is leader then {\color{cyan} // Leader broadcast}
					\begin{itemize}[noitemsep,topsep=0pt]
							\item 	Upon delivery $N-f$ valid message $\{V_j,\sigma_j\}$ from distinct $N-f$ node $P_j$; then
							\item   Input the set $S_i=\{\{V^{'}_1,\sigma_{1}^{'}\},\{V^{'}_2,\sigma_{2}^{'}\},\cdots,\{V^{'}_{N-f},\sigma_{N-f}^{'}\}\}$ to RBC$_i$ protocol;						
					\end{itemize} 
						
					\item Upon delivery $S_j$ from RBC$_j$, if input has not yet been provided to ABA$_j$, then provide input 1 to ABA$_j$;
						
					\item Upon delivery of value 1 from any ABA instance, then input 0 to other ABA instances if input has not yet been provided.
						
					\item Upon  all C ABA instances have completed, then if the ABA of $P_{j}^{'}$ output 1, where $P_{j}^{'}$ is a leader, then put the $S_j$ add into the set $S$;				
					
		    		\item Return $\cup _{V \in S}V$.  	
						
					\end{itemize} 
				
			\end{flushleft}
		}
	}
	\caption{$\fACS$}
	\end{footnotesize}
\end{figure}


\begin{comment}

\begin{breakablealgorithm}
	\caption{the $\fACS$ algorithm (for party $ P_{i} $) in consecutive epoch $ r $}
	\label{alg:fsACS}
	\begin{algorithmic}[1] 
		

		\State Let RBC$ _{j} $ refer to an instance of the reliable broadcast protocol of the block-proposing stage where $ P_{j} $ is the leader.
		
		\State Let ABA$ _{j} $ refer to an instance of the asynchronous binary byzantine protocol correspond to the leader $ P_{j} $. Let $\{ABA_i\}_C$ refer to $ C $ BA instances.
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	-----------------Step1: Leader election-----------------}\vspace*{0.1 cm}
		\end{center}
		
		\State \textbf{Invoke} leader-election protocol to elect $C$ leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$;
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{------------------Step2: All node Broadcast------------------}\vspace*{0.1 cm}
		\end{center}
		
		\State \textbf{Send} message $\{V_i,\sigma_i\}$ to all leader $\{P_1^{'},P_2^{'}\cdots,P_C^{'}\}$;
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{------------------Step3: Leader Broadcast------------------}\vspace*{0.1 cm}
		\end{center}
		
		\If{$P_i$ is leader}
		
		\State \textbf{Upon} delivery $N-f$ valid message $\{V_j,\sigma_j\}$ from distinct $N-f$ node $P_j$;
		
		\State \textbf{then} input the set $S_i=\{\{V^{'}_1,\sigma_{1}^{'}\},\{V^{'}_2,\sigma_{2}^{'}\},\cdots,\{V^{'}_{N-f},\sigma_{N-f}^{'}\}\}$ to RBC$_i$ protocol;
		
		\EndIf
		
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{---------------------Step4: Decision---------------------}\vspace*{0.1 cm}
		\end{center}
		
		\State \textbf{Upon} delivery $S_j$ from RBC$_j$, if input has not yet been provided to ABA$_j$, then provide input 1 to ABA$_j$;
		
		\State \textbf{Upon} delivery of value 1 from any ABA instance, then input 0 to other ABA instances if input has not yet been provided.
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{-----------------------Step5: Output--------------------}\vspace*{0.1 cm}
		\end{center}
		
		\State\textbf{Upon} all C ABA instances have completed, then if the ABA of $P_{j}^{'}$ output 1, where $P_{j}^{'}$ is a leader, then put the $S_j$ add into the set $S$;
		
		
		\State\textbf{Finally} output $\cup _{V \in S}V$.  
		
	\end{algorithmic}
\end{breakablealgorithm}

\end{comment}

\subsection{Analyzing $\fACS$ construction}

In here, we prove the construct of the $\fACS$ satisfies all properties of $\acs$ with overwhelming probability regarding security parameters.

\begin{lemma}
	\emph	{\bf Termination}. If $n-f$ correct nodes receive an input, then every correct node delivers an output.
\end{lemma}	

\begin{proof}

According election-leader protocol, after invoke the protocl, all honest can terminate and receive the same leader set. Since $n-f$ correct nodes receive an input, so the leaders can receiving at least $n-f$ valid message. Besides, there are at least one honest node in the leader set, so at least one ABA instance can finished, in this case, all node will have a input to all instance, according to the termination properties of ABA, all node can completed the all ABA instance, hence, according to the algorithm \ref{alg:fsACS}, every correct node delivers an output.


	$\hfill\blacksquare$ 
\end{proof}

\begin{lemma}
	\emph	{\bf Agreement}. If a correct node output a set $\bf v$, then every node outputs the same set $\bf v$.
\end{lemma}	

\begin{proof}
	 Suppose two correct node $P_i$ and $P_j$ output different $\bf v$ and $\bf v^{'}$, respectively. Then according to the algorithm \ref{alg:fsACS}, $P_i$ and $P_j$ must received different value from a same ABA instance. But it's contradiction with the agreement properties of ABA. Hence, every node outputs the same set $\bf v$.

	
	$\hfill\blacksquare$ 
\end{proof}

\begin{lemma}
	\emph{\bf Validity}. If a correct node outputs a set $\bf v$, then $|{\bf v}| \ge n - f$ and ${\bf v}$ contains the inputs of at least $n - 2f$ correct nodes.
\end{lemma}	

\begin{proof}
	Suppose a correct node outputs a set $\bf v$, according to the algorithm \ref{alg:fsACS}, It's clear that $|{\bf v}| \ge n - f$. Besides, here at most have $f$ byzantine node, hence, it also clear that ${\bf v}$ contains the inputs of at least $n - 2f$ correct nodes.
	
	$\hfill\blacksquare$ 
\end{proof}




\subsection{Cost of the $\fACS$}

In this part, we analysis the message complexity and communication complexity of $\fACS$ protocol. From section 2 we know: The RBC messages complexity is $\mathcal{O}(n^2)$ and communication complexity is $\mathcal{O}(n|m|)$. The ABA messages complexity is $\mathcal{O}(N^2)$ and communication complexity is $\mathcal{O}(n^2)$.

According to the pseudocode of algorithm \ref{alg:fsACS}, the message exchange appears in the next seven place:	
\begin{itemize}		
	\item \textbf{1:} all node participate the leader-election instance;
	\item \textbf{2:} all node multicast message to all leader;
	\item \textbf{3:} the leaders boardcast messages to all node with RBC;
	\item \textbf{4:} all node participate the $C$ ABA instance;

\end{itemize}


\noindent \textbf{The $\fACS$ message complexity:} in place 1, the messages complexity is $\mathcal{O}(n^2)$, in place 2, the messages complexity is $\mathcal{O}(Cn)$, in place 3, the messages complexity is $\mathcal{O}(Cn^2)$. in place 4, the messages complexity is $\mathcal{O}(Cn^2)$. Hence, the $\fACS$ messages complexity is $\mathcal{O}(Cn^2)$.
\vspace{0.2cm}

\noindent \textbf{The $\fACS$ communication complexity:} in place 1, the communication complexity is $\mathcal{O}(Kn^2)$; in place 2, the communication complexity is $n*C*\mathcal{O}(|m|+K)$=$\mathcal{O}(Cn(|m|+K))$; in place 3, the communication complexity is $C*n*\mathcal{O}(n(|m|+K))$=$\mathcal{O}(Cn^2(|m|+K))$; in place 4, the communication complexity is $C\mathcal{O}(n^2)$=$\mathcal{O}(Cn^2)$. Hence, the $\fACS$ communication complexity is $\mathcal{O}(Kn^2)$+$\mathcal{O}(Cn(|m|+K))$+$\mathcal{O}(Cn^2(|m|+K))$+$\mathcal{O}(Cn^2)$=$\mathcal{O}(Cn^2(|m|+K))$, where the length of a threshold signature and a signature share at most is $K$ bits. It's rasonable consider $|m|>>nK$. So the $\fACS$ communication complexity is $\mathcal{O}(Cn^2|m|)$.


==> hybrid.tex <==
%!TEX root=main.tex

\newpage

\section{The Hybrid BFT for atomic broadcast}

The hybrid protocl proceed in sequential round numbered $r$ for each consecutives epoch $e$. For each epoch $e$, consiting of an optimistic phase and recovery phases. A leader was designated for each epoch $e$ in the optimistic phase, it is responsible to broadcast the $n-f$ incoming message to all partys. If the leader don't follow the protocol or when network delay is unexpected, the protocol will swithches to the recovery phase. In fact, the optimistic phase guarantees the agreement and total order properties, but not the liveness property; however, the protocol can effectively determine if the liveness are potentially threatened, the hybrid BFT can get guarantees the liveness by the recovery phase.  The recovery phases can help all party make progress on same checkpoint, and guarantee to obtain some progresss on each epoch. After which all correct nodes will in a consistent state, the optimistic phase starts again with a new leader by \liang{round-robin} election.

\subsection{The optimistic phase of the Hybrid BFT}
In the optimistic phase of epoch $e$, the party of number $(e ~mod ~n)+1$ as the current epoch's leader. Every party have one initial queue, in this quene, the last three block is the $\pending$ block, $1$-$\notarized$ block and $2$-$\notarized$ block.  
%where $\pending$ block stores received message from leader but not yet delivered; $D$ stores all delivered message. 
Every party also maintains an array log of size $B$ that acts as a buffer for all message to deliver in the current epoch. 

\textbf{Details of the optimistic phase:} The optimistic phase algorithm is described in Algorithm \ref{alg:optimistic}. 

For a leader party, in every round, it will wait for receive some valid message from $n-f$ distinct party, upon received $n-f$ valid message, it will forward these message to all node and into next rounds, a new leader will continue this process after $N$ round.

For a non-leader party, it will send message to leader in every round, and wait for receive leader's message, upon the received message is valid after verify, it will into next round and repeat this work until $N$ rounds, and then, change leader to start next epoch.


\begin{breakablealgorithm}
	\caption{The optimistic phase of protocol H-BFT for party $P_{i}$ in epoch $e$(Proceed in sequential round numbered $r$ for each consecutive epoch $e$;):}
	\label{alg:optimistic}
	\begin{algorithmic}[1] 
		
		\noindent\textbf{Initialization}:  
		
		\textbf{B} is the batch size parameter;
		
		$buf$ = [ ] is a FIFO queue of input message;
		
		$D$=$\emptyset$; \hfill \{Delivered\}
		
		$P$=$\emptyset$;\hfill \{Pending\} 
		
		%	\noindent$PP$=$\emptyset.$\hfill \{Pre-pending\}
		
		$e=1$;\hfill\{current epoch\}
		
		$r=1$;\hfill\{current round\}
		
		$s=r-1$;\hfill\{$s$ is the pending sequence numbe\}
		
		$c=0$;\hfill\{the number of current complain partys\}
		
		$l=(e~mod~n)+1$;\hfill\{current leader number\}
		
		$proof_{r}=Hash(P)$\hfill\{$P$ is the pending block\}
		
		$start(T)$;\hfill\{$T$ is the static time parameter\}
		
		complain=false;\hfill\{current party's complaint status\}
		
		recovery=false;\hfill\{current party's recovery status\}
		
		\vspace*{0.2 cm}
		\If{ party $P_i$ \textbf{is} current epoch's leader}	
		\If{$(r>B)$ or (timeout(T))}
		\State complain();
		\Else
		\State \textbf{wait for} receipt valid message $\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}$ from $n-f$ distinct party such that $m_{j}\notin D\bigcup P$;
		\If{ received  $n-f$ valid message}
		\State stop(T);
		% \State  put these message and correspond signature into a set;
		\State  \textbf{send} $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_i}$ to all party;
		\State  put $P$ add into $D$;
		\State empty(P);
		\State  put $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_i}$ add into $P$; 
		\State   $ r=r+1$;
		\State  start(T);
		\EndIf
		\EndIf
		\EndIf
		
		
		\vspace*{0.2 cm}
		\If{party $P_i$ \textbf{is not} current epoch's leader}
		\If{$(r>B)$ or (timeout(T))}
		\State complain();
		\Else
		\State \textbf{send} message $\{m_i,proof_{r},\{e,r,Hash(m_i,proof_{r})\}_{\sigma_i}\}$ to leader $P_{l}$ and $m_{i}\notin D\bigcup P$;
		\If{received a message $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_l}$ from leader $P_l$}
		\State stop(T);
		\State  input the message into verify(); 
		\If{verify()=1}
		\State  put $P$ add into $D$; 
		\State  empty(P); 
		\State  put $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_l}$ add into $P$;
		% \State  buf= buf-$D$;
		\State  $r=r+1$;
		\State  start(T);
		\EndIf	
		\If{verify()=0}
		\State complain();  
		\EndIf
		\EndIf
		\EndIf     
		\EndIf
		
		
		\vspace*{0.2 cm}
		\If{ received $(e,complain)_{\sigma_j}$ from $P_{j}$ for the first time}
		\State set $c=c+1$;
		
		\If{$c=f+1~ and ~\neg complain()$}
		\State complain();
		\EndIf
		
		\If{$c=2f+1$}
		\State complain=false;
		\State recovery=true;
		\State  recovery();
		\EndIf			
		\EndIf
	\end{algorithmic}
\end{breakablealgorithm}


\textbf{Switching to the Recovery Phase:} A correct party will switch to complain mode when one of the conditions happened as follows: 

(1) If the network conditions is unexpected, that is to say, the party can not received message from the leader after time $T$;

(2) the leader is not functioning properly, that is to say, the party verify the message invalid which received from the current leader;

(3) when B round has been finished.

When a party into complain mode, it will invoke the function $complain()$ to told all other party that he was in complain. If a party is in complain mode, he will reject accept any message expect the complain messages.  

The Hybird protocol from the optimistic phase of protocols switches to recovery phase need at least $t+1$ party was in complain mode. If the $t+1$ complaint party was correct party, in this case, the complain mode will amplify which can made all party into complaint mode. Hence, every correct party can receive enough complain message from the $n-f$ distinct party, thereby the optimistic phase will switch to the recovery phase of protocols.




\begin{breakablealgorithm}
	\caption{The function components for party $P_i$:}
	\begin{algorithmic}[1] 
		
		\noindent\textbf{function help$(r_i,S)$}
		\If{$r_i<S$}
		\State\textbf{send} $(help, r_i, S)$ to all party;
		\State\textbf{For} each  value $r \in \{r_i, r_{i}+1,\cdots,S\}$ wait for $N-2f$ valid  VAL$(r;h;b_j;s_j)$ messages such that $b_j$ is a valid Merkle branch for root $h$ and leaf $s_j$; %$\{block[r+1],\cdots, block[S]\}$; 
		\State\textbf{Upon} received $N-2f$ valid messages with same $r$ and $h$,  then decode block[r];
		\State\textbf{then} add $\{block[r_i], block[r_i+1], \cdots, block[S]\}$ into $D$ by increasing order;
		\EndIf
		
		
		
		
		
		
		
		
		
		\vspace*{0.2 cm}\noindent\textbf{function complain()}
		\State complain=true;
		\State \textbf{Send} $(e,complain)_{\sigma_i}$ to all party;
		
		\vspace*{0.2 cm}\noindent\textbf{function verify()}
		
		\State \textbf{input} $\{\{m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_l}$;
		
		\If {for all $m_{j}: m_{j}\notin$ $ D\bigcup P$ \textbf{and}  verifysig$(\{(m_j,proof_{r},\{e,r,Hash(m_j,proof_{r})\}_{\sigma_j}\}_{2f+1}, {\sigma_l})$=1   \textbf{and}  verifysig$(e,r,Hash(m_j,proof_{r}), \sigma_j)$=1   \textbf{and} the value  $proof_{r}$ from $2f+1$ distinct party is the same}
		
		\State \textbf{return} 1;
		\Else
		\State \textbf{return} 0;
		\EndIf
		
		
	\end{algorithmic}
\end{breakablealgorithm}





\subsection{The fully asynchronous phase}


In the recovery phase of epoch $e$, all party first






the party of number $(e ~mod ~n)+1$ as the current epoch's leader. Every party have two initial queue $P$ and $D$, where $P$ stores received message from leader but not yet delivered; $D$ stores all delivered message. A party also maintains an array log of size $B$ that acts as a buffer for all message to deliver in the current epoch. 

\textbf{Details of the recovery phase:} The recovery phase algorithm is described in Algorithm \ref{alg:recovery}. 

The protocol of recovery phase is a leaderless BFT in this phase, it consists of three parts: firstly, all nodes need to agreement on the checkpoint; and then, 



For a leader party, in every round, it will wait for receive some valid message from $n-f$ distinct party, upon received $n-f$ valid message, it will forward these message to all node and into next rounds, a new leader will continue this process after $N$ round.

For a non-leader party, it will send message to leader in every round, and wait for receive leader's message, upon the received message is valid after verify, it will into next round and repeat this work until $N$ rounds, and then, change leader to start next epoch.















\begin{breakablealgorithm}
	\caption{The recovery phase of party $P_i$:}
	\label{alg:recovery}
	\begin{algorithmic}[1] 
		
		\noindent\textbf{function recovery():}
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	--------Step1: Agree on checkpoint--------}\vspace*{0.1 cm}
		\end{center}
		
		\If{$s=0$}
		\State \textbf{send} $\{recovery, e, 0, \emptyset\}_{\sigma_i}$ to all;\hfill// s is the pending sequence number; %is the complain's round number  
		\Else
		\State \textbf{send} %$(recovery, e,r,\{(proof_{r+1})_{\sigma_j}\}_{2f+1})_{\sigma_i}$to all;
		$\{recovery, e, s, \{\{e,s,Hash(m_j,proof_{s})\}_{\sigma_j}\}_{2f+1}\}_{\sigma_i}$ to all;
		\EndIf
		
		\State \textbf{wait for} received $n-f$ valid recevory messages %$\{recovery,e,s,\{(e,s)_{\sigma_{j^{'}}}\}_{2f+1}\}_{\sigma_j}$ or $\{recovery, e, 0, \emptyset\}_{\sigma_j}$ 
		from $n-f$ distinct party $P_j$;% such that these messages verify is valid and $e$ is the current epoch;
		
		
		
		\If{ received  $n-f$ valid message}
		\State Let $R=Max(s^{'}_{1},s^{'}_{2},\dots,s^{'}_{n-f})$;
		\State Propose $R$ to $TCBA$;
		\State $S\leftarrow TCBA-1$;
		\State\textbf{Return} S;
		\EndIf 
		
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	--------Step2: Make sure to obtain progress--------}\vspace*{0.1 cm}
		\end{center}
		\If{$S\leqslant 0$}
		\State Honey-badger();
		\Else
		
		\If{$r=S$}
		\State put $P$ add into $D$; 
		\EndIf
		
		
		\If{$r<S$}
		\State help$(r,S)$;
		\EndIf
		
		
		
		\If{received $(help, r_j, S)$ from party $P_j$}
		\If{$r>r_j$}
		\While {$r>r_j$ and $r_j \leqslant  S$}
		\State \textbf{let} $\{b_k\}_{k \in  [N]}$ be the blocks of an $(N-2f; N)$-erasure coding scheme applied to $block[r_j]$;
		\State \textbf{let} $h$ be a Merkle tree root computed over $\{b_k\}$;
		\State \textbf{send} $VAL(r_j;h;b_i;s_i)$ to  party $P_j$, where $b_i$ is the $i^{th}$ Merkle tree branch;					
		%	\State\textbf{then send} $\{block[r_j], block[r_j+1],\cdots,block[r_i]\}$ to $P_j$;		 
		\State $r_j=r_j+1$;		
		\EndWhile	
		\Else	
		\State discard;
		\EndIf
		\EndIf
		
		
		
		\EndIf
		\begin{center}
			\vspace*{0.1 cm}\noindent \textbf{	------------Step3: Start the next epoch------------}\vspace*{0.1 cm}
		\end{center}
		
		
		
		\State$e=e+1$;
		\State$c=0$;
		\State$empty(P)$;
		\State$buf = buf-D$;
		\State enter the optimistic phase;
		
		
	\end{algorithmic}
\end{breakablealgorithm}








\newpage

\section{The cost of the hybrid BFT}


\begin{table}[htbp]
	
	\centering  
	%	\fontsize{6.5}{8}\selectfont  
	\caption{\bf \large Asymptotic performance comparison for atomic broadcast}  
	\label{tab:performance_comparison}  
	\begin{tabular}{|c|c|c|c|c|c|c|c|}  
		\hline  
		\multirow{2}{*}{Protocol}&\multirow{2}{*}{Async?}&\multicolumn{2}{c|}{Communication Complexity}&\multicolumn{2}{c|}{Message Complexity}\cr
		\cline{3-6}  
		& &Optim.&Worst&Optim.&Worst\cr  
		\hline  
		\hline  
		PBFT&No&$\mathcal{O}(N)$&$\infty$&$\mathcal{O}(N^2)$&$\infty$ \cr
		\hline 
		CKPS01&Yes&$\mathcal{O}(N^3)$&$\mathcal{O}(N^3)$&$\mathcal{O}(N^2)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		KS02&Yes&$\mathcal{O}(N^2)$&$\mathcal{O}(N^3)$&$\mathcal{O}(N^2)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		RC05&Yes&$\mathcal{O}(N)$&$\mathcal{O}(N^3)$&$\mathcal{O}(N)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		HoneyBarger&Yes&$\mathcal{O}(N)$&$\mathcal{O}(N)$&$\mathcal{O}(N^2)$&$\mathcal{O}(N^2)$ \cr
		\hline 
		\multirow{2}{*}{Hybrid}&\multirow{2}{*}{Yes}&\multirow{2}{*}{$\mathcal{O}(N)$}&\multirow{2}{*}{$\mathcal{O}(N)$}&\multirow{2}{*}{$\mathcal{O}(N)$\multirow{2}{*}}&$\mathcal{O}(N^2)$(determistic) \cr
		\cline{6-6}  
		& &&&&$\mathcal{O}(N)$(probability)\cr  		
		
		\hline  
	\end{tabular}  
\end{table}  


==> overview.tex <==


%!TEX root = main.tex

%\subsection{Our contributions}
\medskip
\noindent{\bf Technical overview.}  The key observations and    basic ideas behind our new efficient asynchronous fallback mechanism
 can be briefly explained as follows.
%the $\sys$ framework consists of three key components:
%(i) a deterministic optimistic path, a.k.a. Bolt, supposed to be fast in benign cases but lack live assurance;
%(ii) a robust randomized pessimistic path, a.k.a. Dumbo, expected to progress in arbitrary bad networks but probably be slow;
%(iii) a pace synchronization module, a.k.a. transformer, designed to assist efficient fallback  to Dumbo in case that Bolt loses liveness. 











{\em Prior technique}. 
%In the optimistic case, when messages are delivered within a guessed time parameter $\tau$ and the fastlane leader is honest, 
It is intuitive as in \cite{kursawe05,cachin05} to directly deploy a stable leader version of a (partially) synchronous broadcast protocol for the optimistic path. When sufficient parties feel that the optimistic path is not making fast enough progress (or no progress at all), they could start the pace synchronization
%
%In the optimistic asynchronous BFT protocols, ``pace'' synchronization is the key  to enable the parties who quit from the optimistic path to cooperatively decide
to jointly determine how many blocks  are indeed optimistically outputted  so they can sync  up to here, and more importantly, 
this shall not rollback too many optimistic outputs;
otherwise,  the confirmation of optimistic paths would be slowed down. For example, if $k$ optimistic blocks could be rolled back at worst, then an optimistic block can be finalized   only after $k$ more optimistic blocks are outputted.

To bound the rollback of optimistic blocks,
prior studies let the honest parties sign and   broadcast their current ``paces'' in the optimistic path, 
then each party can wait $n-f$ such pace-signature pairs and take them as input to invoke an MVBA instance. 
A set of $n-f$ valid pace-signature pairs would   be chosen by   MVBA and returned to all honest parties.
Since each signed pace is also attached with a small proof attesting that at least $n-2f$ honest parties indeed output its precedent blocks,  
the parties can choose the maximum pace out of the output set of MVBA minus one as the final common pace of optimistic path to sync up, 
which would simply bound the rollback of optimistic path because the MVBA result contains at least one honestly signed pace that is at most one block earlier than the latest block outputted by the optimistic path.




{\em Our methodology}. We realize that the above ``pace'' synchronization  of using a whole set of $n-f$  pace-signature pairs as MVBA input is unnecessary.
At the core of the $\sys$ framework,
we provide a highly efficient alternative ``pace'' synchronization mechanism  as fast as binary agreement.
%which can avoid the costly and slow MVBA module as well as strictly bound the possible rollback of optimistic blocks.

Our main observation lies in the fact that: there are at least $n-2f$ honest parties that do output the latest two optimistic path blocks,
so once all parties receive $n-f$ valid pace-signature pairs,
they can simply compute the maximum among these paces. Thanks to the ``notarizability'' of our fastlane abstraction, the honest parties would get either the same value or two consecutive integers,
and our task of ``pace'' synchronization is therefore reduced to make the honest parties choose one common integer out of those two unknown consecutive values. 
To this end, we propose and construct a novel asynchronous Byzantine agreement primitive to solve the specific issue of agreeing between two uncertain consecutive values. The construction has  message patterns and execution flows exactly same to the state-of-the-art binary agreement protocol in \cite{guo2020dumbo} %(and its instantiation version \cite{guo2020dumbo}) 
and only has three different lines in pseudocode for checking  slightly updated ``if-else'' conditions.


%{\em Other design mindsets}.
For the   efficiency of this new pace synchronization,
we now can adopt some more aggressive  optimistic tactics as follows.
First, different from \cite{kursawe05} that keeps on running optimistic path until it becomes problematic, we can proactively and even frequently raise ``pace'' synchronizations once the optimistic path has made enough progresses, 
which is important to ensure ``fairness'' when the optimistic path is leader-based. 
%Without an efficient ``pace'' synchronization, proactive switches optimistic path leaders would cause extra overhead.
Second, different from \cite{kursawe05,cachin05} where the pessimistic path is always executed after ``pace'' synchronization, we now can invoke the pessimistic path only if the optimistic path is completely failed, i.e., even if the optimistic path seemingly goes problematic during the course of executing, 
we would keep on trying the optimistic path again after ``pace'' synchronization as long as it remains to return some minimal output (e.g.,   one single block).





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{

barrier. Essence of optimistic path compatible with efficient fallback.


Asynchronous safety is too broad to describe the  that are  with 




\yuan{todo:  seems it is worth to put forth the notion of optimistic liveness for the hybrid paper. The story can be more clean with it. 1. Liveness in async is inherently randomized and therefore suspiciously heavyweight; 2.  a notion called optimistic liveness}
We for the first time give a positive answer to the above open problem.
To characterize what we mean by “fast” or “instant confirmation”, we adopt the same notion of
responsiveness as proposed in the work by Attiya, Dwork, Lynch, and Stockmyer [2] and later
adopted by others [27, 41]. A consensus protocol is said to be responsive iff any transaction input
to an honest node is confirmed in time that depends only on the actual network delay, but not on
any a-priori known upper bound on the network delay. Henceforth in this paper, we use $\delta$ to denote
the actual network delay and use $\Delta $ to denote an a-priori known upper bound of the network’s
delay where $\Delta $ is possibly provided as input to the protocol.
As shown in [41], achieving responsiveness requires us to assume that 2/3 of the players are
honest. (Additionally, all known protocols that are responsive are very complicated, and thus hard
to implement.)
Towards overcoming this issue, we here instead consider a notion of optimistic responsiveness—where responsiveness is only required to hold whenever some “goodness conditions” are
satisfies. More precisely, we consider two sets of conditions:

{\bf Optimistic-case and pessimistic-case.}
\begin{itemize}
	\item Worst-case conditions.
	\item Optimistic-case conditions.
	\item Pessimistic-case conditions.
\end{itemize}


{\bf $\sys$ in a nutshell.}
%, and bridge the gap between the high demands of the consortium blockchain and the robust asynchronous BFT protocols. 
%
On the core of our protocol design, we provide an efficient asynchronous ``view-change'' subprotocol to 
graft a simple optimistic path to a heavier fully asynchronous pessimistic path, 
such that we can hope the best of both. 
In particular, when the optimistic path succeeds to progress, the cost is rather low due to the extreme simplicity of the optimistic path. Even if the optimistic path fails to be live (e.g. due to corrupted leader or unstable network), our ``view-change'' subprotocol allows all correct nodes smoothly fall back into the backup pessimistic path to ensure robust liveness with incurring merely little  overhead that is asymptotically small.

In greater detail, our protocol is repeating to proceed in epoch, and in each epoch, it consists of three critical ingredients hereafter:
\begin{itemize}
	\item {\bf Optimistic path.} 
	Every epoch will begin with trying a simple and highly efficient leader-driven optimistic path, which leverages the  ``pipelining'' idea that was initially hinted by  Lamport \cite{paxos}, and recently revived in the lens of blockchain \cite{hotstuff, sync-hotstuff, pala, casper}.
	The ``pipelining'' design through the lens of blockchain is deemed as the crux to realize the optimistically higher performance, and involves only two types of messages, namely, $\propose$ and $\decide$. The $\decide$ message is sent from the leader to nodes (along with the decided output), while $\propose$ messages are sent from nodes to the leader (along with some proposed input).
	
	
	Generally speaking, in each epoch, a leader node is  ``elected'' (or assigned) to drive the optimistic path to proceed by slots: (i) in each slot,
	the leader node collects $\propose$s from the network, and each $\propose$ contains a digital signature for the $\decide$ committed by the leader in the immediate  precedent slot; (ii) upon the leader receives $n-f$ $\propose$s, the leader can commit a new $\decide$ message for the current slot, and this new $\decide$ message shall include $n-f$ valid signatures for the previous slot's $\decide$; (iii) later, upon receiving the new $\decide$ from the leader, a node checks the message contains $n-f$ valid signatures for the precedent $\decide$, and then digitally signs this current $\decide$ to create a new $\propose$ sent back to the leader for the next slot; (iv) and so forth.
	%
	
	The above scheme follows the recent elegant results on ``pipelining'', and is intuitively high-performing in case both the leader is correct and the timing assumption holds. 
	%In our instantiation, we require the optimistic path of each epoch stop after .
	
	%More importantly, even for arbitrary malicious leader and network, we can observe that: upon receiving a new valid $\decide$ from the leader, a node can extract a string that we call notarization string\footnote{The notarization string might also known as the quorum certificate in the literature.} to attest that ``at least $n-2f$ correct nodes already voted for the same precedent $\decide$ that I voted for''. 
	
	%To interpret the above fact one step further, let a node call its recently received proposal as $\pending$, the immediate precedent proposal as 1-$\notarized$, and the second precedent proposal as 2-$\notarized$, which immediate helps us conclude: once a correct node can extract a notarization string to attest ``at least $n-2f$ correct nodes already voted for its 1-$\notarized$ proposal'', these $n-2f$ correct nodes can also produce notarization strings to attest ``''.
	% This fact further means
	
	\item {\bf View-change.} The view-change protocol is activated and then be terminated, as long as at least $n-2f$ correct nodes ``abandon'' the optimistic path. In our instantiation, a correct node abandons the optimistic path, either when it feels no progress made for a while, or when the optimistic epoch is supposed to be completed as the number of already delivered messages has reached a parameter called epoch size. As such, we indeed place the view-change subprotocol in the critical path of optimistic cases. Remark that such the choice will not introduce much overhead, as view-changes are optimistically rare, especially when we moderately tune up the parameter of epoch size to allow honest leaders drive an epoch for a while.
	
	The efficiency of our view-change component stems from the nice properties of the optimistic path, that are: even for arbitrary malicious leader and network, upon receiving a new valid $\decide$ message from the leader (for the current slot), a correct node can extract a string that we call notarization string\footnote{The notarization string might also known as the quorum certificate in the literature.} to attest that ``at least $n-2f$ correct nodes already voted for the same precedent $\decide$ that I voted for in the previous slot''; in addition, the notarization string can be easily public verified, as it is essentially a set of signatures (bounded to slot numbers); more importantly, if  $\decide$ was not received and voted by $n-2f$ correct nodes in the corresponding asynchronous slot, the notarization string for it cannot be forged by the adversary due to the security of digital signature.
	
	The above facts hint us a solution towards constructing the asynchronous view-change with $\bigO(n^2)$ communications. 
	The basic idea is to let each correct node simply multicast  a view-change message that includes the ``highest'' notarization string abstracted from the optimistic path. Such the view-change message essentially makes a trial to convince the network: ``which slot I am at'' (i.e., ``what is my view'').
	Then, each node simply waits for $n-f$ validly notarized view-change messages from distinct nodes, and count the highest ``view'' out of  the $n-f$ notarized ``views'' as an important intermediate result called by $\maxview$.
	%
	After the multicast of view-change messages, we catch up with another crucial observation   to make our asynchronous view-change asymptotically better than prior studies, which is: $\maxview$s of all correct nodes are already somehow weakly-agreed, say correct nodes' $\maxview$s must either be the same integer (i.e. corresponding the same slot), or two consecutive integers (i.e. corresponding two consecutive slots). These weakly-agreed $\maxview$s correspond the cornerstone to efficiently make the correct nodes agree on how the progress made during the abandoned optimistic path. In particular, we formalize the special Byzantine agreement problem that correct nodes input two consecutive integers, and propose a simple construction with $\bigO(n^2)$ messages and $\bigO(1)$ expected running time  (see more details about the two-consecutive-value Byzantine agreement in Section \ref{sec:tcvba}).
	
	After all, the correct nodes will agree on how many messages are already delivered during the just abandoned optimistic epoch. More importantly, the above view-change procedure ensures at least $n-2f$ correct nodes indeed deliver the output messages up to the agreed ``view'', indicating that the correct nodes who did not deliver these outputs yet can always trivially sync up to this agreed ``view''.
	
	\item {\bf Pessimistic path.} Once the ``view-change'' subprotocol is terminated, all correct nodes can reach an agreement on how much progress the optimistic path does. In case too less progress (e.g., smaller than a security parameter) has been done in the optimistic path of the epoch, a heavier but robuster asynchronous BFT protocol is activated and then terminated. This asynchronous path (or interchangeably called pessimistic path) is inspired by the breakthrough of HBBFT to center around asynchronous common subset (ACS). Once the asynchronous path is done, the protocol proceeds to the next epoch.
	
	Different from Ben-Or ACS, we design and provide an expectedly constant-round ACS called fast ACS ($\fACS$), which realizes $\bigO(1)$ running time without sacrificing the asymptotic complexity of communications; moreover, the total message complexity of ACS is reduced from $\bigO(n^3)$ to $\bigO(\kappa n^2)$ where $\kappa$ is a security parameter (e.g., $\kappa=21$).\footnote{It could be appealing at first glance to leverage the recent MVBA construction \cite{ittai19} due to Abraham {\em et al.} to construct constant-round ACS, but it is not clear how to make it without asymptotically increasing commutations. For example, when we adopt the reduction in \cite{cachin01} to construct ACS from MVBA and count an ACS input as a word, the input size of MVBA has already been $\bigO(n)$ words. Once the MVBA instantiation in \cite{ittai19} is applied, the total  communications of ACS becomes $\bigO(n^3)$ words, which is equivalent to $\bigO(n^2)$ communication  per delivered ACS input and clearly sacrifices the ``communication-optimal''.}
	%, since the MVBA in \cite{ittai19} brings $\bigO(n^2|m|)$ words where $|m|=n$ due to the ACS construction \cite{cachin01}.}
	
	
	The construction of $\fACS$ is highly inspired by Ben-Or ACS with a few exceptions to introduce a small committee consisting of $\kappa$ nodes. In high-level, $\fACS$ proceeds as: (i) call a simple randomized election subprotocol to elect a committee of $\kappa$ nodes; (ii) all correct nodes send their input-signature pairs to the $\kappa$ committee nodes; (iii) each committee node collects a set of $n-f$   input-signature pairs, and uses reliable broadcast to send the set of input-signature pairs to the network; (iv-1) every correct node executes $\kappa$ ABA instances, each of which corresponds a particular committee node; (iv-2) a correct node assigns the input of a certain binary agreement to 1, iff it receives the valid input-signature pairs from the corresponding committee node (through reliable broadcast); (iv-3) as soon as one binary agreement terminates (with output 1), $\fACS$ outputs the input-signature pairs reliably broadcasted by the corresponding committee node.
	
	Due to the above $\fACS$, the bandwidth usage (of each node) is slightly amplified by $\kappa$ times relative to Ben-Or construction. However, the $\log(n)$ running time is removed, as $\fACS$ only ``halts'' to wait the termination of constant ABAs. In addition, the message complexity is also reduced by a factor of $\bigO(n)$, because $\fACS$ only requires $\kappa$ reliable broadcasts and $\kappa$ ABAs (instead of $n$) where $\kappa$ is a constant security parameter.
	As such, we can slightly trade off the concrete bandwidth usage for asymptotically less running time and asymptotically fewer messages. 
	Remark that this new trade-off option becomes appropriate, when the system burden is small and/or the bandwidth is somehow abundant. 
	
\end{itemize}

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> preliminary.tex <==
%!TEX root=main.tex
\medskip
\section{Preliminaries}
\label{sec:pre}



 
\noindent{\bf Collision-resistance hash function.}
A hash function $\hash: \{0,1\} ^ {*} \rightarrow \{0,1\} ^ \lambda$ is said to be collision-resistant, if no probabilistic polynomial algorithm adversary can generate a couple of distinct values $x_1$ and $x_2$ subject to $\hash(x_1)=\hash(x_2)$ except with negligible probability. %Through the paper, we assume that there exists a hash function $\hash$ that is collision-resistant.
 
\smallskip 
\noindent{\bf Non-interactive threshold signature.}
A non-interactive $(t, n)$-threshold signature scheme  $\TSIG$ is a tuple of  algorithms/protocols involving $n$ parties $\{\node_i\}_{i\in[n]}$ hereunder:
\begin{itemize}
	\item $\TSIG.\Setup(1^\lambda, t, n) \rightarrow (pk, { vk}, { sk})$. Once this algorithm/protocol is completed, there generates a public key $pk$,  a vector of public verification keys ${vk} := (vk_1, \cdots, vk_n)$, along with a vector of private secret keys ${ sk} := (sk_1, \cdots, sk_n)$ where $\node_i$ gets $sk_i$ only.
	\item $\TSIG.\SignShare_t(sk_i, m) \rightarrow \sigma_i$. It takes   a message $m$ and a private key share $sk_i$ as input, and outputs a signature share $\sigma_i$. We also use $\SignShare_t(m)$ for short.
	\item $\TSIG.\VrfyShare_t(pk, { vk}, m, (i, \sigma_i)) \rightarrow \{0,1\}$. This is a deterministic algorithm taking a message $m$, the public key $pk$, the verification keys ${ vk}$, a ``partial'' signature $\sigma_i$ and an index $i$ as input. It outputs 1 or 0 depending on whether $\sigma_i$ is deemed as a valid ``partial'' signature share produced by party $\node_i$ or not. We also use  $\VrfyShare_t(m, (i,\sigma_i))$ for short.
	\item $\TSIG.\Combine_t(pk, { vk}, m, \{(i, \sigma_i)\}_{i \in [n]}) \rightarrow \sigma $. The algorithm takes  the public key $pk$, the verification keys ${ vk}$, a message $m$, along with $t$ partial signature-index pairs $(i, \sigma_i)$  as input. This algorithm either outputs a full signature $\sigma$ for message $m$, or $\bot$ when $\{(i, \sigma_i)\}_{i \in [n]}$ contains ill-formed $(i, \sigma_i)$. We might use $\Combine_t(m, \{(i,\sigma_i)\}_{i \in [n]})$ for short.
	\item $\TSIG.\Vrfy_t(pk, m,\sigma) \rightarrow \{0,1\}$. This is a deterministic algorithm that takes as input a message $m$, the public key $pk$ and an ``combined'' signature $\sigma$. It outputs 1 or 0 depending on whether $\sigma$ is the valid signature for message $m$ or not. The notation $\Vrfy_t(m, \sigma)$ can be used for short.
\end{itemize}


	Besides the  trivial {\em correctness} of enforcing all honestly produced signature shares and signatures to pass verification, we   require {\em robustness} and {\em unforgeability} for  $\TSIG$:
\begin{itemize}
	
	\item {\em Robustness}. No probabilistic polynomial time (P.P.T.) adversary can produce $t$ valid ``partial'' signature shares, s.t. running $\Combine$ to aggregate them does {\em not} produce a valid ``full'' signature, except with  negligible probability. % in $\lambda$. 
	%
	Intuitively, it ensures any $t$ valid ``partial'' signatures of a message must induce a valid ``full''  signature \cite{shoup2000practical}.
	
	\item {\em Unforgeability}. This can be defined by a threshold version Existential UnForgeability under Chosen Message Attack  game.
	%, which   means that  for any message $m$, it is computational infeasible for the adversary $\A$ (who can adaptively corrupt $f$ parties that $f < t$) to produce
	%a valid ``full'' signature for $m$, unless $\A$ submits signing requests  to $t-f$ distinct uncorrupted parties to sign $m$.
	%
	Intuitively, it ensures that no P.P.T. adversary $\A$ controlling $t-1$ parties   can produce a valid ``full'' signature except with  negligible probability, unless $\A$ receives a ``partial'' signature  produced by an honest party.  
	%See \cite{libert2012non} for the formal definition.
	
\end{itemize}

%Remark that we assume $\TSIG.\Setup$ has already been correctly executed before the start of protocols, i.e., the setup of $\TSIG$ is taken for granted. 

%Remark that through the paper, we let $(t, n)$-$\TSIG$ scheme's parameter $n$ to be same as the number of 
%threshold $t=2f+1$, where $f$ is the number of Byzantine faulty parties to tolerate.




\smallskip
\noindent{\bf Threshold public key encryption ($\mathsf{TPKE}$)}. A $(t, n)$-threshold public key encryption scheme $\mathsf{TPKE}$ is a tuple of  algorithms/protocols involving $n$ parties $\{\node_i\}_{i\in[n]}$:
\begin{itemize}
	\item $\TPKE.\Setup(1^\lambda, t, n) \rightarrow (epk, { esk})$. It generates a public encryption key $epk$, along with a vector of private keys ${ esk}:= (esk_1, \cdots, esk_n)$, each item of which $esk_i$ is the secret key held by the corresponding party $\node_i$.
	\item $\TPKE.\Enc(epk, m) \rightarrow c$. It   encrypts a message $m$ to a ciphertext $c$ with using the public encryption key $epk$.
	\item $\TPKE.\DecShare(esk_i, c) \rightarrow c_i$. It allows a party $\node_i$ to use its secret key $esk_i$ to produce a   decryption share $c_i$  for $c$ (or a special symbol $\bot$ in case $c$ is ill-formed).
	\item $\TPKE.\Dec(epk, \{(i, c_i)\}_{i \in  [n]}) \rightarrow m$. It combines a set of valid decryption shares $(i,c_i)$ from at least $t$ distinct parties to reconstruct the plaintext $m$.
\end{itemize}

The {\em  correction} requirement of $\mathsf{TPKE}$ is obvious, which is any $t$ honest parties can cooperate to decrypt a ciphertext $c$ to get the corresponding plaintext $m$, as long as $c$ is produced by an honest party to encrypt $m$. 
%
Informally speaking, we expect an established $(t, n)$-$\mathsf{TPKE}$ scheme to be {\em robust} and {\em IND-CCA secure} (see \cite{shoup1998securing, boneh2006chosen} for rigor definitions).

%\begin{itemize}
%	\item {\bf Robustness} essentially requires the consistency of decryptions, which means no computationally bounded adversary (who statically corrupts up to $t-1$ parties) can produce a ciphertext $c$, such that two or more distinct plaintexts can be reconstructed from $c$.
%	\item {\bf Threshold-version of IND-CCA security} essentially ensures the adversary (who statically corrupts $t-1$ parties and is given decryption oracle) shall learn negligible information from a ciphertext    as if she does not see the ciphertext at all (before calling the decryption oracle to decrypt it).
	%, which is known to be strictly stronger than IND-CPA security.
%\end{itemize}

%Remark that we assume $\TPKE.\Setup$ has already been correctly executed before the start of protocols, i.e., the setup of $\TSIG$ is taken for granted. 


%\subsection{Threshold public key encryption}
%A $(t, n)$-threshold public key encryption scheme $\TPKE$ is a tuple of following four algorithms:
%\begin{itemize}
%	\item $\TPKE.\Setup(1^\lambda, t, n) \rightarrow (epk, \{esk_i\})$
%	\item $\TPKE.\Enc(epk, m) \rightarrow c$
%	\item $\TPKE.\DecShare(esk_i, c) \rightarrow c_i$
%	\item $\TPKE.\Dec(epk, c, \{i, c_i\}_{i \in S}) \rightarrow m$
%\end{itemize}



%\smallskip 
%\noindent{\bf Threshold common-coin scheme ($\coin$).} A $(t, n)$-threshold common-coin scheme $\coin[\id]$  \cite{cachin00} is a protocol joined by $n$ parties and satisfies the following properties:
%\begin{itemize}
%	\item {\em Agreement}. If $t$ parties invoke $\coin[\id]. \getcoin()$, then all honest parties that activate $\coin[\id]. \getcoin()$ can receive a common value $r \in \{0,1\} $. 
	%More importantly, the value $r$ is uniformly sampled in the range $\{0,1\}^{\lambda}$ and cannot be biased by P.P.T. adversary (who statically corrupts up to $t$ parties) except with negligible advantage.
%	\item {\em Unpredictability}. The value $r \leftarrow \coin[\id].\getcoin()$ cannot be predicated by P.P.T. adversary (who can statically corrupt up to $t-1$ parties) except with negligible advantage, until  one honest party calls $\coin[\id]. \getcoin()$.
%\end{itemize}

%Note that it is well-known to realize the above $(t, n)$-threshold common-coin scheme from an  established non-interactive $(t, n)$-threshold signature scheme among $n$ parties \cite{cachin00, honeybadger}. The detailed construction is too trivial to mention, and it only requires $\bigO(\lambda n)$ communication cost per party, $\bigO(n)$ messages per party and one asynchronous round to run.








 
\smallskip
\noindent{\bf Asynchronous binary   agreement ($\ABA$).} In an asynchronous binary agreement \cite{MMR15,lamport1982byzantine}, each party has a single-bit input, and their goal is to output a common bit. In particular, a protocol $\ABA$ running among $n$ parties with identification $\id$ is said to be asynchronous binary agreement, if it guarantees the following properties except with negligible probability:
\begin{itemize}
	\item {\em Termination}. If all honest parties pass inputs to $\ABA[\id]$, then all honest parties output associated to $\id$.

	\item {\em Agreement}. If any honest party outputs a bit $ b $  associated to $\id$,  then  all honest parties  output  the same   $ b $  on $\id$.
	
	\item {\em Validity}. If any honest party outputs $ b $ (associated to $\id$), then at least one honest party takes $ b $    as input to $\ABA[\id]$.
\end{itemize}

%We defer the concrete constructions of $\RBC$ and $\ABA$ protocols to Appendix.
 

\ignore{
\medskip
\noindent{\bf $(\eta, \kappa, \epsilon)$-Committee election ($\ACE$).} In a $(\eta, \kappa, \epsilon)$-committee election protocol running among $n$ parties (identified from $1$ through $n$) \cite{kapron2010fast,abraham2018solida}, the parties aim to output a $\kappa$-sized committee set $C$, such that $C$ is a subset of $\{1, \cdots, n\}$ containing at least $\eta$ correct parties' identities. In particular, a protocol with identification $\id$ is said to be $(\eta, \kappa, \epsilon)$-committee election, if it satisfies the following properties  in the presence of $f$ statically corrupted parties except with probability $\epsilon+negl(\lambda)$, where $negl(\lambda)$ is a negligible function of security parameter:
\begin{itemize}
	\item {\bf Termination.} If $f+1$ correct parties activate the protocol  $\ACE[\id]$, then all correct parties output (associated to $\id$).
	\item {\bf Agreement.} If a correct party outputs a committee set $C$  (associated to $\id$), all correct parties output the same set $C$  (associated to $\id$).
	\item {\bf Validity.} If any correct party outputs $C$  (associated to $\id$), then $|C|=\kappa$ and $C$ contains the identities of at least $\eta$ correct parties.
\end{itemize}

We emphasize on $(1, \kappa, \epsilon)$-$\ACE$ through the paper, namely, to elect a $\kappa$-sized committee containing at least one correct party with probability $1-\epsilon$. So $\kappa$ is essentially a security parameter of the committee election protocol \cite{abraham2019communication}.
%, and we might thus use $\ACE[\id]$ or $\kappa$-$\ACE[\id]$ as abbreviated forms of $(1, \kappa)$-$\ACE[\id]$.  
%
Also note that conditioned on  static corruptions up to $f$ as well as the already established $(f+1, n)$-threshold common-coin scheme $\coin$, for any given $\epsilon$, a security parameter $\kappa$ can be determined, such that it becomes trivial to construct $(1, \kappa, \epsilon)$-$\ACE$. Remark that the computational cost of $(1, \kappa,\epsilon)$-$\ACE$ is essentially same to $\coin.\getcoin()$.}



 
\smallskip
\noindent{\bf Asynchronous common subset ($\acs$).}
%We follow the elegant prior art to let the pessimistic path center around asynchronous common subset  ($\acs$). 
In the  $\acs$ protocol among $n$ parties (including up to $f$ Byzantine faulty parties) with identification $\id$,
each party takes as input a value and outputs a set of values.
%
It   satisfies   the following properties except with negligible probability:
	\begin{itemize}
		\item {\em Validity}. If an honest party outputs a set of values $\bf v$, then $|{\bf v}| \ge n - f$ and ${\bf v}$ contains the inputs from at least $n - 2f$ honest parties.
		\item {\em Agreement}. If an honest party outputs a set of values $\bf v$, then every party outputs the same set $\bf v$.
		\item {\em Termination}. If $n-f$ honest parties receive an input, then every honest party delivers an output.
	\end{itemize}
 

%{\em Remark}. We emphasize that this paper will not focus on designing new concrete construction of asynchronous common subset to improve the pessimistic path, as it actually targets to design an efficient way to grafting a super-efficient optimistic path into existing fully asynchronous BFT protocols. We might adopt the best performing constructions of $\acs$ so far due to \cite{honeybadger}. More importantly, due to our modular  protocol design and analysis, any $\acs$ construction (e.g. from MVBA \cite{cachin01}) can be adopted.

 

\smallskip
\noindent{\bf Strong provable  reliable broadcast ($\prbc$).} A protocol among a set of $n$ parties with   a designated sender, a predicate function  $\prbc.\Verify$  and an identification $\id$ is said to be  $\prbc$, if it satisfies the  next properties  (in presence of $f$ static   Byzantine faults) except with negligible probability:

\begin{itemize}
	\item {\em Validity}. If all honest parties invoke $\prbc[\id]$ and the sender is honest with taking a message $ m $ as input, all honest parties eventually output $m$   with proof $\sigma$  s.t. $\prbc.\Verify(\id, \sigma)=1$.
	
	\item {\em Agreement}. If two honest parties output $ m $ and $ m' $  in $\prbc[\id]$ respectively, then  $ m = m' $.
	
	\item {\em Totality}. If any (probably malicious) party outputs $ m $ and $\sigma$ in $\prbc[\id]$ s.t. $\prbc.\Verify(\id, \sigma)=1$, then all honest parties eventually output a value attached with a proof $\sigma$  s.t. $\prbc.\Verify(\id, \sigma)=1$ in $\prbc[\id]$.
	
	\item {\em Unforgeability}.  If $f+1$ or more honest parties do not activate $\prbc[\id]$, it computationally infeasible for any   party to produce a proof $\sigma$ 
	s.t. $\prbc.\Verify(\id, \sigma)=1$.
	
\end{itemize}

%\noindent
Note that {\em strong} provable  reliable broadcast adds   unforgeability   to    provable  reliable broadcast introduced in \cite{guo2020dumbo}, 
so it ensures that  when a valid proof is generated, there are enough honest parties that did activate the protocol.
Existing provable reliable broadcasts can   trivially obtain this property. For example, one can either   use any reliable broadcast as black-box with adding one extra round of multicasting $(n-f,n)$ threshold signatures as in \cite{guo2020dumbo},
or modify  Bracha's reliable broadcast \cite{bracha1987asynchronous} (or its variant \cite{honeybadger}) with encapsulating $(n-f,n)$ threshold signatures in the last $\ready$ messages as if in \cite{cachin2002asynchronous}.
%The original Bracha's RBC requires $ O(N^{2}|v|) $ bits of communication in order to broadcast a value of size $ |v| $. HoneyBadgerBFT uses RBC from Cachin and Tessaro, with erasure coding to reduce the cost to $ O(N|v|+N^{2}LogN) $.




==> viewchange.tex <==
%!TEX root=main.tex

\section{View change}
\label{sec:viewchange}

\subsection{Strong Total-Order Broadcast(STOB)}

Definition 1


Strong Total-Order Broadcast
